Finding Birkhoff Averages via Adaptive Filtering

In many applications, one is interested in classifying trajectories of Hamiltonian systems as invariant tori, islands, or chaos. The convergence rate of ergodic Birkhoff averages can be used to categorize these regions, but many iterations of the return map are needed to implement this directly. Recently, it has been shown that a weighted Birkhoff average can be used to accelerate the convergence, resulting in a useful method for categorizing trajectories. In this paper, we show how a modified version the reduced rank extrapolation method (named Birkhoff RRE) can also be used to find optimal weights for the weighted average with a single linear least-squares solve.Using these, we classify trajectories with fewer iterations of the map than the standard weighted Birkhoff average. Furthermore, for the islands and invariant circles, a subsequent eigenvalue problem gives the number of islands and the rotation number. Using these numbers, we find Fourier parameterizations of invariant circles and islands. We show examples of Birkhoff RRE on the standard map and on magnetic field line dynamics.

==> Appendices/RealAnalyticStuff.tex <==
Just to make sure I still know how to do analysis...
\begin{lemma}
    A real analytic function $f\in C^{\omega}(\Tbb_\rho)$ with $\norm{f}_\rho < \infty$ has Fourier coefficients that obey
    \begin{equation*}
        \abs{f_n} \leq \norm{f}_\rho e^{-n\rho}.
    \end{equation*}
\end{lemma}
\begin{proof}
    A Fourier coefficient of $f$ can be computed via
    \begin{equation*}
        f_n = \frac{1}{2\pi}\int_{\Tbb} f(\theta) e^{- i n \theta} \dif \theta,
    \end{equation*}
    where WLOG we assume $n>0$. 
    For any $\rho_* < \rho$, by deforming the integration contour vertically, we have
    \begin{equation*}
        f_n = \frac{e^{-n\rho_*}}{2\pi}\int_{\Tbb} f(\theta - i \rho_*) e^{-i n \theta} \dif \theta.
    \end{equation*}
    This can be bounded by
    \begin{equation*}
        \abs{f_n} = \norm{f}_{\rho} e^{- n\rho_*}.
    \end{equation*}
    Now, we have that
    \begin{equation*}
        \limsup_{\rho_* \to \rho} \abs{f_n} \leq \limsup_{\rho_*\to\rho} \norm{f}_{\rho} e^{-n\rho_*} = \norm{f}_{\rho} e^{-n\rho}.
    \end{equation*}
\end{proof}

\begin{lemma}
    Furthermore, we have 
    \begin{equation*}
        \sum_{\abs{n} > N} \abs{f_n} < C e^{-N\rho}.
    \end{equation*}
\end{lemma}
\begin{proof}
    We have
    \begin{align*}
        \sum_{\abs{n} > N} \abs{f_n} &< 2 \norm{f}_{\rho} \sum_{n > N}\left(e^{-\rho}\right)^n,\\
        &= \frac{2 \norm{f}_{\rho} e^{-\rho{N+1}}}{1-e^{-\rho}}
    \end{align*}
\end{proof}

==> Appendices/fourier_gaps.tex <==
\section{Distribution of gaps in a Fourier series}
\mr{A better version of this must exist somewhere...}
\begin{lemma}
\label{lemma:Fourier-gaps}
    Let $\dobsT$ be a function with a bound on the Fourier coefficients of the form $\abs{\dobsT_n} < C n^{-M}$ for some $M\geq 1$. Then for every $\epsilon > 0$, there exists a gap $\delta$ between values of $\abs{\dobsT_n}$ with the lower bound
    \begin{equation*}
        \delta > C_2 \epsilon^{1 + 1/M}.
    \end{equation*}
\end{lemma}
\begin{proof}
    First, consider the value of $N$ such that $n > N$ implies $\abs{\dobsT_n} < \epsilon/2$. This is given by
    \begin{equation*}
        N = \left( \frac{\epsilon}{2 C}\right)^{-1/M}.
    \end{equation*}
    This means that at most $N$ coefficients can be within the region $(\epsilon/2, \epsilon]$, guaranteeing a gap of size at least $\epsilon/(2N+2)$. This gives our theorem
\end{proof}

==> Appendices/integrated_convergence.tex <==

\section{Integrated Sequence Bound}
\begin{lemma}
    Let $\{a_n\}$ be a sequence with the bound $\abs{a_n} < C n^{-M}$. Then,
    \begin{equation*}
        \abs{\sum_{n>N} a_n} \leq \sum_{n>N}\abs{a_n} \leq C_2 N^{-M+1}.
    \end{equation*}
\end{lemma}
\begin{proof}
    The first part is obvious. The second part is performed by the integral test.
    \begin{align*}
        \sum_{n > N} \abs{a_n} \leq C \sum_{n > N} n^{-M} \leq C \int_{N}^\infty x^{-M} \dif x = \frac{C}{M-1} N^{-M+1}.
    \end{align*}
\end{proof}

\begin{lemma}
\label{lemma:Diophantine}
    Let $\omegabf$ satisfy the Diophantine condition
    \begin{equation*}
        \abs{\nbf \cdot \omega - m} \geq \frac{C}{\abs{\nbf}^{\nu}}.
    \end{equation*}
    Then, 
    \begin{equation*}
        \abs{1-e^{2\pi i \nbf \cdot \omegabf}} > \frac{2C}{\abs{\nbf}^{\nu}}.
    \end{equation*}
\end{lemma}
\begin{proof}
    First, we note that 
    \begin{equation*}
        \abs{1-e^{2\pi i \nbf \cdot \omegabf}} = \abs{\sin\left(\pi (\nbf \cdot \omegabf - m) \right)},
    \end{equation*}
    where we assume $m\in \Zbb$ is chosen so that $\abs{\nbf \cdot \omegabf - m}\leq 1/2$. On this domain, the function 
    \begin{equation*}
        \abs{\sin\left(\pi (\nbf \cdot \omegabf - m) \right)} > 2\abs{\nbf \cdot \omegabf - m} \geq \frac{2C}{\abs{\nbf}^{\nu}}.
    \end{equation*}
\end{proof}

\begin{theorem}
    Under Hypotheses \ref{setting} with $M > \nu + d$, the unweighted Birkhoff average of invariant circles converges as $\Ocal(T^{-1})$. 
\end{theorem}
\begin{proof}
    The unweighted Birkhoff average is given by
    \begin{align*}
        \BA_T[\obs](\xbf) = \sum_{t = 0}^{T-1} \frac{1}{T} (\obs \circ \zbf)(\thetabf + \omegabf).
    \end{align*}
    Using the Fourier series representation of $\obs \circ \zbf$, we have
    \begin{align*}
        \BA_T[\obs](\xbf) - h_0 &= \frac{1}{T} \sum_{\nbf \in\Zbb^d \backslash\{0\}} \obsT_{\nbf}  \sum_{t=0}^{T-1}e^{2\pi i t \nbf \cdot \omegabf},\\
        &= \frac{1}{T} \sum_{\nbf \in\Zbb^d \backslash\{0\}} \obsT_{\nbf} \frac{e^{-2\pi i \nbf \cdot \omegabf}-e^{2\pi i (T-1)\nbf \cdot \omegabf}}{1-e^{2\pi i \nbf \cdot \omegabf}}.
    \end{align*}
    Using the continuity bounds $\abs{\obsT_{\nbf}}<C_h \abs{\nbf}^{-M}$ and Lemma \ref{lemma:Diophantine}, we have
    \begin{align*}
        \abs{\BA_T[\obs](\xbf) - h_0} & \leq \frac{C_h}{C T} \sum_{\nbf \in\Zbb^d \backslash\{0\}} \obsT_{\nbf} \abs{\nbf}^{-M + \nu}.
    \end{align*}
    For the convergence of this sum, we require $-M+\nu < -d$, or $M > d+\nu$.
\end{proof}

==> Appendices/symmetric_eigenvalue_perturbation_theorems.tex <==
\section{Eigenvalue Problem Perturbation Theorems}
Here, we quote three eigenvalue perturbation theorems used in the proofs herein. For the following theorems, denote $\mathcal L(A)$ as the set of eigenvalues of a matrix $A$. All theorems are taken from Stewart and Sun\cite{Stewart1990} (SS).

\begin{theorem}[Gershgorin, SS Thm.~2.2.1]
\label{thm:gershgorin}
For $A \in \Cbb^{n\times n}$ let
\begin{equation*}
    R_i = \sum_{j \neq i} \abs{a_{ij}}
\end{equation*}
and
\begin{equation*}
    \mathcal G_i(A) = \left\{z \in \Cbb \mid \abs{z-a_{ii}} \leq a_i \right\}.
\end{equation*}
Then 
\begin{equation*}
    \mathcal L (A) \subset \bigcup_{i=1}^n \mathcal G_i(A).
\end{equation*}
\end{theorem}

\begin{theorem}[Weyl's, SS Cor.~4.4.9] 
\label{thm:Weyl}
Let $A$ and $E$ be symmetric matrices with eigenvalues $\{\sigma_i\}$ and $\{\epsilon_i\}$ respectively, ordered so that $\sigma_i \geq \sigma_{i+1}$ and $\epsilon_i \geq \epsilon_{i+1}$.  Then, for $i = 1, \dots, n$, the eigenvalues $\tilde{\sigma}_i$ of $\tilde{A} = A + E$ satisfy
\begin{equation*}
    \tilde{\sigma}_i \in [\sigma_i + \epsilon_n, \sigma_i + \epsilon_1].
\end{equation*}
\end{theorem}

\begin{theorem}[Davis-Kahan $\sin(\Theta)$, SS Thm.~5.3.4, 5.3.6, 5.3.8]
\label{thm:DavisKahan}
    Let $A$ be a Hermitian matrix with spectral resolution
    \begin{equation*}
        \begin{pmatrix}
            X_1^* \\ X_2^*
        \end{pmatrix}
        A
        \begin{pmatrix}
            X_1 & X_2
        \end{pmatrix}
        = 
        \Diag(L_1, L_2),
    \end{equation*}
    where $\begin{pmatrix}
        X_1 & X_2
    \end{pmatrix}$ is unitary with $X_1 \in \Cbb^{n\times k}$. Let $Z \in \Cbb^{n\times k}$, and $M\in \Cbb^{k\times k}$ be Hermitian, and
    \begin{equation*}
        R = A Z - Z M.
    \end{equation*}
    Suppose that 
    \begin{equation*}
        \mathcal L (M) \subset [\alpha, \beta]
    \end{equation*}
    and that for some $\delta > 0$
    \begin{equation*}
        \mathcal L (L_2) \subset \mathbb{R} \backslash [\alpha-\delta, \beta + \delta].
    \end{equation*}
    Then for any unitarially invariant norm
    \begin{equation*}
        \norm{\sin \Theta[\Rcal(X_1), \Rcal(Z)]} \leq \frac{\norm{R}}{\delta \inf_2(Z)},
    \end{equation*}
    where $\inf_2(Z)$ is the smallest singular value of $Z$. 
\end{theorem}


==> Deprecated/4proof.tex <==
\section{Proofs}
\label{sec:proofs}
In this section, we will prove that as $K$ and $T$ increase, the frequencies of the filter polynomial solutions of \eqref{eq:LeastSquares} applied to islands go to the frequencies appearing in \eqref{eq:a-island}, i.e.
\begin{equation*}
    \omega_{m\nbf} = \frac{\nbf \cdot \omega + m}{p}, \qquad \nbf \neq 0, \qquad 0 \leq m < p.
\end{equation*}
With this notation, the sequence $\ubf_t$ on islands can be written as a Fourier series
\begin{equation*}
    \ubf_t = \sum_{m = 0}^{p-1} \sum_{\nbf\in\Zbb^d} \dobsT_{m\nbf} \lambda_{m\nbf}^t, \qquad \lambda_{m\nbf} = e^{2\pi i \omega_{m\nbf}},
\end{equation*}
where $g_{00}=0$. 

It is convenient to be able to transform between the above multi-index $(m,\nbf) \in [p] \times \Zbb^d $ and a linear ordering of the frequencies over $n \in \Zbb$. Let $\Pi : n \mapsto (m,\nbf)$ be the bijective indexing over the integers and $\Pi_{\nbf} : n\mapsto \nbf$ be the projected ordering onto $\nbf$. We require two things of the bijection:
\begin{enumerate}
    \item Conjugacy symmetry $\lambda_{\Pi(n)} = \overline{\lambda}_{\Pi(-n)}$, and
    \item Monotonicity in $\nbf$: $\norm{\Pi_{\nbf}(n)}_{\infty} \leq \norm{\Pi_{\nbf}(n')}_{\infty}$ for $\abs{n} < \abs{n'}$. 
\end{enumerate}
Otherwise, the ordering is arbitrarily fixed (say, lexicographically). 
Note that the conjugacy symmetry implies that $\Pi(0) = (0,0)$. 
Using the 1D ordering, we use the abbreviated notation
\begin{equation*}
    \omega_n = \omega_{\Pi(n)}, \quad \lambda_n = \lambda_{\Pi(n)}, \quad \dobsT_n = \dobsT_{\Pi(n)}, \quad \text{etc.}
\end{equation*}

The monotonicity condition is important for translating the convergence of multi-indices to convergence in the single index. 
In particular, the ordering tells us that
\begin{equation*}
    \norm{\Pi_{\nbf}(n)}_\infty = \begin{cases}
        0 & \abs{n} = 0, \\
        1 & 0 < \abs{n} \leq \frac{3^d-1}{2}, \\
        \vdots & \vdots \\
        m & \frac{(2m-1)^d - 1}{2} < n \leq \frac{(2m+1)^d-1}{2}, \\
        \vdots & \vdots
    \end{cases}
\end{equation*}
In this way, $\norm{\Pi_{\nbf}(n)}_{\infty} \sim c_{\infty} n^{1/d} $ for some constant $c_\infty > 0$. Using the infinity norm, there are equivalent bounds for any other norm on $\Pi_{\nbf}(n)$, which we use for rates of convergence of Fourier series in the $2$-norm.

To motivate the steps in the following sections, we first consider the problem of polynomial perturbation alone.
Let $\halffilter = P^T \filter$ be a palindromic filter with a root at $\lambda_n$ for some $n$. 
Evaluation of the associated polynomial is a linear function of the coefficients
\begin{equation*}
    q_K(\lambda_n) = \lambda_n^K \bm \phi_n^T \halffilter = 0,
\end{equation*}
where
\begin{equation*}
    \bm \phi_n = \bm \phi_{m\nbf} = \begin{pmatrix}
        1 \\ \sqrt{2} \cos(2\pi \omega_n) \\ \vdots \\ \sqrt{2} \cos(2 \pi K \omega_n)
    \end{pmatrix} = P \begin{pmatrix}
        \lambda_n^{-K} \\ \vdots \\ \lambda_n^{-1} \\ 1 \\ \lambda_n \\ \vdots \\ \lambda_n^K
    \end{pmatrix}.
\end{equation*}
Now, we consider how the root $\lambda_n$ is perturbed when we perturb $\halffilter$ by an amount $\delta \halffilter$. 
Letting the perturbation of $\lambda_n$ be $\delta \lambda_n$, a direct application of chain rule finds
\begin{equation}
\label{eq:eval-perturbation}
    \delta \lambda_n = -\frac{\bm \phi_n^T \delta \halffilter}{\pd{\lambda_n^K \bm \phi_n^T}{\lambda_n} \halffilter} = - \frac{\delta q_K(\lambda_n)}{q_K'(\lambda_n)},
\end{equation}
where $\delta q_K$ is the polynomial with coefficients $\delta \halffilter$. So, if we want to show that a root is not strongly perturbed, we have two simultaneous goals:
\begin{enumerate}
    \item We must bound $\bm \phi_n^T \delta \halffilter$ so that it is small, and
    \item We must bound $q_K'(\lambda_n)$ away from zero.
\end{enumerate}
We note that we do not have to specifically bound $\delta \halffilter$ so that it is small. Rather, we must make sure the perturbation is only large in a direction orthogonal to the vector $\bm \phi_n$.

In order to find the perturbation $\delta \halffilter$, we perturb the least squares problem \eqref{eq:LeastSquares}. Solving the system with $\halffilter = \halffilter_0 + \delta \halffilter$ under the assumption that $\bm \phi_0^T \halffilter_0 = 1$ and $\bm \phi_n^T \halffilter_0 = 0$, we find
\begin{equation*}
    \delta \halffilter = - \halffilter_0 + \frac{(\tilde A + \epsilon \Whalf)^{-1}\bm \phi_0}{\bm \phi_0^T (\tilde A + \epsilon \Whalf)^{-1}\bm \phi_0}.
\end{equation*}
Substituting this into the eigenvalue perturbation formula \eqref{eq:eval-perturbation}, we find that
\begin{equation*}
    \delta \lambda_n = - \frac{1}{q'_K(\lambda_n)} \frac{\bm \phi_n^T (\tilde A + \epsilon \Whalf)^{-1}\bm \phi_0}{\bm \phi_0^T (\tilde A + \epsilon \Whalf)^{-1}\bm \phi_0}.
\end{equation*}



The key insight of the proof is showing that the modes $\bm \phi_n$ are nearly orthogonal under the inner product defined by $W_K$. 
That is, if we let $\dbf = \Whalf^{-1/2} \halffilter$ and $\tilde{B} = \Whalf^{1/2} \tilde{A} \Whalf^{1/2}$, we have the new least-squares problem
\begin{equation}
\label{eq:transformedleastsquares}
    \min_{\dbf} \dbf^T (\tilde{B} + \epsilon I) \dbf, \qquad \text{s.t. } \bm \psi_0^T \dbf = 1,
\end{equation}
where $\bm \psi_n = \Whalf^{1/2} \bm \phi_n$ and we have used the identity $\bm \psi_0 = \Whalf^{1/2} P \bm{1}$ for the constraint. 
In this new basis, polynomial evaluation is equivalent to evaluating $\bm \phi_n^T \halffilter = \bm \psi_n^T \dbf$. 
Additionally, the eigenvalue perturbation becomes
\begin{equation}
\label{eq:lambda-perturbation}
    \delta \lambda_n = - \frac{1}{q'_K(\lambda_n)} \frac{\bm \psi_n^T (\tilde B + \epsilon I)^{-1}\bm \psi_0}{\bm \psi_0^T (\tilde B + \epsilon I)^{-1}\bm \psi_0}
\end{equation}
In the following sections, we show the matrix $\tilde B$ is approximately diagonalized in the basis of $\bm \psi_n$, implying the right term in the above formula is small. 

We start in Sec.~\ref{subsec:41} where we show that as $T$ grows, the normal matrix approaches a normal matrix from the continuous problem. Then, we show that as $K$ grows, errors associated with the decay of Fourier coefficients of $\dobsT$ (Sec.~\ref{subsec:42}) and the orthogonality of the modes $\bm \psi_n$ (Sec.~\ref{subsec:43}) also decay sufficiently fast. These matrix perturbation bounds are then combined in Sec.~\ref{subsec:44} to obtain Thm.~\ref{thm:SVD}, a subspace perturbation theorem for the normal matrix. 
Finally, the results are combined in the proof of Thm.~\ref{thm:least-squares}, given in Sec.~\ref{subsec:46}.


\subsection{Choosing $T$ via Birkhoff average convergence}
\label{subsec:41}

This section links the finite-time least square problem
\eqref{eq:LeastSquares} 
to the invariant measure least squares problem 
\eqref{eq:FKg}. 
In particular, the finite time normal matrix is
\begin{equation*}
    \tilde{A} = P U^T W_T U P^T, 
\end{equation*}
where 
\begin{equation*}
    (U^T W_T U)_{mn} = \WBA_T[(\dobs\circ\sympmap^m)\cdot(\dobs\circ\sympmap^n)](\xbf_0)
\end{equation*}
and we assume that $\xbf_0$ is in an island. We will compare the error of $\tilde{A}$ when compared against the infinite-time normal matrix defined as
\begin{equation*}
    E_{TA} = \tilde{A} - A, \qquad A = P A_{\infty} P^T,
\end{equation*}
where
\begin{equation*}
    (A_{\infty})_{mn} = \BA[(\dobs\circ\sympmap^m)\cdot(\dobs\circ\sympmap^n)](\xbf_0).
\end{equation*}
When expanded in Fourier series, the matrix $A$ becomes
\begin{equation*}
    A = \sum_{n =1}^\infty 2 \abs{\dobsT_n}^2 \bm \phi_n \bm \phi_n^T.
\end{equation*}


The term $E_{TA}$ is the error introduced by the Birkhoff average used to find the elements of $A$, and depends on the value of $T$ and the initial point on the orbit $\xbf_0$. Specifically, the error has the form
\begin{align}
\label{eq:Ecoef}
    E_{TA} = P (U^T W_T U - A_\infty) P^T,
\end{align}
where
\begin{multline*}
     (U^T W_T U - A_\infty)_{mn} = \WBA_T[(\dobs\circ\sympmap^m)\cdot (\dobs\circ\sympmap^n)](\xbf_0) \\- \BA[(\dobs\circ\sympmap^m)\cdot(\dobs\circ\sympmap^n)](\xbf_0).
\end{multline*}
We can bound $E_{TA}$ in Frobenius norm as:
\begin{lemma}
\label{lemma:ET_entrywise}
    Under Hypotheses \ref{setting} (H1-2), there exists a constant $C_{T,M_T}$ independent of $k$ and $\ell$ such that
    \begin{equation}
    \label{eq:ET_entrywise}
        \abs{E_{TA, k\ell}} \leq C_{T,M_T} T^{-M_T},
    \end{equation}
    provided that $M > d + \nu M_T$.
\end{lemma}
\begin{proof}
    The weighted Birkhoff average in \eqref{eq:Ecoef} is expanded as 
    \begin{equation*}
        (U^T W_T U)_{mn} = \sum_{t = 0}^{T-1} w_{t,T} \ubf_{m+t} \cdot \ubf_{n+t},
    \end{equation*}
    where the signal $\ubf_{m+t}\cdot \ubf_{n+t}$ can be written in terms of the Fourier series as
    \begin{equation*}
        \ubf_{m+t}\cdot \ubf_{n+t} = \sum_{k, \ell\in\Zbb}\dobsT_k \cdot \dobsT_\ell \lambda_k^{m+t} \lambda_\ell^{n+t} = \sum_{k\in\Zbb} U_{k,m,n}\lambda_k^t.
    \end{equation*}
    Using the convolutional structure of the second equality above, one can show that $U_{k,m,n}\leq C_{U,M} k^{-M}$ where $C_{U,M}$ is independent of $m$ and $n$. The proof of Thm.~\ref{thm:Das2018} only depends on the decay rates of these coefficients, so Thm.~\ref{thm:Das2018} implies the bound \eqref{eq:ET_entrywise} independent of $m$ and $n$.
    
    % \mr{The below is slightly wrong and for the invariant circle case, because of the sum not including $m=0,n$. However, none of this is really interesting anyway. In the end, I think we should remove all of this.
    
    % We can write the Fourier series of $\dobsT(\cdot) \dobsT(\cdot + \bm \phi)$ as a convolution:
    % \begin{equation*}
    %     \dobsT(\theta)^T \dobsT(\theta + \bm \phi) = \sum_{n \in \Zbb} \left[\sum_{m \in \Zbb} e^{2\pi i m \bm \phi} \dobsT_{m}^T \dobsT_n \right] e^{2\pi i n \theta} = \sum_{n\in\Zbb} \tilde{g}_n e^{2\pi i n \theta}.
    % \end{equation*}
    % Because $\dobsT \in C^{M}$, we have a coefficient $C_{g,M}$ such that $\abs{\dobsT_n} < C_{g,M} \abs{n}^{-M}$. Using this, we can bound $\tilde{g}_{n}$ as
    % \begin{equation*}f
    %     \abs{\tilde{g}_n} \leq C_{g,M}^2 \sum_{m\in\Zbb \backslash \{0, n\}} \abs{m}^{-M} \abs{n-m}^{-M} = C_{g,M}^2 \sum_{m \in \Zbb \backslash \{0, n\} } \abs{m(n-m)}^{-M}.
    % \end{equation*}
    % We can bound the above sum by integrals for $n>2$:
    % \begin{align*}
    %     \abs{\tilde{g}_n} &< 2 C^2_{g,M} \left[2 (n-1)^{-M} + \int_{1}^{n/2} (x(n-x))^{-M} \dif x + \int_{1}^\infty (x(x+n))^{-M} \dif x   \right] ,\\
    %     &< 4 C^2_{g,M}\left[2 (n-1)^{-M} + \left((2^{M})+1\right)n^{-M} \int_{1}^{\infty} x^{-M} \dif x \right],\\
    %     &< C_{\tilde{g},M}n^{-M}.
    % \end{align*}}
\end{proof}
\begin{remark}
    Here and throughout this paper, constants suppress information about $\dobsT$, $\omega$, and the bump function $w$. They never suppress information on system size.
\end{remark}

From here, we consider the perturbation in the weighted least squares problem \eqref{eq:transformedleastsquares}:
\begin{equation*}
    \tilde{B} = B + E_T, 
\end{equation*}
where
\begin{equation*}
    E_T = \Whalf^{1/2} E_{TA} \Whalf^{1/2}, 
\end{equation*}
and
\begin{equation*}
    B = \Whalf^{1/2} A \Whalf^{1/2} = \sum_{n=1}^\infty 2 \abs{\dobsT_n}^2 \bm \psi_n \bm \psi_n^T.
\end{equation*}
The perturbation of $B$ can be bounded in Frobenius norm using our previous result:
\begin{lemma}
\label{lemma:ET}
    Under the same conditions as Lemma \ref{lemma:ET_entrywise}, we have
    \begin{equation*}
        \norm{E_T}_F \leq C_{T,M_T} T^{-M_T}.
    \end{equation*}
\end{lemma}
\begin{proof}
    Directly calculating the norm:
    \begin{align*}
        \norm{E_T}^2_F &= \norm{\Whalf^{1/2} E_{TA} \Whalf^{1/2}}^2_F, \\
        &= \sum_{k, \ell = 0}^{K} E_{TA,k\ell}(\Whalf)_{kk}(\Whalf)_{ll}, \\
        & \leq C_{T,M_T}^2 T^{-2M_T}\sum_{k, \ell = 0}^{2K} \tilde{w}_{k,K} \tilde{w}_{\ell,K}, \\
        &= C_{T,M_T}^2 T^{-2M_T}.
    \end{align*}
\end{proof}



\subsection{Bounding the tail error}
\label{subsec:42}
From here, we are interested in showing that the perturbation of $B$ with respect to the rank $N \leq K$ subspace
\begin{equation*}
    E_B = B - \Psi \Sigma^2 \Psi^T
\end{equation*}
is small in some norm, where 
\begin{equation*}
    \Psi = \begin{pmatrix}
        \bm \psi_1 & \dots & \bm \psi_N
    \end{pmatrix}, \qquad \Sigma^2 = \begin{pmatrix}
        \sigma_1^2 \\ 
         & \ddots \\
         &  & \sigma_N^2
    \end{pmatrix},
\end{equation*}
and
\begin{equation*}
    \sigma_j^2 = 2\abs{\dobsT_j}^2.
\end{equation*}
A bound on $E_B$ shows that if $N$ is large enough, the linearly independent modes in $\Psi$ capture most of the Fourier content of $\dobsT$. 

\begin{lemma}
\label{lemma:EB}
    If $\dobsT \in C^{M}$ with Fourier coefficient bounds $\abs{\dobsT_{m\nbf}} \leq C_{g,M} \norm{\nbf}^{-M}$, we have for some constant $C_B$
    \begin{equation*}
        \norm{E_B}_F < C_{B} N^{-2M/d+1}
    \end{equation*}
\end{lemma}
\begin{proof}
    By the triangle inequality,
    \begin{equation*}
        \norm{E_B}_F \leq \sum_{n > N} 2 \abs{\dobsT_n}^2 \norm{\bm \psi_n\bm \psi_n^T}_F = \sum_{n > N} 2 \abs{\dobsT_n}^2 \norm{\bm \psi_n}_2^2.
    \end{equation*}
    Looking at the $\norm{\bm \psi_n}_2^2$ term, we have
    \begin{equation}
    \label{eq:psi_norm}
        \norm{\bm \psi_n}^2_2 = \frac{\sum_{k = -K}^K \WBAw(k / (K+1)) \cos^2(2\pi k \omega_n)}{\sum_{k=-K}^K \WBAw(k/(K+1))} < 1.
    \end{equation}
    For the sum over $\abs{\dobsT_n}^2$, we note that the multi-indexing monotonicity condition gives the bound 
    \begin{align*}
        \norm{\dobsT_n}^2 &= \norm{\dobsT_{\Pi(n)}}^2, \\
        &\leq C_{g,M} \norm{\Pi(n)}^{-2M}, \\
        &\leq C_{2} n^{-2M/d}.
    \end{align*}
    Using this, we find
    \begin{align}
    \nonumber
        \sum_{n > N} \abs{\dobsT_n}^2 &< \int_{N}^\infty C_{g,M}^2 x^{-2M/d} \dif x, \\
    \nonumber
        &= C_{g,M}^2 \left[ \frac{x^{-2M/d+1} d}{-2M+d} \right]_{N}^{\infty}, \\
    \label{eq:g_tail_energy}
        &= \frac{dC_{g,M}^2}{2M-d} N^{-2M/d+1}.
    \end{align}
    Combining \eqref{eq:psi_norm} and \eqref{eq:g_tail_energy} and letting $C_B = \frac{dC_{g,M}^2}{2M-d}$, we have our result.
\end{proof}

\subsection{Error of approximate orthogonalization}
\label{subsec:43}

In this section, we show that as $K$ grows, $\Psi$ approaches orthonormality. First, we bound the error of individual inner products $\ip{\bm \psi_n}{\bm \psi_m}$ for $0 \leq n,m \leq N$ away from the Kronecker delta $\delta_{nm}$. One can view this as a statement about aliasing for our specific set of frequencies. Then, we use this to bound the difference of $B$ from a orthonormal matrix. For the first step, we first need the following lemma:
\begin{lemma}[Poisson summation formula] 
\label{lemma:PoissonSummation}
For each $f \in L^2(\Rbb)$,
\begin{equation*}
    \sum_{n\in\Zbb} f(n) = \sum_{n\in\Zbb} \int_{\Rbb}f(x) e^{-2\pi i n x} \dif x.
\end{equation*}
\end{lemma}

We start with a helper lemma:
\begin{lemma}
\label{lemma:lambda-orthogonality}
    Under Hypotheses \ref{setting} H1 and H2, for all $\Mperp \in \Nbb$ there are constants $C_{\lambda, \Mperp} > 0$ independent of $n$ such that
    \begin{equation*}
        \abs{S_{m\nbf} - \delta_{(m,\nbf),0}} < C_{\lambda, \Mperp} \norm{\nbf}^{\Mperp \nu} K^{-\Mperp},
    \end{equation*}
    where 
    \begin{equation*}
        S_{m\nbf} = \sum_{t=0}^{T-1} \WBAw_{t,T} \lambda_{m\nbf}^t, \quad \delta_{(m,\nbf),0} = \begin{cases}
            1 & m = 0 \text{ and } \nbf = 0, \\
            0 & \text{else}.
        \end{cases}
    \end{equation*}
\end{lemma}
\begin{proof}
    Applying the Poisson summation formula, we have
    \begin{align*}
        S_{m\nbf} &= \frac{1}{A_K}\sum_{t \in \Zbb} \int_{\Rbb} \WBAw\left(\frac{x}{K+1}\right) e^{2\pi i (\omega_{m\nbf}-t) x}\dif x,\\
        &= \frac{K+1}{A_K} \sum_{t\in\Zbb} \int_{-1}^1 \WBAw(x) e^{2\pi i  (K+1) (\omega_{m\nbf} - t) x} \dif x,
    \end{align*}
    where
    \begin{equation*}
        A_K = \sum_{t=0}^{T-1} w\left(\frac{t+1}{T+1} \right).
    \end{equation*}
    The factor $A_K$ scales as $K$, so for some constant $C_W$ we have $(K+1)/A_K < C_{W}$.

    From here, we can perform repeated integration by parts against $\WBAw$. Doing so, we have that
    \begin{align*}
        &\abs{\int_{-1}^1 \WBAw(x) e^{2\pi i  (K+1) (\omega_{m\nbf} - t) x} \dif x}\\
        &\qquad= (K+1)^{-\Mperp} \abs{2 \pi (\omega_{m\nbf} - t)}^{-\Mperp}\\
        &\quad \qquad \times \abs{\int_{-1}^1 \WBAw^{(\Mperp)}(x) e^{2\pi i  (K+1) (\omega_{m\nbf} - t) x} \dif x}, \\
        &\qquad \leq K^{-\Mperp} \abs{2\pi (\omega_{m\nbf} - t)}^{-\Mperp} \norm{\WBAw^{(\Mperp)}}_{L^1}.
    \end{align*}
    Going back to $S_{m\nbf}$, we have
    \begin{equation*}
        \abs{S_{m\nbf}} \leq  C_W \norm{\WBAw^{(\Mperp)}}_{L^1} K^{-\Mperp} \sum_{n \in \Zbb} \abs{2 \pi (\omega_{m\nbf} - t)}^{-\Mperp}.
    \end{equation*}
    To bound the sum, let $t_0$ be the closest integer to $m\omega$. Then,
    \begin{multline*}
        \sum_{t \in \Zbb} \abs{2 \pi (\omega_{m\nbf} - t)}^{-\Mperp} = \abs{2 \pi (\omega_{m\nbf} - t_0)} \\
        + \sum_{t \in \Zbb\backslash\{t_0\}} \abs{2 \pi (\omega_{m\nbf} - t)}^{-\Mperp}.
    \end{multline*}
    The term on the first line is bounded by an $O(\norm{\nbf}^{\Mperp(1+\nu)})$ Diophantine condition, while the rest of the sum is bounded by a constant. The Diophantine bound dominates, giving $\sum_t \abs{\omega_{m\nbf} - t}^{-\Mperp} \leq C_{\omega, \Mperp} \norm{\nbf}^{\Mperp(1+\nu)}$. Using this, we have our result.
    
\end{proof}


The above lemma serves as a numerical linear algebra reinterpretation of the results of the weighted Birkhoff average \cite{Das2018}. 
We note that it can easily be used to prove Thm.~\ref{thm:Das2018}:
\begin{proof}[Proof of Thm.~\ref{thm:Das2018}]
    Assuming a $C^M$ island chain, the signal can be written as 
    \begin{equation*}
        (\obs \circ \sympmap^t)(\xbf_0) = \sum_{m=0}^{p-1} \sum_{\nbf \in \Zbb^d }\obsT_{m\nbf} \lambda_{m\nbf}^t,
    \end{equation*}
    where $\abs{\obsT_{m\nbf}} < C \norm{\nbf}^{-M}$. Then, the average can be written as
    \begin{align*}
        \WBA_T[\obs](\xbf_0) &= \sum_{m=0}^{p-1} \sum_{\nbf \in \Zbb^d }\obsT_{m\nbf} \sum_{t=0}^{T-1}w_{t,T} \lambda_{m\nbf}^t,\\
        &= \sum_{m=0}^{p-1} \sum_{\nbf \in \Zbb^d }\obsT_{m\nbf} S_{m\nbf}.
    \end{align*}
    Applying Lemma \ref{lemma:lambda-orthogonality}, we find
    \begin{equation*}
        \abs{\WBA_T[\obs](\xbf_0) - \obsT_0} < p C_{\lambda,m} \sum_{n=1}^{\infty} \norm{\nbf}^{-M+m\nu}.
    \end{equation*}
    Using the condition that $M > d + m\nu$, we know the above sum converges, giving the result.
\end{proof}

Returning to the proof of the RRE root convergence, we can also look at the orthogonality of the $\bm \psi_m$ modes:
\begin{lemma}
\label{lemma:orthogonality}
    Under Hypotheses \ref{setting} (H1-2), for all $\Mperp \in \Nbb$ the basis vectors $\bm \psi_n$ and $\bm \psi_m$ are nearly orthonormal with constants $C_{\psi, \Mperp} > 0$ independent of $n$ and $m$ as
    \begin{equation*}
        \abs{\bm \psi_n^T \bm \psi_m - \delta_{nm}} < C_{\psi, \Mperp} (m+n)^{\Mperp \nu / d} K^{-\Mperp}
    \end{equation*}
\end{lemma}
\begin{proof}
    We can write
    \begin{align*}
        \bm \psi_n^T \bm \psi_m &= \sum_{k = -K}^K \tilde{w}_{k+K, K} \cos(2\pi k \omega_n)\cos(2 \pi k \omega_m),\\
        &= \frac{1}{4} (S_{n+m} + S_{n-m} + S_{m-n} + S_{-m-n}),
    \end{align*}
    where
    \begin{equation*}
        S_n = S_{\Pi(n)}. 
    \end{equation*}
    The result follows directly from Lemma \ref{lemma:lambda-orthogonality} and the ordering of $\Pi$. 
\end{proof}


We aim to turn the result in Lemma \ref{lemma:orthogonality} into an error term for the normal matrix from a known singular value decomposition. Specifically, we consider the singular value decomposition of $\Psi$:
\begin{equation*}
    \Psi = U (I + \Delta) V^T,
\end{equation*}
where $\Delta$ measures the separation of $\Psi$ from orthogonality.
Using this decomposition, we can represent the normal matrix as
\begin{equation}
\label{eq:FullPerturbation}
    \tilde{B} = Q \Sigma^2 Q^T + E_{\Delta} + E_B + E_T,
\end{equation}
where $Q = U V^T$ and
\begin{equation*}
    E_\Delta = (\Psi-Q)\Sigma^2 Q^T + Q \Sigma^2(\Psi-Q)^T + (\Psi-Q)\Sigma^2(\Psi-Q)^T.
\end{equation*}
We recognize $Q \Sigma^2 Q^T$ as an approximate eigenvalue decomposition of $\tilde{B}$, which is the subject of the Sec.~\ref{subsec:44}. However, first we must bound the error introduced via $E_{\Delta}$:
\begin{lemma}
\label{lemma:EDelta}
    Under the conditions of Lemma \ref{lemma:orthogonality}, there exists a constant $C_\Psi$ such that if
    \begin{equation*}
        \Delta_{\max} = C_\Psi K^{-\Mperp} N^{1+\Mperp\nu/d} < 1,
    \end{equation*}
    the matrix $\Psi$ is full rank with singular values $1+\Delta_{m}$ satisfying $-\Delta_{\max} < \Delta_{m} < \Delta_{\max}$.
    Additionally, the normal matrix error term is bounded as
    \begin{equation*}
        \norm{E_\Delta}_2 < C_{\Delta} K^{-\Mperp} N^{1+\Mperp\nu/d}.
    \end{equation*}
\end{lemma}
\begin{proof}
    In order to bound $E_\Delta$, it is easiest to bound $\norm{\Delta}_2 = \norm{\Psi - Q}_2$. Then, the bound for the full norm is a straightforward application of the triangle inequality. 
    
    The bounds for $\Delta$ are obtained by through the singular values of $\Psi$, which are defined as the square roots of the eigenvalues of $\Psi^T \Psi$. We can bound the eigenvalues of $\Psi^T \Psi$ by a Gershgorin argument using bounds on the entries from Lemma \ref{lemma:orthogonality}. We consider the Gershgorin circles for each row, all centered at $1$, defined as
    \begin{equation*}
        C_m = \left\{z\in\Cbb \mid \abs{z - 1} \leq5 R_m \right\}
    \end{equation*}
    with radii
    \begin{equation*}
        R_m = \sum_{n=0}^N\abs{(\Psi^T \Psi - I)_{mn}}.
    \end{equation*}
    By the Gershgorin theorem (Thm.~\ref{thm:gershgorin}), we know the squares of the singular values of $\Psi$ must lie within the largest of these circles.
    
    We can bound the radii as
    \begin{align}
    \nonumber
        R_m &= \sum_{n=0}^N \abs{\bm \psi_m^T \bm \psi_n -\delta_{mn}}, \\
    \nonumber
            &\leq C_{\bm \psi, \Mperp}K^{-\Mperp} \sum_{n=0}^N (N + n)^{\Mperp \nu/d}, \\
    \label{eq:GershgorinBound}
            &< C_\Psi K^{-\Mperp} N^{1+\Mperp\nu/d}.
    \end{align}
    So,
    \begin{align}
    \label{eq:DeltaBound}
        \abs{(1+\Delta_{m})^2-1} &= \abs{2\Delta_{m} + \Delta_{m}^2},\\
    \nonumber
        &< C_\Psi K^{-\Mperp} N^{1+\Mperp\nu/d}.
    \end{align}
    This bound gives the first part of the theorem, as $\abs{\Delta_{m}} < \abs{2\Delta_{m} + \Delta_{m}^2}$ when $\abs{\Delta_{m}} < 1$.
    Combining this with the fact that $\norm{U}_2 = \norm{V}_2 = 1$ and $\norm{\Sigma^2}_2 \leq \norm{\dobsT}^2_{L^2}$, we have the error term result.
\end{proof}

\subsection{Eigenvalue perturbation}
\label{subsec:44}
Now, we have enough information to directly apply symmetric eigenvalue and eigenvector perturbation theory to Eq.~\eqref{eq:FullPerturbation}. The proof has two steps. First, we show for eigenvalues separated by a gap, the perturbation from $E$ maintains that gap for large enough $K$. From here, we prove the angle of the eigenvector subspace is near that of the associated modes $\bm \psi_n$. At the end of the section, we specify the general invariant subspace theory to the most useful used in Birkhoff RRE as a corollary. 

Before we state the theorem, we first define the angle between subspaces
\begin{definition}[$\nu$-gap, from Stewart and Sun\cite{Stewart1990}]
\label{def:nu-gap}
    Let $\Xcal, \Ycal$ be the $N$-dimensional subspaces of $\Rbb^K$ with associated unitary matrices $X, Y \in \Rbb^{K, N}$. We define the $X$ projection operator as $P_X = X X^T$ and similarly $P_Y = Y Y^T$. For a given matrix norm $\nu$, we define the $\nu$-gap as
    \begin{equation*}
        \rho_{\nu}(\Xcal, \Ycal) = \nu(P_X - P_Y).
    \end{equation*}
    In particular, we define the following subspace angles:
    \begin{align*}
        \rho_2 &= \norm{\sin(\Theta[\Xcal, \Ycal])}_2 = \norm{P_X - P_Y}_2, \\
        \rho_F &= \sqrt{2} \norm{\sin(\Theta[\Xcal, \Ycal])}_F = \norm{P_X - P_Y}_F.
    \end{align*}
\end{definition}

Given this, the eigenvalue perturbation is as follows:
\begin{theorem}
\label{thm:SVD}
    Under Hypotheses \ref{setting}, let $0<\alpha<\beta$ and such that that there exists $L\geq 1$ singular values that $\sigma_n^s \in [\alpha,\beta]$. Additionally, suppose there is a gap $\delta$ such that $\sigma_n^2 \notin [\alpha-\delta,\alpha] \cup [\beta,\beta+\delta]$ for all $n$. 
    % be repeated singular value such that $s = \sigma_{n_1} = \sigma_{n_2} = \dots = \sigma_{n_L}$ for $L\geq 1$. Let the gap between $s$ and the next nearest singular value be 
    % \begin{equation*}
    %     \delta = \min_{n \notin \{n_l\}} \abs{\sigma_n^2 - s^2}.
    % \end{equation*}
    Then, under the condition that $\Delta_{\max} \leq 1/2$ (see Lemma \ref{lemma:EDelta}) and
    \begin{align}
    \nonumber
        \epsilon_B = &\ C_{T, M_T} T^{-M_T} + C_B N^{-2M/d+1} \\
    \nonumber
        &+  C_{\Delta} K^{-\Mperp} N^{1+\Mperp\nu/d}, \\
    \label{eq:spectrum-gap}
        < &\ \frac{\delta}{4},
    \end{align}
    the eigenvalues $\tilde{\sigma}_n^2$ of $\tilde{B}$ are bounded as
    \begin{equation*}
        \abs{\tilde{\sigma}_{n}^2 - \sigma_n^2} \leq \epsilon_B.
    \end{equation*}
    
    \mr{Is there a simple way to do this without indexing? I just cant figure it out...} Furthermore, let $n_\ell$ for $1\leq \ell \leq L$ index the singular values $\sigma_{n_\ell}^2 \in[\alpha,\beta]$. Then, the associated invariant subspace $X_1 = \begin{pmatrix} \xbf_{n_1} & \dots & \xbf_{n_{L}} \end{pmatrix}$ is close to the modes $\Psi_s = \begin{pmatrix} \bm \psi_{n_1} & \dots & \bm \psi_{n_{L}} \end{pmatrix}$ as
    \begin{multline}
    \label{eq:subspace-error}
        \norm{\sin (\Theta[\Rcal(X_1), \Rcal(\Psi_s)])}_F \leq C_{B\Psi} N^{-2M/d+1} \\ + C_{T\Psi}T^{-M_T} + C_{\Delta\Psi} K^{-\Mperp} N^{1+\Mperp\nu/d}.
    \end{multline}
\end{theorem}
\begin{proof}
    The proof for the eigenvalue bounds is a direct application of Weyl's theorem (see Thm.~\ref{thm:Weyl}). We note that $\epsilon$ gives a bound for the spectral radius of the perturbation, so $-\epsilon \leq \epsilon_n \leq \epsilon_1 \leq \epsilon$. A direct application combined with Lemmas \ref{lemma:ET}, \ref{lemma:EB}, and \ref{lemma:EDelta} then gives the eigenvalue result.
    
    For the subspace bound, we use Davis-Kahan $\sin(\Theta)$ theorem (Thm.~\ref{thm:DavisKahan}). To begin, we note that the eigenvalue perturbation theorem guarantees that there are exactly $L$ eigenvalues of $\tilde B$ in the region $[\alpha - \delta/4, \alpha + \delta/4]$. So, $\tilde{B}$ has a spectral resolution (eigenvalue decomposition)
    \begin{equation*}
        \begin{pmatrix}
            X_1^* \\ X_2^*
        \end{pmatrix} \tilde B \begin{pmatrix}
            X_1 & X_2
        \end{pmatrix} = \Diag(L_1, L_2),
    \end{equation*}
    where $L_1 \in \Rbb^{L \times L}$ and $X_1 \in \Rbb^{L \times K+1}$ are the eigenvalue-eigenvector pairs associated with the eigenvalues in $[\alpha-\delta/4, \alpha+\delta/4]$, and $(L_2, X_2)$ are the rest of the eigenvalues and eigenvectors, where $L_2\in \Rbb^{K+1-L \times K+1-L}$ has a spectrum in $\mathbb R \backslash [\alpha-\delta/4, \beta+3\delta/4]$.
    
    For the residual $R$ in Thm.~\ref{thm:DavisKahan}, we want to bound the distance to the subspace $Z = \Psi_s$. Let $M = \Sigma_s^2 \Diag(\sigma_{n_1}^2, \dots, \sigma_{n_L}^2)$. Then, the residual has the form
    \begin{align*}
        R &= \tilde B Z - Z M, \\
          &= (\Psi \Sigma^2 \Psi^T + E_B + E_T)\Psi_s - \Psi_s\Sigma_s^2.
    \end{align*}
    Now, let $P_s\in\Rbb^{N\times L}$ be the projection $P_{s,ij} = \delta_{in_j}$, so that $\Psi_s = \Psi P_s$ and $\Sigma_s^2 = P_s^T \Sigma^2 P_s$. We have
    % $\Psi_\perp$ include the modes of $\Psi$ not in $\Psi_s$ and $\Sigma_\perp^2$ be the associated submatrix of $\Sigma^2$. Then,
    % \begin{multline*}
    %     R = \Psi_s\Sigma_s^2 (\Psi_s^T \Psi_s - I) + \Psi_\perp \Sigma_\perp^2 \Psi_\perp^T \Psi_s + (E_B + E_T) \Psi_s.
    % \end{multline*}
    \begin{align*}
        R &= \Psi \Sigma^2 (\Psi^T\Psi-I)P_s + (E_B + E_T)\Psi P_s.
    \end{align*}
    To bound the above, we note that $\norm{\Sigma^2}_2 \leq \norm{\dobsT}_{L^2}^2$ and that Lemma \ref{lemma:EDelta} gives $1/2 \leq \norm{\Psi}_2\leq 3/2$. For the matrix $(\Psi^T \Psi - I)$ we can bound the $2$ norm by Eq.~\eqref{eq:DeltaBound}. So,
    \begin{multline*}
        \norm{R}_F \leq \frac{3 C_\Psi}{2} \norm{\dobsT}_2^2 K^{-\Mperp} N^{1+\Mperp\nu/d} \\+ \frac{3}{2}(C_{T, M_T} T^{-M_T} + C_B N^{-2M/d+1}).
    \end{multline*}
\end{proof}

The combination of three constants $T$, $N$, and $K$ can make using Thm.~\ref{thm:SVD} unwieldy. This can be remedied by choosing $N$ and $T$ to scale with $K$. In practice, we use $T = \gamma K$ for some $\gamma \geq 1$, so we can dramatically simplify this statement. 
\begin{corollary}
\label{corollary:SVD}
    Take the setting of Thm.~\ref{thm:SVD}. Let $K = \gamma T$ with $\gamma > 0$ and $N = K^{\alpha_*}$ where
    \begin{equation*}
        \alpha_* = \frac{d}{2M/\Mperp +\nu}.
    \end{equation*} 
    Then, there exists a $K_* > 0$ such that for all $K>K_*$ \eqref{eq:spectrum-gap} is satisfied, the subspace in $X_1$ in Thm.~\ref{thm:SVD} is well defined, and the subspace distance is bounded as
    \begin{equation}
    \label{eq:nice-subspace-bound}
        \norm{\sin \Theta[\Rcal(X_1), \Rcal(\Psi)]} \leq C_* K^{-M_*},
    \end{equation}
    where 
    \begin{equation*}
    % \label{eq:Mstar}
        M_* = \min\left(\frac{2M - d}{2M/\Mperp + \nu} , \ M_T \right).
    \end{equation*}
    Moreover, for the same $N$ scaling, we have the bounds
    \begin{equation*}
        \norm{\Psi^T \Psi - I}_2 < C_{\Psi} K^{-M_*}, \qquad \norm{\Psi^T \bm \psi_0}_2 < C_{\psi_0} K^{-M_*}.
    \end{equation*}
\end{corollary}
\begin{proof}
    To obtain the value of $M$, we consider $N$ to scale as $K^\alpha$ for a to-be-determined value of $\alpha$. In this case, the subspace error term \eqref{eq:subspace-error} is
    \begin{multline*}
        \norm{\sin (\Theta[\Rcal(X_1), \Rcal(\Psi_s)])}_F \leq C_{B\Psi} K^{\alpha(-2M/d+1)} \\ + C_{T\Psi}\gamma^{-M_T}K^{-M_T} + C_{\Delta\Psi} K^{-\Mperp+\alpha(1+\Mperp\nu/d)}.
    \end{multline*}
    So, the dominant error will be $\mathcal O(K^{-M_*})$, where
    \begin{equation*}
        M_* = \min\left(\frac{\alpha(2M-d)}{d}, \ M_T, \ \frac{d \Mperp - \alpha(d+\Mperp \nu)}{d}\right).
    \end{equation*}
    We choose the value of $\alpha$ to balance the first and third arguments. Doing so, we find
    \begin{equation*}
        \alpha = \frac{d}{2M/\Mperp +\nu}.
    \end{equation*}
    Substituting this value of $\alpha$ into $M_*$, we find our result.

    The bound on $\Psi^T \Psi - I$ comes from substituting $N$ into \eqref{eq:GershgorinBound}. For the bound on $\Psi^T \bm \psi_0$, we use Lemma \ref{lemma:orthogonality}
    \begin{align*}
        \norm{\Psi^T \bm \psi_0}_2^2 &= \sum_{n=1}^N (\bm \psi_n^T\bm \psi_0)^2, \\
        &\leq C_{\psi,M_\perp}N^{1+2M\perp \nu/d}K^{-2M_\perp}.
    \end{align*}
    Substituting $N$ into this expression gives the result.
\end{proof}
\begin{remark}
    Because $\Mperp$ is arbitrary, the value of $M_*$ can approach arbitrarily close to
    \begin{equation*}
        M_* = \min\left(\frac{2M - d}{\nu} , \ M_T \right).
    \end{equation*}
    \mr{I think that $M_T$ might basically always than $(2M-d)/\nu$. We can choose $M_T = \floor{(M-d)/\nu} = \floor{(2M-d)/\nu - M/\nu}$. So, if $M/\nu > 1$, then $M_T$ is surely the dominant rate. }
\end{remark}



\subsection{The Least-Squares Problem}
\label{subsec:46}
We are now able to prove Thm.~\ref{thm:least-squares}:
\begin{proof}[Proof of Thm.~\ref{thm:least-squares}]
    We begin by fixing an $n$ such that $\abs{\dobsT_n} \neq 0$. We will perturb about the degree two $\halffilter$ that is orthogonal to $\bm \phi_n$, i.e.
    \begin{equation*}
        \halffilter = \frac{1}{1-\cos(2\pi \omega_n)} \begin{pmatrix}
            -\cos(2\pi \omega_n) \\ 2^{-1/2} \\ 0 \\ \vdots \\ 0
        \end{pmatrix}.
    \end{equation*}
    Because we treat $n$ as fixed, the derivative of the characteristic polynomial $q_K'(\lambda_n)$ is fixed.

    
    % The proof has three major steps:
    % \begin{enumerate}
    %     \item We show that the residual of the least squares problem is not too large when a polynomial of the form \eqref{eq:refpoly} is used as an ansatz.
    %     \item We use the matrix perturbation developed in the previous sections to show that the error correction from that polynomial is small in the direction of evaluating $\lambda_n$.
    %     \item We apply polynomial perturbation theory to show that the root cannot move too much.
    % \end{enumerate}

    % \mr{Move this somewhere? ::: and a weighting function $w$ s.t. $W_s > w(x) > w_s$ for $s/2 \leq x \leq 1-s/2$ and $0 < s < 1$}

    % \mr{Be careful with cbf tilde} We start by fixing a value of $\alpha < 1/4$ and by assuming $\omega$ satisfies the condition in Lemma \ref{lemma:DenominatorDistribution}. Then,
    % using Lemma \ref{lemma:DenominatorDistribution}, we choose $\tilde M$ such that $m\geq \tilde M$ implies the continued fraction denominator obeys $\alpha^{-1} K^\eta \leq L_m \leq s K$ where $\eta < 1$. Choosing the associated polynomial $q_{\alpha, \omega, m, p}$, we know the associated vector of coefficients $\halffilter_K$ will be padded by greater than $s K$ zeros. Then, letting $\tilde{\dbf}_K = \Whalf^{-1/2} \halffilter_K$ and using Lemma \ref{lemma:refpolybound}, we have
    % \begin{equation*}
    %     \norm{\tilde{\dbf}_K} \leq \norm{\Whalf^{-1/2}}_2 \norm{\tilde{\filter}_K} \leq w_s^{-1/2} C_\alpha.
    % \end{equation*}

    % We expect the solution to \eqref{eq:transformedleastsquares} to be nearby $\tilde{\dbf}_K$ in certain directions. To see this, we can write the solution to the least squares problem via
    % \begin{equation*}
    %     \begin{pmatrix}
    %         \tilde B + \epsilon I & \bm \psi_0 \\ \bm \psi_0^T & 0 
    %     \end{pmatrix}
    %     \begin{pmatrix}
    %         \dbf_K \\ \mu
    %     \end{pmatrix}
    %     =
    %     \begin{pmatrix}
    %         0 \\ 1
    %     \end{pmatrix}
    % \end{equation*}
    % where $\mu$ is a Lagrange multiplier for the constraint. If we choose $\dbf_K = \tilde{\dbf}_K + \delta \dbf_K$, we find the new system
    % \begin{equation}
    % \label{eq:Deltadsystem}
    %     \begin{pmatrix}
    %         \tilde B + \epsilon I & \bm \psi_0 \\ \bm \psi_0^T & 0 
    %     \end{pmatrix}
    %     \begin{pmatrix}
    %         \delta \dbf_K \\ \mu
    %     \end{pmatrix}
    %     =
    %     \begin{pmatrix}
    %         -(\tilde B + \epsilon I)\tilde{\dbf}_K \\ 1 - \bm \psi_0^T \tilde{\dbf}_K.
    %     \end{pmatrix}
    % \end{equation}
    % By construction, we have $\bm \psi_0^T \tilde{\dbf}_K = q_{\alpha, \omega, m, p}(1) = 1$, so the constraint is satisfied. Similarly, for $1 \leq \abs{n} < K^\eta$, we have $\bm \psi_n^T \tilde \dbf_K = q_{\alpha, \omega, m, p}(\lambda_n) = 0$. So, looking at $\tilde{B}$ applied to $\tilde{\dbf}$, we have
    % \begin{align*}
    %     \norm{\tilde{B} \tilde{\dbf}} &\leq \norm{\sum_{n = 1}^{\infty} 2 \abs{\dobsT_n}^2 \bm \psi_n \bm \psi_n^T \tilde{\dbf}} + \norm{E_T}_F \norm{\dbf}, \\
    %     &\leq w_s^{-1/2} C_\alpha \left(\sum_{n > K^{\eta}} 2 \abs{\dobsT_n}^2 + C_{T, M_T} T^{-M_T}\right),\\
    %     &\leq C_1 K^{\eta(-2 M + 1)}+ C_2 T^{-M_T}.
    % \end{align*}
    % We are specifically interested in how much polynomial evaluation changes at a root $n < K^{\eta}$ by the perturbation $\delta \dbf_K$, which amounts to bounding the value of $\bm \psi_n^T \delta \dbf_K$. To find this, we first must solve the linear system \eqref{eq:Deltadsystem}. The matrix $\tilde{B} + \epsilon I$ is invertible, so the Lagrange multiplier can be found via
    % \begin{equation*}
    %     \mu = -(\bm \psi_0^T (\tilde B+\epsilon I)^{-1} \bm \psi_0)^{-1}.
    % \end{equation*}
    % Then, solving for $\bm \psi_n^T \delta \dbf_K$, we have
    % \begin{equation}
    % \label{eq:Delta-dbf-evaluation}
    %     \bm \psi_n^T \delta \dbf_K = \frac{\bm \psi_n^T (\tilde B + \epsilon I)^{-1} \bm \psi_0}{\bm \psi_0^T (\tilde B + \epsilon I)^{-1} \bm \psi_0}.
    % \end{equation}

    % To bound \eqref{eq:Delta-dbf-evaluation}, we must lower bound the denominator and upper bound the numerator.
    % \mr{Sketchiness starts now.}
    Now, consider the perturbation formula \eqref{eq:lambda-perturbation}. 
    If we bound the numerator quadratic form $\bm \psi_n^T (\tilde B + \epsilon I)^{-1}\bm \psi_0$ to be much smaller than the denominator term $\bm \psi_0^T (\tilde B + \epsilon I)^{-1}\bm \psi_0$, we have our result. 
    For this, let $\delta>0$ be a gap in the spectrum so that $\sigma_m^2 \notin (\sigma_{n}^2 - \delta, \sigma_{n}^2)$ for all $m$.
    Then, we can split the spectrum into $L<\infty$ mode numbers $n_\ell$ where $\sigma_{n_\ell}^2 \geq \sigma_n^2$ and the rest are in the interval $[0, \sigma_n^2-\delta]$.
    By choosing $K>K*$ as in Cor.~\ref{corollary:SVD}, we can diagonalize the operator $\tilde B + \epsilon I$ as
    \begin{equation*}
        \tilde B + \epsilon I = \begin{pmatrix}
            X_1 & X_2
        \end{pmatrix} \begin{pmatrix}
            L_1 & \\ & L_2
        \end{pmatrix}
        \begin{pmatrix}
            X_1^T \\ X_2^T
        \end{pmatrix}
        % \tilde \Psi (\tilde \Sigma^2 + \epsilon I) \tilde \Psi^T + \tilde \Psi_{\perp} (\tilde \Sigma_\perp^2 + \epsilon I) \tilde \Psi_{\perp}^T, 
    \end{equation*}
    where $L_1$ has a spectrum in $[\sigma_n-\delta/4 + \epsilon, \max_{\ell} (\sigma_{n_\ell})+\delta/4+\epsilon]$, $L_2$ has a spectrum in $[\epsilon, \sigma_n-3\delta/4 + \epsilon]$, and $X_1$ and $X_2$ are the associated eigenvectors. 
    % $(\tilde \Sigma^2)_{\ell\ell} = \tilde \sigma_{\ell}^2 \geq \sigma_n^2 - \delta/4 > 3\sigma_n^2/4 $ and $0 \leq ( \tilde \Sigma_{\perp}^2)_{\ell\ell} \leq \sigma_n^2 - 3\delta/4 < \sigma_n^2/4 $. 
    % Additionally, $\tilde \Psi$ orthogonal and its range is close to $\Psi$ \mr{with the bound in the remark}.

    Substituting this representation into \eqref{eq:lambda-perturbation}, we have
    \begin{equation*}
        \delta \lambda_n = -\frac{1}{q'_K(\lambda_n)} \frac{\begin{pmatrix}
            X_1^T \psi_n \\
            X_2^T \psi_n
        \end{pmatrix}^T\begin{pmatrix}
            L_1 & \\ & L_2
        \end{pmatrix}\begin{pmatrix}
            X_1^T \psi_0 \\
            X_2^T \psi_0
        \end{pmatrix}}{\begin{pmatrix}
            X_1^T \psi_0 \\
            X_2^T \psi_0
        \end{pmatrix}^T\begin{pmatrix}
            L_1 & \\ & L_2
        \end{pmatrix}\begin{pmatrix}
            X_1^T \psi_0 \\
            X_2^T \psi_0
        \end{pmatrix}}.
    \end{equation*}
    Due to the regularization, the denominator is bounded from below by $\epsilon$. For the numerator, we will show that $X_2^T \bm \psi_n$ and $X_1^T \bm \psi_0$ are both small. 

    We start with $X_1^T \bm \psi_0$. First, we note that because $X_1$ is unitary,
    \begin{align*}
        \norm{X_1^T \psi_0} &= \norm{X_1 X_1^T \psi_0}. % X_1 is unitary
    \end{align*}
    Now, we can compare this to the projector onto the range of $\Psi_1$ using Corollary \ref{corollary:SVD} and Definition \ref{def:nu-gap}:
    \begin{align*}
         \norm{X_1^T \psi_0} &\leq \norm{(X_1 X_1^T - P_{\Psi_1}) \psi_0} + \norm{P_{\Psi_1} \psi_0} \\ % Subspace angle between X_1 and \Psi_1 is bounded
         &\leq C_* K^{-M_*} + \norm{P_{\Psi_1} \psi_0}.
    \end{align*}
    We can further compare $P_{\Psi_1}$ against $\Psi_1 \Psi_1^T$, giving
    \begin{align*}
        \norm{X_1^T \psi_0} &\leq C_* K^{-M_*} + \norm{(P_{\Psi_1}-\Psi_1 \Psi_1^T)\psi_0} + \norm{\Psi_1 \Psi_1^T \psi_0}.
    \end{align*}
    To bound the middle term, we first note that
    \begin{equation*}
        \norm{P_{\Psi_1} - \Psi_1 \Psi_1^T}_F = \norm{\Psi_1^T \Psi_1 - I}_F.
    \end{equation*}
    Then, because $\Psi_1$ is a submatrix of $\Psi$, the bounds from Corollary \ref{corollary:SVD} apply, giving
    \begin{align*}
        \norm{X_1^T \psi_0} \leq C_1 K^{-M_*}.
    \end{align*}

    As for $X_2^T \bm \psi_n$, we have
    \begin{align*}
        \norm{X_2^T \bm \psi_n}_2 &= \norm{X_2 X_2^T \bm \psi_n}, \\
        &= \norm{(I-X_1 X_1^T) \bm \psi_n}.
    \end{align*}
    Applying the subspace bound from Corollary \ref{corollary:SVD}, we have
    \begin{align*}
        \norm{X_2^T \bm \psi_n}_2 &\leq \norm{(I-P_{\Psi_1}) \bm \psi_n} + \norm{(P_{\Psi_1}-X_1 X_1^T) \bm \psi_n}, \\
        &\leq C_* \norm{\psi_n} K^{-M_*}.
    \end{align*}

    These bounds, combined with the bounds $\norm{L_1}_2 \leq \max_m (\sigma_m)+\delta/4 + \epsilon $ and $\norm{L_2}_2 \leq \sigma_n-3\delta/4 + \epsilon$ give the result.
\end{proof}



==> Deprecated/Appendices/base_polynomial.tex <==
\section{The Base Polynomial}
\label{subsec:45}

In the introduction, we mentioned that not only do we need control over the normal matrix, but also over the filter that we perturb around. For this, we will use the following polynomial:
\begin{lemma}
\label{lemma:refpolybound}
    Let $0 < \omega \leq 1$ have a sequence of continued fractions approximants with $\{a_n / L_n \}$. For any $n \geq 1$ and $\alpha < 1/4$, define the polynomial
    \begin{equation}
    \label{eq:refpoly}
        \refpoly(z) = \left(\prod_{j = 1}^{\floor{\alpha p L_{n}}}\frac{(z - \lambda_j)(z - \lambda_{-j})}{(1 - \lambda_j)(1 - \lambda_{-j})}\right)
        \left(\prod_{j = \floor{\alpha p L_{n}}+1}^{\floor{{p L_{n}}/{2}}}\frac{(z - \tilde \lambda_j)(z - \tilde \lambda_{-j})}{(1 - \tilde \lambda_j)(1 - \tilde \lambda_{-j})}\right)
    \end{equation}
    where for $0 \leq \ell < p$ and $j\geq 0$
    \begin{equation*}
        \tilde \lambda_{j p + \ell} = e^{2 \pi i (j a_n/L_n + \ell)/p}.
    \end{equation*}
    Then, the polynomial obeys the bound $\abs{\refpoly(z)} \leq C_\alpha$ for $\abs{z} \leq 1$ and $C_\alpha > 1$, where $C_\alpha$ is independent of $\omega$ and $m$.
\end{lemma}
\begin{proof}
    The proof consists of comparing the polynomial above to the polynomial with equispaced nodes 
    \begin{equation*}
        Q_{\alpha, \omega, n, p}(z) = \prod_{j = 1}^{\floor{{L_{n}}/{2}}}\frac{(z - \tilde \lambda_j)(z - \tilde \lambda_{-j})}{(1 - \tilde \lambda_j)(1 - \tilde \lambda_{-j})}.
    \end{equation*}
    We begin by assuming $L_n$ is odd. In this case, the polynomial coefficients of $Q_{\alpha, \omega, n, p}$ can be thought of as a column of the inverse discrete Fourier transform. This is because we have $Q(1) = 1$ and $Q(\tilde \lambda_j) = 0$ for $1 \leq \abs{j} \leq \floor{\nicefrac{L_n}{2}}$ So, $Q_{\alpha, \omega, n, p}$ is simply the interpolation of a unit vector that is nonzero at $1$, i.e.~$\qbf = F^{-1} \ebf_0$ where $\qbf$ are the polynomial coefficients and $F$ is the mapping from Fourier coefficients to values at equispaced nodes.

    The problem of how Fourier interpolation changes when the nodes are perturbed is addressed in \cite{yu2023}. In this paper, Yu and Townsend prove an analogue to the Kadec-$1/4$ theorem \cite{kadets1964} from sampling theory, which states that as long as the locations of Fourier nodes does not move a length farther than $\alpha/4$ from the equispaced grid, the mapping from these Fourier space to these modes $\tilde{F}$ does not differ too much in norm from the standard mapping, i.e.
    \begin{equation*}
        \norm{\tilde F} \leq (1 + \phi_\alpha)\norm{F}_2,
    \end{equation*}
    where $\norm{F} = L_n$ and $\phi_\alpha = 1 - \cos \pi \alpha + \sin \pi \alpha$. Additionally, via Weyl's inequality we have
    \begin{equation*}
        \norm{\tilde F^{-1}}_2 \leq \frac{1}{(1 - \phi_\alpha) \norm F}_2.
    \end{equation*}
    
    We can apply these identities to our problem. In particular, we note that continued fraction approximations obey the bound
    \begin{equation*}
        \abs{\omega - \frac{a_n}{L_n}} < \frac{1}{L_n^2}.
    \end{equation*}
    Using this, we find that $\abs{\lambda_j - \tilde \lambda_j} < \alpha \pi / L_n$ for $\abs{j} < \floor{\alpha L_n}$, obeying the hypothesis for the $1/4$ theorem. Hence, the coefficients of $\refpoly$ 
    \begin{equation*}
        \norm{\pbf_{\alpha, \omega, n}}_2 = \norm{\tilde F^{-1} \ebf_0}_2 \leq \frac{1}{(1-\phi_\alpha)\sqrt{L_n}}. 
    \end{equation*}
    The bound directly follows from the above inequality. 
\end{proof}
The polynomials $\refpoly$ also obeys a bound on its derivatives. In Lemma \ref{lemma:refpolyderivbound}, we show that general polynomials with perturbed roots have lower bounds on their derivatives. We state the result for our polynomial as a corollary:
\begin{corollary}
\label{corollary:refpolyderivbound}
    Let $\alpha < 1/4$. The derivative of $\refpoly(z)$ at each root $\lambda$ obeys
    \begin{equation*}
        \abs{\refpoly'(\lambda)} \geq C N^{-4\alpha}
    \end{equation*}
    for some constant $C$.
\end{corollary}
\begin{proof}
    See Lemma \ref{lemma:refpolyderivbound} and use the bounds from the proof of Lemma \ref{lemma:refpolybound}.
\end{proof}


==> Deprecated/Appendices/choosing_L.tex <==
\section{Choosing the Number of Circle Interpolation Modes}
\label{app:choosing-L}
In this section, we will give a method to determine the number of Fourier modes to project a given trajectory onto. 
We will do this by controlling the condition number of the linear system \eqref{eq:circle-projection}.
We define the least-squares condition number of the linear system defined by the matrix $Y = W_T^{1/2} \Phi$ as
\begin{equation*}
    \kappa = \norm{Y^{\dagger}}_2 = \max_{\bm v} \frac{\norm{Y^{\dagger} \bm v}}{\norm{v}_2} = \frac{\sigma_1}{\sigma_L},
\end{equation*}
where $Y^{\dagger} = (\Phi^T W_T \Phi)^{-1}\Phi^T W_T^{1/2}$ is the Moore-Penrose pseudoinverse and $\sigma_1$ and $\sigma_L$ are the smallest and largest singular values of $Y$.

To bound the condition number, we first note that the matrix $Y^T Y$ has a Toeplitz structure:
\begin{equation}
\label{eq:eta_n}
    (Y^T Y)_{mn} = \eta_{n-m} = \sum_{t=0}^{T}w_{t,T+1}\lambda_1^{(n-m)t},
\end{equation}
where we note that $\eta_0 = 1$. In this way, we have a Gershgorin circle bound on the eigenvalues of $Y^T Y$ of
\begin{equation*}
    \abs{\sigma^2_j - 1} \leq 2 \gamma_L = 2 \sum_{n = 1}^{2L} \abs{\eta_n},
\end{equation*}
where we used the fact that $\abs{\eta_n} = \abs{\eta_{-n}}$. This can be translated to a bound on the condition number of
\begin{equation}
\label{eq:condition-bound}
    \kappa \leq \frac{\sqrt{1+2\gamma_L}}{\sqrt{1-2\gamma_L}}.
\end{equation}

The expression \eqref{eq:condition-bound} allows for an algorithm to bound the condition number of this linear system. We simply choose a maximum allowed radius $\gamma_{\max}$, and find the largest $L$ such that $\gamma_L < \gamma_{\max}$. This requires $\mathcal O(L T)$ operations, which is always cheaper than the linear solve. By default, we have found $\gamma_{\max} = 0.5$ to give good results. The algorithm is summarized in the following pseudocode:
\begin{algorithm}[H]
\caption{Parameterization Dimension $L$}
\label{alg:parameterization-dimension}
\begin{algorithmic}[1]
\Require System height $T$, Frequency $\omega$, Tolerance $\gamma_{\max}$
\State $L \gets \ceil{\frac{T-1}{2}}$
\State $\gamma_0 \gets 0$; $n \gets 0$
\While {$n \leq T$}
    \State $n \gets n + 1$
    \State $\gamma_n \gets \gamma_{n-1} + \eta_n$ via \eqref{eq:eta_n}
    \If {$\gamma_n \geq \gamma_{\max}$}
        \State $L \gets \ceil{\frac{n-2}{2}}$
    \EndIf
\EndWhile
\Ensure Parameterization dimension $L$
\end{algorithmic}
\end{algorithm}

==> Deprecated/Appendices/continued_fraction_distribution.tex <==
\section{The distribution of continuous fraction denominators}
\begin{theorem}
For almost all $\omega \in [0,1)$, the denominators of continued fractions $L_n$ obey the limit \cite{khinchin1997}
\begin{equation*}
    \lim_{n\to \infty}L_n^{1/n} \to \gamma,
\end{equation*}
where
\begin{equation*}
    \gamma = \exp\left(\frac{\pi^2}{12 \log 2}\right).
\end{equation*}
\end{theorem}
This allows for us to get the following result
\begin{lemma}
\label{lemma:DenominatorDistribution}
    Let $r, s > 0$ and $\eta < 1$. For almost all $\omega \in [0,1)$, there is a value $M$ such that for all $m > M$, there exists a continued fraction approximation $p_n/L_n$ such that 
    \begin{equation}
        \label{eq:denominatorbounds}
        r m^\eta < L_n < s m.
    \end{equation}
\end{lemma}
\begin{proof}
\mr{This needs to be cleaned up}
    First, we fix $\epsilon > 0$ and note that there exists an $N$ such that 
    \begin{equation*}
        \gamma - \epsilon < L_n^{1/n} < \gamma + \epsilon.
    \end{equation*}
    Taking a logarithm of the above equation and \eqref{eq:denominatorbounds}, it is clear that if we can show the full set of bounds for a given $m$ that there exists and $n$ such that
    \begin{equation}
    \label{eq:bigdenominatorbound}
        \log r + \eta \log m < n \log (\gamma - \epsilon) < \log L_n < n \log(\gamma + \epsilon) < \log s + \log m,
    \end{equation}
    then we have proven our theorem.

    For \eqref{eq:bigdenominatorbound} to hold, we first note that $n > N$ is automatically satisfied when
    \begin{equation*}
        m > M \geq \frac{1}{r^2} (\gamma - \epsilon)^{2N}.
    \end{equation*}
    Additionally, when
    \begin{equation*}
        \log s - \log r + \eta \log m > 2 \log \gamma > 2 \log (\gamma - \epsilon), 
    \end{equation*}
    we are guaranteed that there are at least two points $n$ such that 
    \begin{equation*}
        \log r + \eta \log m < n \log (\gamma - \epsilon) < \log s + \log m.
    \end{equation*}
    In particular, there is a point such that
    \begin{equation*}
        \log r + \eta \log m < n \log (\gamma - \epsilon) < \frac{1}{2}(\log r + \log s) + \frac{2 - \eta}{2} \log m.
    \end{equation*}
    Using the above expression, we additionally know that
    \begin{equation*}
        n \log(\gamma + \epsilon) \leq \frac{\log(\gamma + \epsilon)}{\log(\gamma - \epsilon)}\left[ \frac{1}{2}(\log r + \log s) + \frac{2 - \eta}{2} \log m \right].
    \end{equation*}
    So, if $\epsilon$ is chosen small enough so that
    \begin{equation*}
        \frac{\log(\gamma + \epsilon)}{\log(\gamma - \epsilon)} < \frac{2}{2-\eta},
    \end{equation*}
    then an $M$ can be chosen large enough so that 
    \begin{align*}
        \left(\log s + \log m\right) -& \frac{\log(\gamma + \epsilon)}{\log(\gamma - \epsilon)}\left[ \frac{1}{2}(\log r + \log s) + \frac{2 - \eta}{2} \log m \right] \\
        &\geq \left(1 - \frac{\log(\gamma + \epsilon)}{\log(\gamma - \epsilon)} \frac{2 - \eta}{2}\right) \log M - \frac{1}{2} \frac{\log(\gamma + \epsilon)}{\log(\gamma - \epsilon)}(\log r - \log s) > 0,
    \end{align*}
    and we have our result.
\end{proof}

==> Deprecated/Appendices/fourier_gaps.tex <==
\section{Distribution of gaps in a Fourier series}
\mr{A better version of this must exist somewhere...}
\begin{lemma}
\label{lemma:Fourier-gaps}
    Let $\dobsT$ be a function with a bound on the Fourier coefficients of the form $\abs{\dobsT_n} < C n^{-M}$ for some $M\geq 1$. Then for every $\epsilon > 0$, there exists a gap $\delta$ between values of $\abs{\dobsT_n}$ with the lower bound
    \begin{equation*}
        \delta > C_2 \epsilon^{1 + 1/M}.
    \end{equation*}
\end{lemma}
\begin{proof}
    First, consider the value of $N$ such that $n > N$ implies $\abs{\dobsT_n} < \epsilon/2$. This is given by
    \begin{equation*}
        N = \left( \frac{\epsilon}{2 C}\right)^{-1/M}.
    \end{equation*}
    This means that at most $N$ coefficients can be within the region $(\epsilon/2, \epsilon]$, guaranteeing a gap of size at least $\epsilon/(2N+2)$. This gives our theorem
\end{proof}

==> Deprecated/Appendices/integrated_convergence.tex <==

\section{Integrated Sequence Bound}
\begin{lemma}
    Let $\{a_n\}$ be a sequence with the bound $\abs{a_n} < C n^{-M}$. Then,
    \begin{equation*}
        \abs{\sum_{n>N} a_n} \leq \sum_{n>N}\abs{a_n} \leq C_2 N^{-M+1}.
    \end{equation*}
\end{lemma}
\begin{proof}
    The first part is obvious. The second part is performed by the integral test.
    \begin{align*}
        \sum_{n > N} \abs{a_n} \leq C \sum_{n > N} n^{-M} \leq C \int_{N}^\infty x^{-M} \dif x = \frac{C}{M-1} N^{-M+1}.
    \end{align*}
\end{proof}

\begin{lemma}
\label{lemma:Diophantine}
    Let $\omegabf$ satisfy the Diophantine condition
    \begin{equation*}
        \abs{\nbf \cdot \omega - m} \geq \frac{C}{\abs{\nbf}^{\nu}}.
    \end{equation*}
    Then, 
    \begin{equation*}
        \abs{1-e^{2\pi i \nbf \cdot \omegabf}} > \frac{2C}{\abs{\nbf}^{\nu}}.
    \end{equation*}
\end{lemma}
\begin{proof}
    First, we note that 
    \begin{equation*}
        \abs{1-e^{2\pi i \nbf \cdot \omegabf}} = \abs{\sin\left(\pi (\nbf \cdot \omegabf - m) \right)},
    \end{equation*}
    where we assume $m\in \Zbb$ is chosen so that $\abs{\nbf \cdot \omegabf - m}\leq 1/2$. On this domain, the function 
    \begin{equation*}
        \abs{\sin\left(\pi (\nbf \cdot \omegabf - m) \right)} > 2\abs{\nbf \cdot \omegabf - m} \geq \frac{2C}{\abs{\nbf}^{\nu}}.
    \end{equation*}
\end{proof}

\begin{theorem}
    Under Hypotheses \ref{setting} with $M > \nu + d$, the unweighted Birkhoff average of invariant circles converges as $\Ocal(T^{-1})$. 
\end{theorem}
\begin{proof}
    The unweighted Birkhoff average is given by
    \begin{align*}
        \BA_T[\obs](\xbf) = \sum_{t = 0}^{T-1} \frac{1}{T} (\obs \circ \zbf)(\thetabf + \omegabf).
    \end{align*}
    Using the Fourier series representation of $\obs \circ \zbf$, we have
    \begin{align*}
        \BA_T[\obs](\xbf) - h_0 &= \frac{1}{T} \sum_{\nbf \in\Zbb^d \backslash\{0\}} \obsT_{\nbf}  \sum_{t=0}^{T-1}e^{2\pi i t \nbf \cdot \omegabf},\\
        &= \frac{1}{T} \sum_{\nbf \in\Zbb^d \backslash\{0\}} \obsT_{\nbf} \frac{e^{-2\pi i \nbf \cdot \omegabf}-e^{2\pi i (T-1)\nbf \cdot \omegabf}}{1-e^{2\pi i \nbf \cdot \omegabf}}.
    \end{align*}
    Using the continuity bounds $\abs{\obsT_{\nbf}}<C_h \abs{\nbf}^{-M}$ and Lemma \ref{lemma:Diophantine}, we have
    \begin{align*}
        \abs{\BA_T[\obs](\xbf) - h_0} & \leq \frac{C_h}{C T} \sum_{\nbf \in\Zbb^d \backslash\{0\}} \obsT_{\nbf} \abs{\nbf}^{-M + \nu}.
    \end{align*}
    For the convergence of this sum, we require $-M+\nu < -d$, or $M > d+\nu$.
\end{proof}

==> Deprecated/Appendices/palindromic_roots.tex <==
\section{Finding the Roots of a Palindromic Polynomial}
\label{app:palindromic-roots}
Here, we detail how we solve for the roots of palindromic polynomials. This method is no more or less accurate than solving for the eigenvalues of the standard Frobenius companion matrix (see the book by Trefethen\cite{trefethen2013} for an introduction). However, this process halves the dimension of the eigenvalue problem, resulting a significantly faster method than the standard companion matrix approach. 

The algorithm results from the observation that palindromic polynomials of the form 
\begin{equation*}
    P(z) = \sum_{k = 0}^{2K} c_k z^{k},
\end{equation*}
can be reduced to degree $K$ polynomials in $(z+z^{-1})/2$. In particular, we have that
\begin{equation*}
    z^{-K} P(z) = Q\left(\frac{z+z^{-1}}{2}\right), \qquad Q(x) = \sum_{k=0}^K b_k T_k(x),
\end{equation*}
where $T_k$ are the Chebyshev polynomials. If all of the roots of $P$ are on the unit circle, the change of variables implies that all the roots of the $Q$ are on the interval $[-1,1]$, so we expect Chebyshev polynomials to be well conditioned for this problem. Typically results of Birkhoff RRE have almost all of the roots on the unit circle for non-chaotic orbits, so they satisfy this assumption. Additionally, using the Chebyshev three-term recurrence
\begin{align*}
    T_0(x) &= 1, \\
    T_1(x) &= x, \\
    T_{n+1}(x) &= 2x T_n - T_{n-1},
\end{align*}
one sees that the polynomials in $z$ coordinates have a convenient form of
\begin{equation*}
    T_k\left(\frac{z+z^{-1}}{2} \right) = \frac{z^k + z^{-k}}{2}.
\end{equation*}
This results in the convenient relations
\begin{equation*}
    b_k = \begin{cases}
        c_K, & k=0, \\
        2c_{K+k}, & 0<k\leq K.
    \end{cases}
\end{equation*}

To find the roots of $p$, we use the Chebyshev colleague matrix
\begin{equation*}
    C = \begin{pmatrix}
        0 & 1 \\
        \frac12 & 0 & \frac12 \\
         & \frac12 & 0 & \ddots   \\
          & & \ddots & \ddots & \frac12 \\
         & &  & \frac12  & 0
    \end{pmatrix} - \frac{1}{2 b_K} 
    \begin{pmatrix}
        b_0 & \dots & b_{K-1}
    \end{pmatrix}
    \begin{pmatrix}
        0 \\ \vdots \\ 0 \\ 1
    \end{pmatrix}.
\end{equation*}
The eigenvalues $x_n$ of this matrix, found via \texttt{eigvals} in Julia, are the roots of the polynomial $q$.
In order to get roots of $p$, we simply solve the equation
\begin{equation*}
    \frac{z + z^{-1}}{2} = x_n
\end{equation*}
for both values of $z$. 
We note that this equation is sensitive near $x_n = \pm 1$, so the Chebyshev method here does not avoid larger errors of frequencies near $0$ and $1/2$. 





==> Deprecated/Appendices/polynomial_derivative_bound.tex <==
\section{Bounding the polynomial derivative}
\begin{lemma}
\label{lemma:refpolyderivbound}
    Let
    \begin{equation*}
        p(z) = \prod_{\substack{0 \leq n < N \\ n \neq 0}} \frac{z - \lambda_n}{\lambda_0 - \lambda_n}, \qquad \lambda_n = e^{2\pi i (n + \alpha_n)/N},
    \end{equation*}
    where $\alpha_n < \alpha$. If $\alpha < 1/4$, the derivative of $p$ at the roots $\lambda_m$ obeys
    \begin{equation*}
        \abs{p'(\lambda_m)} \geq C N^{-4\alpha}, \qquad 1 \leq m < N
    \end{equation*}
    for some constant $C$.
\end{lemma}
\begin{proof}
    Evaluating $p'$ at a node, we have
    \begin{equation*}
        p'(\lambda_m) = \frac{1}{\lambda_0 - \lambda_m} \prod_{\substack{0 \leq n < N \\ n \neq 0, m}}\frac{\lambda_m - \lambda_n}{\lambda_0 - \lambda_n}.
    \end{equation*}
    We can reorder the product numerator so that
    \begin{equation*}
        p'(\lambda_m) = \frac{1}{\lambda_0 - \lambda_m} \prod_{\substack{0 \leq n < N \\ n \neq 0, m}}\frac{\lambda_m - \lambda_{m - n}}{\lambda_0 - \lambda_n},
    \end{equation*}
    where we identify $\lambda_n = \lambda_{n-N}$. Focusing on the term inside the product, we have
    \begin{equation*}
        \lambda_m - \lambda_n = 2 i e^{\pi i (m + n +\alpha_m + \alpha_n)/N} \sin\left(\pi \frac{m - n + \alpha_m - \alpha_n}{N} \right),
    \end{equation*}
    so
    \begin{equation*}
        \frac{\lambda_m - \lambda_{m-n}}{\lambda_0 - \lambda_n} = - e^{\pi i (\alpha_m + \alpha_{m-n} - \alpha_0 - \alpha_n)} \frac{\sin\left(\pi (n + \alpha_m - \alpha_{m-n})/N \right)}{\sin\left(\pi (n + \alpha_n - \alpha_{0})/N \right)},
    \end{equation*}
    and
    \begin{align*}
        \log \abs{p'(\lambda_m)} =& \log \abs{\frac{1}{\lambda_0 - \lambda_m} } + \sum_{\substack{0 \leq n < N \\ n \neq 0, m}} \log \left(\frac{\sin\left(\pi (n + \alpha_m - \alpha_{m-n})/N \right)}{\sin\left(\pi (n + \alpha_n - \alpha_{0})/N \right)}\right), \\
        =& \ C + \sum_{\substack{0 \leq n < \floor{(N-1)/2} \\ n \neq 0, m}}\log \left(\frac{\sin\left(\pi (n + \alpha_m - \alpha)/N \right)}{\sin\left(\pi (n - \alpha_{0} + \alpha )/N \right)}\right) \\
        &+\sum_{\substack{\ceil{(N-1)/2 + 1} \leq n < N \\ n \neq 0, m}}\log \left(\frac{\sin\left(\pi (n + \alpha_m + \alpha)/N \right)}{\sin\left(\pi (n - \alpha_{0} - \alpha )/N \right)}\right),
    \end{align*}
    where $C$ is a constant that includes the the leading term as well as the factor contributed by $n=N/2$ when $N$ is even, which are both bounded from below. Now, for $0 \leq n < \floor{(N-1)/2}$, we have
    \begin{equation*}
        \sin\left(\frac{\pi(n + \alpha_m - \alpha)}{N}\right) 
        \geq 
        \sin\left( \frac{\pi (n - \alpha_0 + \alpha)}{N}\right) 
        - \frac{\pi (2 \alpha - \alpha_0 - \alpha_m)}{N}
        \cos\left(\frac{\pi(n + \alpha_m - \alpha)}{N}\right).
    \end{equation*}
    So,
    \begin{align*}
        \sum_{\substack{0 \leq n < \floor{(N-1)/2} \\ n \neq 0, m}} &\log \left(\frac{\sin\left(\pi (n + \alpha_m - \alpha)/N \right)}{\sin\left(\pi (n - \alpha_{0} + \alpha )/N \right)}\right)
        \geq \\ & \geq
        \sum_{\substack{1 \leq n < \floor{(N-1)/2}}} \log \left( 1 - \frac{\pi (2 \alpha - \alpha_0 - \alpha_m)}{N} \frac{\cos\left(\pi(n + \alpha_m - \alpha)/N\right)}{\sin\left(\pi (n - \alpha_{0} + \alpha )/N \right)}\right),\\
        & \geq 
        \sum_{\substack{1 \leq n < \floor{(N-1)/2}}} \log \left( 1 - \frac{\pi (2 \alpha - \alpha_0 - \alpha_m)}{N} \cot\left(\pi (n - \alpha_{0} + \alpha )/N \right)\right), \\
        & \geq
        \sum_{\substack{1 \leq n < \floor{(N-1)/2}}} \log \left( 1 - \frac{2 \alpha - \alpha_0 - \alpha_m}{n - \alpha_{0} + \alpha} \right), \\
        & \geq -(2\alpha - \alpha_0 - \alpha_m) \sum_{\substack{1 \leq n < \floor{(N-1)/2}}} \frac{1}{n - \alpha_0 + \alpha}, \\
        % & \geq -\frac{(2 \alpha - \alpha_0 - \alpha_m)(1 + 2 \alpha)}{1-2\alpha} \sum_{\substack{1 \leq n < \floor{(N-1)/2}}} \frac{1}{n - \alpha_{0} + \alpha}, \\
        & \geq  -(2\alpha - \alpha_0 - \alpha_m) \left(\frac{1}{1-\alpha_0 + \alpha} + \int_{1-\alpha_0 + \alpha}^{N/2} \frac{1}{x} \dif x \right), \\
        & =  -(2\alpha - \alpha_0 - \alpha_m)\left(\frac{1}{1-\alpha_0 + \alpha} - \log(1 - \alpha_0 + \alpha) - \log 2 + \log(N) \right), \\
        & \geq -(2\alpha - \alpha_0 - \alpha_m) \log N + C,
    \end{align*}
    where we used $\alpha < 1/4$ for the logarithm to have a valid domain and the facts that $1/x \geq \cot x$ for $0 < x \leq \pi/2$ and $\log(1 - y) \geq -y/(1-y)$ for $0 \leq y < 1$. By symmetry, we similarly have
    \begin{align*}
        \sum_{\substack{\ceil{(N-1)/2 + 1} \leq n < N \\ n \neq 0, m}}\log \left(\frac{\sin\left(\pi (n + \alpha_m + \alpha)/N \right)}{\sin\left(\pi (n - \alpha_{0} - \alpha )/N \right)}\right) \geq -(2\alpha + \alpha_0 + \alpha_m) \log N + C,
    \end{align*}
    In total, we find
    \begin{align*}
        \log \abs{p'(\lambda_m)} \geq - 4 \alpha \log N + C,
    \end{align*}
    so
    \begin{align*}
        \abs{p'(\lambda_m)} \geq C N^{- 4 \alpha }
    \end{align*}
\end{proof}

==> Deprecated/Appendices/symmetric_eigenvalue_perturbation_theorems.tex <==
\section{Eigenvalue Problem Perturbation Theorems}
Here, we quote three eigenvalue perturbation theorems used in the proofs herein. For the following theorems, denote $\mathcal L(A)$ as the set of eigenvalues of a matrix $A$. All theorems are taken from Stewart and Sun\cite{Stewart1990} (SS).

\begin{theorem}[Gershgorin, SS Thm.~2.2.1]
\label{thm:gershgorin}
For $A \in \Cbb^{n\times n}$ let
\begin{equation*}
    R_i = \sum_{j \neq i} \abs{a_{ij}}
\end{equation*}
and
\begin{equation*}
    \mathcal G_i(A) = \left\{z \in \Cbb \mid \abs{z-a_{ii}} \leq a_i \right\}.
\end{equation*}
Then 
\begin{equation*}
    \mathcal L (A) \subset \bigcup_{i=1}^n \mathcal G_i(A).
\end{equation*}
\end{theorem}

\begin{theorem}[Weyl's, SS Cor.~4.4.9] 
\label{thm:Weyl}
Let $A$ and $E$ be symmetric matrices with eigenvalues $\{\sigma_i\}$ and $\{\epsilon_i\}$ respectively, ordered so that $\sigma_i \geq \sigma_{i+1}$ and $\epsilon_i \geq \epsilon_{i+1}$.  Then, for $i = 1, \dots, n$, the eigenvalues $\tilde{\sigma}_i$ of $\tilde{A} = A + E$ satisfy
\begin{equation*}
    \tilde{\sigma}_i \in [\sigma_i + \epsilon_n, \sigma_i + \epsilon_1].
\end{equation*}
\end{theorem}

\begin{theorem}[Davis-Kahan $\sin(\Theta)$, SS Thm.~5.3.4, 5.3.6, 5.3.8]
\label{thm:DavisKahan}
    Let $A$ be a Hermitian matrix with spectral resolution
    \begin{equation*}
        \begin{pmatrix}
            X_1^* \\ X_2^*
        \end{pmatrix}
        A
        \begin{pmatrix}
            X_1 & X_2
        \end{pmatrix}
        = 
        \Diag(L_1, L_2),
    \end{equation*}
    where $\begin{pmatrix}
        X_1 & X_2
    \end{pmatrix}$ is unitary with $X_1 \in \Cbb^{n\times k}$. Let $Z \in \Cbb^{n\times k}$, and $M\in \Cbb^{k\times k}$ be Hermitian, and
    \begin{equation*}
        R = A Z - Z M.
    \end{equation*}
    Suppose that 
    \begin{equation*}
        \mathcal L (M) \subset [\alpha, \beta]
    \end{equation*}
    and that for some $\delta > 0$
    \begin{equation*}
        \mathcal L (L_2) \subset \mathbb{R} \backslash [\alpha-\delta, \beta + \delta].
    \end{equation*}
    Then for any unitarially invariant norm
    \begin{equation*}
        \norm{\sin \Theta[\Rcal(X_1), \Rcal(Z)]} \leq \frac{\norm{R}}{\delta \inf_2(Z)},
    \end{equation*}
    where $\inf_2(Z)$ is the smallest singular value of $Z$. 
\end{theorem}


==> Deprecated/Sections/0abstract.tex <==
\begin{abstract}
% insert abstract here
\end{abstract}

==> Deprecated/Sections/0glossary.tex <==
\section*{Glossary of quantities}
\mr{There are too many letters in this document, so I am making something that at least keeps track of things. Disclaimer: the use of tildes is also inconsistent and mostly bad. It appears that I started using tildes to designate objects that had been projected down by $P$. However, this logic conflicts directly with the thing I define as $A$, making it so that the tildes probably just do more to confuse than help...}
\begin{center}
    \begin{tabular}{c|c}
         Quantity & Meaning \\ \hline
         $\Rbb$ & The real numbers \\
         $\Tbb$ & The torus on $[0,1)$ \\
         $\Zbb$ & The integers \\\
         $C^M$  & $M$-times differentiable functions \\
         $L^p$ & Space of functions with bounded $p$-norm \\
         $M$ & Commonly used for number of derivatives, including... \\
         $M_g$ & for $\dobsT$ \\
         $M_T$ & for \cref{lemma:ET_entrywise} \mr{Probably a bad name}\\
         $\sympmap$ & The symplectic map \\
         $\zbf$ & An invariant circle \\
         $\omega$ & The rotation number in $\Tbb$ \\
         $c$, $\nu$ & Diophantine constants \\
         $\obs$ & Observable on $\Rbb^2$ \\
         $\obsT$ & Observable composed with KAM parameterization on $\Tbb$ \\
         $\obsT_n$ & Fourier coefficients of $\obsT$ \\
         $\dobsT$ & $\obsT \circ R_\omega - \obsT$, main function used in the analysis \\
         $m$, $n$, $\ell$, $t$, $j$ & Integers \\
         $\theta$ & Element of $\Tbb$ \\
         $T$ & Maximum time in Birkhoff average \\
         $\BA_T$ & Finite-time Birkhoff average \\
         $\BA$ & Birkhoff average limit \\
         $\WBA_T$ & Weighted Birkhoff average \\
         $w_{t,T}$ & Weighted Birkhoff average weights \\
         $w$ & Function that $w_{t,T}$ are sampled from \mr{Change this?}\\ 
         & \textbf{and} bound used for non-uniform DFT theorems \\
         $\lambda_n$ & Ideal roots of filter polynomial : $e^{2\pi i n \omega}$ \\
         $\filter$ & Filter weights (to be solved for, cf. $w_t$) \\
         $K$ & $\filter$ is length $2K+1$ \\
         $\ebf_n$ & $n$th unit vector \\
         $\abf_t$ & Samples of $\obs$ \\
         $\Abf_t$ & Averaged values of $\abf_t$ with $\filter$ \\
         $\ubf_t$ & $\abf_{t+1} - \abf_t$, samples of $\dobs$ \\
         $U$ & Rectangular block Hankel matrix with entries $\ubf_t$ \\
         & Also used as a matrix in SVD \mr{This one seems fine} \\
    \end{tabular}
    \begin{tabular}{c|c}
        Continued... \\ \hline
         $P_K$ & Polynomial with coefficients $\filter$ \\
         $F_K$ & Filter operation on sequence $\obs$ \\
         $P$, $G$, $P_{\xi}$ & Time reversal projection matrices \\
         $\halffilter$ & Folded filter weights $P \filter$ \\
         $\tilde{A}$ & Matrix in least-squares problem \\ 
         $A$ & Limit of $\tilde{A}$ as $T\to\infty$ \\
         $\epsilon$ & Regularization parameter \\ 
         & Also used for some other small numbers \\
         $J$ & Number of islands \\ 
         $\phi_n$ & Cosine basis function used in the proof \\
         $W$ & Diagonal matrix with weights $w_t$ \\ 
         $\psi_n$ & Weighted cosine basis function $W^{1/2} \phi_n$ \\
         $\dbf$ & Weighted filter polynomial $W^{-1/2} \filter$ \\
         $\tilde{B}$ & Weighted least-squares matrix \\
         $B$ & Limit of $\tilde{B}$ as $T \to \infty$ \\
         $E$ & Error matrix, including \\
         $E_T$ & Error in $\tilde{E}$ due to finite $T$: $\tilde A - A$ \\
         $E_B$ & Error in $B$ due to finite $K$ \\
         $E_\Delta$ & Error in $B$ from SVD with known SVs from non-orthogonality \\
         $\Sigma$ & Matrix of approximate singular values of $B$ \\ 
         $\Delta$ & Matrix used for perturbation of near-orthogonal modes \\
         $N$ & Number of modes $\psi_n$ considered in approximating $\tilde B$ \\&(choice of $N$ discussed after \cref{thm:SVD}) \\
         $\Xcal$, $\Ycal$ & Subspaces \\
         $X$, $Y$ & orthogonal matrices representing $\Xcal$ and $\Ycal$ \\
         $\delta$ & Spectral gap \\ 
         $L_n$ & Continued fraction denominators of $\omega$ \\
         $P_{\alpha, \omega, n}$ & Polynomials used for comparison \\
         $\gamma$ & Proportionality constant in adaptive algorithm \\
         $\bar{\epsilon}$ & Convergence tolerance of adaptive algorithm \\
    \end{tabular}
\end{center}

==> Deprecated/Sections/1introduction.tex <==
\section{Introduction}
Invariant tori are ubiquitous structures in symplectic maps and Hamiltonian dynamics. 
Examples of systems with invariant tori include the pendulum, the standard map, halo orbits in astrodynamics \cite{kolemen2012}, and the nested flux surfaces in magnetic confinement devices\cite{paul2022}.
Such orbits are known to be stable to perturbation due to the KAM theorem \cite{LLave_2004}.
However, numerically identifying orbits from trajectories is often difficult, due to both the difficulties of high-dimensional geometry and the problems of small denominators.

One standard numerical method to find invariant tori is the parameterization method \cite{haro2016}.
This method is based on the same Newton iteration on the conjugacy relation, and can be accelerated using the fast Fourier transform.
This allows for highly accurate computations of invariant tori, which can be proven to exist by a numerical variant of the KAM theorem \cite{Figueras2017}. 
However, one of the main drawbacks of the parameterization method is that it needs an initial guess.
In the case of 1D and 1.5D Hamiltonian systems, a manual initial guess can found relatively easily with a Poincar\'e plot of a trajectory.
Once one solution is found, continuation\cite{kolemen2012} can be used to find more solutions.
However, in the cases of higher dimensional systems or islands, initial guesses are significantly more difficult find.
The initial guess issue is faced by other methods relying on iterations on torus parameterizations, such as the flux minimizing surfaces\cite{dewar1992,dewar1994}.

Additionally, initial guesses of the rotation number are also difficult.
Simple methods for finding the rotation are available for invariant circles where there is a natural point to wind about.
In such cases, one can find the rotation number via classical limits\cite{guckenheimer1997} or more accurately using the weighted Birkhoff average\cite{Das2018,sander2020,sander2023} or Richardson-like extrapolation algorithms\cite{Luque2014,Villanueva2022}\mr{Need to check this citation}. 
Once the rotation number is found, then it is straightforward to find a parameterization of the orbit \cite{blessing2023}.
Without good guesses at the winding structure, the typical solution is to look for peaks in the Fourier spectrum of the signal. 
Unfortunately, these peaks are only as accurate as the discretization resolution of the spectrum.
This issue is again made more complicated in higher dimensions, where winding is a less well-defined concept.

An additional issue that we will discuss is that of orbit classification.
Before an invariant torus can be fit to a trajectory, we must first be confident that trajectory is, in fact, a torus.
Classical methods for this typically rely on the Lyapunov exponent, but this can be quite slow to converge.
More recently, the rapid convergence of the weighted Birkhoff average\cite{Das2016,Das2017,Das2018,Das2019,sander2020,sander2023} (WBA) has been shown to be capable distinguishing chaotic from non-chaotic trajectories.

In application settings, symplectic maps typically arise from evolving Hamiltonian dynamics by numerical integration, and this can present its own problems.
One problem is that of noise: reliable methods must be robust to potentially non-symplectic errors in the symplectic map.
This is particularly relevant when symplectic integrators are not available for a given application.
We note that for the parameterization method, this is alleviated by a overdetermined formulation of the method\cite{Baresi2018}.
A second issue is that of the cost of evaluating the map.
Both the parameterization method using the Fast Fourier Transform and WBA can be performed in nearly linear time in the number of samples, so the dominant cost is typically dominated by evolving Hamiltonian trajectories.
When considering classifying potentially large numbers of trajectories, any reduction in the number of evaluations is very useful.
We note that structured symplectic interpolants such as the HenonNet\cite{Burby2021}, SympNet\cite{Jin2020}, or a Gaussian Process approach\cite{Rath2021} can be used to alleviate both issues of numerical integration.
However, symplectic interpolants are necessarily nonlinear, and may require more data than simply finding the invariant circle. 
Linear interpolants can similarly be used, but require high accuracy, and the evaluation time of the interpolant may still represent the dominant cost of any algorithm.

In this paper, we classify and parameterize invariant tori from single trajectories efficiently in the number of map evaluations. 
For the classification step, we will rely on a variant of the reduced rank extrapolation method\cite{Sidi2017}, which we will refer to as Birkhoff RRE.
Birkhoff RRE works by attempting to find a filter (or linear model) for measurements on a trajectory using only the time-series information.
Because Birkhoff RRE only depends on a single trajectory, it does not require any initial guesses or continuation of invariant tori.
Additionally, Birkhoff RRE is phrased as a linear least-squares problem.
This means its implementation is straightforward and robust, and there is a residual indicating the fit of the linear model.
We prove that when the trajectory is on an invariant torus, the residual of Birkhoff RRE approaches zero as rapidly as the weighted Birkhoff average, allowing for the same classification ability.
Additionally, we show experimentally that RRE converges significantly faster than WBA on a set of trajectories of the standard map, with a large majority of trajectories being classified to highly accurate residuals below $10^{-11}$ in fewer than $1000$ iterations of the map.

For the parameterization step, we show that the frequencies filtered by the Birkhoff RRE filter are multiples of the rotation number. 
In particular, we prove that these frequencies converge with similar rates to the residual, allowing for highly accurate approximations of the rotation number.
This proof is novel, as typical proofs for RRE typically require the composing linear modes to decay, which we do not see.
By finding the frequencies of the signal, we show experimentally that we can identify both the number of islands and rotation numbers for maps in 2D. 
Once this information is known, we project the signal back onto the corresponding Fourier modes, giving a parameterization of the invariant torus.
We note that this process is quite similar to that of the filter diagonalization method\cite{Mandelshtam2001}.

We proceed by first introducing the necessary background in Sec.~\ref{sec:background}, including a review of the weighted Birkhoff average.
In Sec.~\ref{sec:method}, we build upon WBA to introduce the Birkhoff RRE algorithm, stating the relevant convergence theorems (the proofs of which are given in App.~\ref{sec:proofs}).
Then, in Sec.~\ref{sec:examples}, we show two examples of the method.
In the first example, we examine the convergence of Birkhoff RRE on the standard map, confirming the predicted rates from Sec.~\ref{sec:method}.
Then, in the second example, we show how the method can be applied to an example on a symplectic map obtained from a toroidal plasma confinement device known as a stellarator, showing how the method can be used in a real-world situation.
Finally, we conclude in Sec.~\ref{sec:conclusions}.


==> Deprecated/Sections/2background.tex <==
\section{Background}
\label{sec:background}

% Make a figure of the standard map, showing circles, islands, and chaos
\begin{figure*}
    \centering
    \includegraphics[width=0.7\textwidth]{Figures/sm1_rotation_and_chaos.png}
    \caption{Phase portrait of the standard map \eqref{eq:standard-map}. Parameterizations of the invariant circles and islands are obtained via the methodology in Sec.~\ref{sec:method}, using Algorithm \ref{alg:adaptiveRRE} with $\epsilon=0$, $\gamma=3$, $\delta=10^{-10}$, $K_{\mathrm{init}}=50$, $K_{\max}=600$, and $\Delta K = 50$. Invariant circles and islands are colored according to their rotation numbers, while trajectories classified as chaotic are plotted in black. }
    \label{fig:standard-map}
\end{figure*}

We consider maps of the form $\sympmap : X \to X$, where $X$ is a $C^M$ manifold. A $d$-dimensional \textit{invariant torus} is a map $\zbf : \Tbb^d \to X$ that satisfies the conjugacy
\begin{equation*}
    \sympmap \circ \zbf - \zbf \circ R_\omega = 0,
\end{equation*}
where $R_\omega : \Tbb^d \to \Tbb^d$ is the rotation map $R_\omega(\thetabf) = \thetabf + \omegabf$ with $\omegabf \in \Tbb^d$. The invariant torus has an associated invariant measure $\mu$ on its image $X_0 \subseteq X$. We assume that the invariant tori are smooth enough, i.e.~$\zbf \in C^M$ for some positive integer $M$ or $\zbf \in C^\infty$. We refer to $d=1$ invariant tori as \textit{invariant circles}. 

We additionally require the rotation vector $\omegabf$ satisfy the $(c, \nu)$ Diophantine condition 
\begin{equation*} 
    \abs{\omegabf \cdot \nbf - m} \geq \frac{c}{\norm{\nbf}^{\nu}} \qquad \text{for all } \nbf\in\Zbb^d\backslash \{0\}, \ m \in \Zbb.
\end{equation*}
For $d=1$, the Diophantine condition tells us the $\omega \in \Rbb$ is ``sufficiently irrational.''
In higher dimensions, the condition additionally gives a measure of irrational independence, requiring that the rotation numbers also be far from being rational multiples of the others.
It is important to note that the Diophantine condition, while technical, is satisfied by almost all rotation numbers under the Lebesgue measure \cite{LLave_2004}.
It is therefore safe to assume that an arbitrarily sampled invariant torus is Diophantine. 

We define an \textit{island} to be a set of $p \geq 1$ tori $\zbf^{(j)}:\Tbb^d \to X$ with $1 \leq j \leq p$ such that for some $\omegabf$ the following conjugacy is satisfied:
\begin{equation}
\label{eq:island-conjugacy}
    \sympmap \circ \zbf^{(j)} = \begin{cases}
        \zbf^{(j+1)}, & 1 \leq j < p,\\
        \zbf^{(1)} \circ R_\omega, & j = p.
    \end{cases}
\end{equation}
A direct result of the above definition is that each $\zbf^{(j)}$ is an invariant torus of the map $\sympmap^p$ (and hence a $p=1$ island is equivalent to an invariant torus). 
Another special case of an island is a periodic orbit, where each $\zbf^{(j)}$ is a constant function.

We note that the definitions of invariant tori and islands above do not require any special properties of the map.
However, they are both commonly found in the case of \textit{symplectic maps}, which preserve some symplectic 2-form under the pushforward of the map.
In the case of symplectic maps, we will refer to everything that is not deemed integrable (i.e.~an invariant torus or island) as \textit{chaotic}. 
Unfortunately, this definition ignores much of the nuance of invariant structures in symplectic maps.
For instance, cantori\cite{meiss2015} are cantor-like orbits that have been proven to exist in the standard map.
Cantori are not space filling (a standard property of chaos), but neither are they conjugate to the torus; it depends on application whether such orbits count as ``chaos.''
In our case, we heuristically use chaos as a name for orbits that do not match the assumptions of integrability (and so the cantorus would be chaotic), but likely a more refined definition would be needed for the technical details of chaos.

% Paragraph on the standard map here
% Give equation of the standard map \label{eq:standard-map}
% Rotation number is only uniquely defined on [0.0, 0.5]
In Fig.~\ref{fig:standard-map}, we plot the phase portrait of the Chirikov standard map $F : (x_t, y_t) \mapsto (x_{t+1}, y_{t+1})$ where
\begin{align}
\nonumber
    x_{t+1} &= x_t + y_{t+1} \mod 1,\\
\label{eq:standard-map}
    y_{t+1} &= y_t - \frac{k}{2\pi} \sin (2\pi x_t),
\end{align}
and $k=0.7$. The map has invariant circles (e.g.~nested about $(0,0)$ and the blue-to-green gradient of trajectories in the center), islands (e.g.~the $p=2$ island chain centered at $(0.0,0.5)$ and $(0.5,0.5)$), and chaos in black (e.g.~about $(0.5, 0)$). The invariant circles and islands are both colored by the rotation number $\omega$, found using the methods in Sec.~\ref{sec:method}. We note that $\omega$ has a unique representation in $[0.0,0.5]$ due both to the fact that $\omega \in \Tbb$ and the freedom to take $\theta \to -\theta$ in the parameterization. 



To categorize orbits, we consider the problem of finding ergodic averages. Let $\obs : X \to \Rbb^D$ be an observable function on our state space. The \textit{Birkhoff average} of $\obs$ is defined as the limit of finite time averages:
\begin{equation*}
    \BA[\obs](\xbf) = \lim_{\Kback \to \infty} \BA_{\Kback}[\obs](\xbf)
\end{equation*}
where
\begin{equation*}
    \BA_{\Kback}[\obs] = \frac{1}{\Kback} \sum_{k=0}^{\Kback-1} (\obs \circ \sympmap^k)(\xbf).
\end{equation*}
For functions $\obs \in L^1(X_0)$ where $X_0$ is the set $\xbf$ is ergodic on, the Birkhoff ergodic theorem \cite{???} guarantees the convergence of the Birkhoff average almost everywhere to the spatial average
\begin{equation*}
    \BA[\obs](\xbf) = \int_{X_0}\obs(\xbf) \dif \mu.
\end{equation*}
Additionally, when $\obs\in C^M$ for $M>\nu+d$, one can show that the partial averages have an error $\abs{\BA[\obs] - \BA_{\Kback}[\obs]} = \Ocal(\Kback^{-1})$ on invariant circles and islands. In contrast, chaotic trajectories are conjectured to have a convergence rate of $\Ocal(\Kback^{-1/2})$\cite{sander2020}. 


If we compose the observable with an invariant circle, we can define the observable using coordinates on the torus. That is, if we let $\obsT = \obs \circ \zbf$, the finite-time Birkhoff average of the function $\obsT$ at a point $\thetabf \in \Tbb^d$ is 
\begin{equation*}
    \BA_{\Kback}[\obsT](\thetabf) = \frac{1}{\Kback} \sum_{k=0}^{\Kback-1} (\obsT \circ R_\omega^k)(\thetabf) = \frac{1}{\Kback} \sum_{k=0}^{\Kback-1} (\obs \circ \sympmap^k)(\zbf(\thetabf)).
\end{equation*}
Assuming $\obsT$ is continuous and $\omegabf$ is irrational and rationally independent (i.e.~$R_\omega$ is ergodic on $\Tbb^d$), the limit of these averages is independent of the initial point, where the average is given by the Birkhoff ergodic theorem as
\begin{equation}
\label{eq:BirkhoffAverage}
    \BA[\obsT] = \lim_{\Kback \to \infty} \BA_{\Kback}[\obsT] = \int_{\Tbb^d} \obsT(\thetabf) \dif \thetabf.
\end{equation}
In this way, we connect averages of time series to averages over invariant tori.

One application of Birkhoff averages is to find Fourier coefficients of $\obsT$. Consider that
\begin{equation*}
    \obsT(\thetabf) = \sum_{\nbf \in \Zbb^d} \obsT_{\nbf} e^{2\pi i \nbf \cdot \thetabf}.
\end{equation*}
Then, we can determine the coefficients $\obsT_{\nbf}$ simply by noting
\begin{align}
\label{eq:FourierBirkhoff}
    \obsT_{\nbf} &= \int_{\Tbb^d} \obsT(\theta)e^{-2\pi i \nbf \cdot \thetabf} \dif \thetabf \\
\nonumber
    &= \BA\left[\obsT(\star) e^{-2\pi i \nbf \cdot \star}\right]\\
\nonumber
    &= \lim_{\Kback \to \infty} \frac{1}{\Kback} \sum_{k=0}^{\Kback-1}\obsT(k \omegabf) e^{2\pi i k \nbf \cdot \omegabf},
\end{align}
where we use `$\star$' for the argument to be averaged over.
If $\obs$ is the identity (and therefore the dynamics occur on Euclidean space), the coefficients $\obsT_{\nbf} = \zbf_{\nbf}$ provide a Fourier parameterization of an invariant torus
\begin{equation*}
    \zbf(\thetabf) = \sum_{n\in\Zbb} \zbf_{\nbf} e^{2\pi i \nbf \cdot \thetabf} = \sum_{n\in\Zbb}\BA\left[\zbf(\star) e^{-2\pi i \nbf \cdot \omegabf \star}\right] e^{2\pi i n \theta}.
\end{equation*}
Additionally, the ergodic average of $\obsT$ without weighting is an algorithm to obtain $\obsT_0 = \BA[\obsT]$. 

In order to apply the above process for finding coefficients, one must first obtain the rotation vector. For invariant circles, another application of the ergodic average is to obtain the rotation number $\omega$. For instance, if one has access to a symplectic map $\sympmap:\Tbb\times \Rbb \to \Tbb \times \Rbb$ of the form 
\begin{equation}
\label{eq:winding_map}
    x_{t+1} = x_t + y_{t+1} \mod 1, \qquad y_{t+1} = F(x_t, y_t),
\end{equation}
the average of $y$ is the rotation number of irreducible circles (i.e., those that wind exactly around the torus). Additionally, if one has access to a point $\xbf_0$ inside of an invariant circle $\zbf \subset \Rbb^2$, one can often find the rotation number by averaging the winding about that point.

However, the winding process to find rotation numbers has some potential difficulties. 
The most immediate difficulty is with orbits that have complicated shapes (such as crescent- or banana-like orbits), where the average position lies outside of the circle.
Even more difficult is when $\zbf$ is not injective, as can happen when considering delay embeddings.

Another difficulty is automatically analyzing islands.
Using the fact that islands consist of $p$ periodic circles, one can similarly define Fourier series for the observable on each island $\obsT^{(j)} = \obs\circ \zbf^{(j)}$. Then, we see that the subsequences associated with each island in the chain can be written as
\begin{equation}
\label{eq:a-island-single}
    \abf_{j+s p} = \sum_{\nbf\in\Zbb^d} \obsT_{\nbf}^{(j)}e^{2\pi i s \nbf \cdot \omegabf}.
\end{equation}
For each $n$, the coefficients $\obsT_{\nbf}^{(j)}$ can be written as a finite discrete Fourier series 
\begin{equation*}
    \obsT^{(j)}_{\nbf} = \sum_{m = 0}^{p-1} \obsT_{m\nbf} e^{2\pi i m j / p}.
\end{equation*}
Combining this with \eqref{eq:a-island-single}, we find that the full sequence can be written as 
\begin{equation}
\label{eq:a-island}
    \abf_t = \sum_{\nbf\in\Zbb^d} \sum_{m=0}^{p-1} \obsT_{m\nbf} e^{2\pi i t (\nbf \cdot \omegabf + m)/p}
\end{equation}
From this, we see signals associated with islands have two frequency components: the rational frequencies $m/p$ associated with jumping between islands and the irrational frequencies $\nbf \cdot \omegabf/p$ associated with the rotation number.
So, when considering averaging maps such as \eqref{eq:winding_map}, averaging $y_t$ will typically return a rational number $m/p$ associated with the number of islands, rather than the rotation. 
One process could be to use the denominator could be used to identify islands (as is done in Sander and Meiss\cite{sander2020}), and then use a second average could be used to determine rotation.
In the case of higher-dimensional tori and islands, there are multiple irrational frequencies, making it increasingly difficult to solve for frequencies using winding. 

Another difficulty is that the $\Ocal(\Kback^{-1})$ convergence rate of the Birkhoff averages on circles and islands is too slow for most applications.
For smooth enough maps and invariant circles, this can be improved via the \textit{weighted Birkhoff average}
\begin{equation}
\label{eq:WBA}
    \WBA_{\Kback}[\obs](\xbf) = \sum_{k = 0}^{\Kback-1} w_{k,\Kback} (\obs \circ \sympmap^k)(\xbf),
\end{equation}
where the coefficients $w_{k,\Kback}$ are sampled from a positive function $w\in C^{\infty}$ compactly supported on $[0,1]$ as
\begin{equation*}
    w_{k,\Kback} = \left(\sum_{j=0}^{\Kback-1} w\left(\frac{j+1}{\Kback+1} \right)\right)^{-1} w\left(\frac{k+1}{\Kback+1} \right).
\end{equation*}

To state the convergence rate theorem of the weighted Birkhoff average, we first summarize our assumptions:
\begin{hypotheses}
\label{setting}
    We assume that the three hypotheses hold:
    \begin{enumerate}[label=H\arabic*.]
        \item (Smooth bump function) We have a bump function $w\in C^{\infty}(\Rbb)$ with compact support on $[0,1]$ and $w(x)>0$ for all $x\in(0,1)$.
        \item (Diophantine) We have a rotation vector $\omegabf$ satisfying a $(c,\nu)$ Diophantine condition.
        \item (Smooth system) We have a symplectic map defined as $\sympmap : X \to X$ where $X$ is a $C^M$ manifold and $\sympmap \in C^M$. Additionally, $X_0 \subseteq X$ is a set where $\sympmap$ is conjugate to island dynamics with $\zbf^{(j)}\in C^M$ (see \eqref{eq:island-conjugacy}), rotation vector $\omegabf$, invariant measure $\mu$ and period $p\geq1$. Finally, $\obs:X\to \Rbb^d$ is an observable in $C^M$.
    \end{enumerate}
\end{hypotheses}
Additionally, we note that the simpler case of an invariant circle can be considered by setting $p=1$ in the above setting. The following theorem gives the convergence rate of the weighted Birkhoff average:
\begin{theorem}[Das and Yorke\cite{Das2018} Thm 3.1] 
\label{thm:Das2018}
Let $m>1$ be an integer. Under Hypotheses~\ref{setting}, there is a constant $C_m$ depending on $w$, $\obs$, $m$, $M$, $\nu$, and $p$ but independent of $\xbf \in X_0$ such that
\begin{equation*}
    \abs{\WBA_{\Kback} [\obs](\xbf) - \int_{X_0}\obs \dif \mu} \leq C_m \Kback^{-m},
\end{equation*}
provided the `smoothness' $M$ satisfies
\begin{equation*}
    M > d + m\nu.
\end{equation*}
\end{theorem}
Theorem \ref{thm:Das2018} has been slightly modified for this work. 
Specifically, we have assumed $w\in C^\infty$ and extended the theorem to the case of islands. 
An alternative proof of this theorem is included in Sec.~\ref{app:WBA}. 
The proof deviates from the original by emphasizing the approximate orthogonality of the individual Fourier modes under the weighting function in Lemma \ref{lemma:lambda-orthogonality}.

When $M=\infty$ for Thm.~\ref{thm:Das2018}, one can obtain constants $C_m$ for any $m \in \Nbb$. That is, the weighted Birkhoff average converges as $\Ocal(\Kback^{-m})$ for all $m$. Of course, this is useful if you want to quickly compute Birkhoff averages. Additionally, this result does not hold for chaotic trajectories, so the convergence rate of the weighted Birkhoff average can be used to classify trajectories \cite{sander2020}. 

\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{Figures/PaperBackground.png}
    \caption{ (top) A test signal $\obsT(\theta) = e^{\cos 2\pi \theta}$, sampled at the points $\omega t$ where $\omega = (\sqrt 5 - 1)/2$. (middle) A discrete Fourier transform of the signal, showing peaks near the expected frequencies. (bottom) Three candidate $\Kback=11$ filters: the all-ones filter, a weighted Birkhoff filter, and an tuned filter to the first five roots of the frequency. We see that the all-ones filter is largest where there is a large amount of power if the signal, the weighted filter is small far from the zero frequency, and the tuned filter is zero exactly at the relevant frequencies. The absolute errors of the Birkhoff average for each filter are: (all-ones) $7.11 \times 10^{-2}$, (weighted Birkhoff) $7.38 \times 10^{-3}$, and (tuned) $2.72 \times 10^{-5}$.}
    \label{fig:background}
\end{figure*}

One way of understanding the weighted Birkhoff average is as a filter on the sequence $\obsT_t = \obs(\sympmap^t(\xbf))$. When $\xbf$ is on an invariant torus, the sequence of observables has the form
\begin{equation}
\label{eq:a-sequence}
    \abf_t = (\sympmap^t\circ \obs)(\xbf) = \obsT(\omegabf t) = \sum_{n \in \Zbb} \obsT_{\nbf} \lambda_{\nbf}^t, \quad \lambda_{\nbf} = e^{2\pi i \nbf \cdot \omegabf}.
\end{equation}
That is, the sequence $\abf_t$ is built out of equispaced samples of the trigonometric functions $e^{2\pi i \theta \nbf \cdot \omegabf}$. When we apply the weights $w_{k,\Kback}$ to the sequence and flip the order of summation, we find that
\begin{equation*}
    \WBA_{\Kback}[\obsT] = \sum_{n\in\Zbb} \obsT_{\nbf} P(\lambda_{\nbf}), \qquad P(\lambda) = \sum_{k = 0}^{\Kback-1} w_{k,\Kback} \lambda^k.
\end{equation*}
In this way, the weights act as a filter, where $w_{k,\Kback}$ will preferentially remove frequencies from the signal where the polynomial $P$ is small. An effective filter will return the mean $\obsT_0$, i.e.~$P(1) = 1$. The rest of the frequencies contribute to the error, so ideally $\abs{P(\lambda_{\nbf})} \ll 1$ for $\nbf \neq 0$. This is particularly important for the small $\abs{\nbf}$ modes that dominate the signal.

In Fig.~\ref{fig:background}, we see an example of this for an example observable $h(\theta) = e^{\cos (2\pi \theta)}$. We sample this signal at equispaced points $h(\omega t)$ where $\omega = (\sqrt 5-1)/2$ is the golden ratio. The top plot shows this signal and the samples. The middle plot shows a windowed discrete Fourier transform of the length $10000$ signal. The peaks of the power of the signal appear regularly at multiples of the frequency $\omega$, as is expected from the Fourier form of \eqref{eq:a-sequence}. In the bottom plot, we plot $\abs{P(e^{2\pi i \omega \theta})}$ for three potential filters:
\begin{itemize}
    \item The ``all-ones'' filter $w_{k,\Kback} = 1/\Kback$, used for the regular Birkhoff average.
    \item The weighted Birkhoff filter $w_{k,\Kback}$ sampled from the window function
\begin{equation*}
    w = e^{- ( t (1 - t))^{-1}}.
\end{equation*}
    \item A ``tuned'' filter that perfectly eliminates the first $\floor{\Kback/2}$ frequencies, found from the coefficients of the polynomial
    \begin{equation*}
        P_{\mathrm{tuned}} = \prod_{k=1}^{\floor{\Kback/2}}\frac{(z-e^{2\pi i \omega k})(z-e^{-2\pi i \omega k})}{(1-e^{2\pi i \omega k})(1-e^{-2\pi i \omega k})}.
    \end{equation*}
\end{itemize}
In each case we take $\Kback = 11$. In each case, we can judge the absolute error of the filter's average by comparing it to the exact average (found via a weighted Birkhoff average with $\Kback=10^4$ to be $1.266066$). From Fig.~\ref{fig:background} (bottom), we see the all-ones filter polynomial has relatively large value at the peaks of the spectrum, resulting in the worst error of $7.11 \times 10^{-2}$. The weighted Birkhoff filter is much smaller at the spectral peaks with the most mass, resulting in a more accurate average with error $7.38 \times 10^{-3}$. The tuned filter does the best, with an error of $2.72 \times 10^{-5}$. 

We note that while the tuned filter is small at the frequencies that dominate the signal, it is large in between. So, while the tuned filter worked well for this example, it would not work well if applied to a signal with a different value of $\omega$, as the polynomial roots are specifically related to multiples of the rotation number. 

% \section{Background}
% \label{sec:background}
% In this paper, we will primarily consider maps of the form $\sympmap : X \to X$, where $X$ is a $C^M$ manifold. An \textit{invariant circle} of the map $\sympmap$ satisfies the equation $\zbf : \Tbb \to X$ that satisfies the conjugacy
% \begin{equation*}
%     \sympmap \circ \zbf - \zbf \circ R_\omega = 0,
% \end{equation*}
% where $R_\omega : \Tbb \to \Tbb$ is the rotation map $R_\omega(\theta) = \theta + \omega$. We let the image of $\zbf$ be $X_0 \subseteq X$, and we let $\mu$ be the unique invariant measure on $X_0$. Typically, invariant circles are assumed to have some level of regularity, e.g.~$\zbf \in C^M$ for some positive integer $M$ or $\zbf \in C^\infty$. Additionally, we require that the rotation number $\omega$ satisfies the $(c, \nu)$ Diophantine condition 
% \begin{equation*}
%     \abs{\omega - \frac{m}{n}} \geq \frac{c}{n^{\nu + 1}}.
% \end{equation*}
% We will consider an \textit{island} to be a set of $p \geq 1$ circles $\zbf^{(j)}$ with $1 \leq j \leq p$ such that 
% \begin{equation}
% \label{eq:island-conjugacy}
%     \sympmap \circ \zbf^{(j)} = \begin{cases}
%         \zbf^{(j+1)}, & 1 \leq j < p,\\
%         \zbf^{(1)} \circ R_\omega, & j = p.
%     \end{cases}
% \end{equation}
% A natural result of the above definition of an island is that each $\zbf_{(j)}$ is an invariant circle of the map $\sympmap^p$ (and hence a $p=1$ island is equivalent to an invariant circle). 

% We are concerned with finding ergodic averages of functions on the circle. Let $\obs : X \to \Rbb^d$ be an observable function on our state space. The \textit{Birkhoff average} of $\obs$ is defined as the limit of finite time averages:
% \begin{equation*}
%     \BA[\obs](\xbf) = \lim_{\Kback \to \infty} \BA_{\Kback}[\obs](\xbf)
% \end{equation*}
% where
% \begin{equation*}
%     \BA_{\Kback}[\obs] = \frac{1}{\Kback} \sum_{k=0}^{\Kback-1} (\obs \circ \sympmap^k)(\xbf).
% \end{equation*}
% The Birkhoff ergodic theorem guarantees the convergence of the Birkhoff average almost everywhere for $\obs \in L^1$ to the spatial average
% \begin{equation*}
%     \BA[\obs](\xbf) = \int_{X_0}\obs(\xbf) \dif \mu.
% \end{equation*}
% Additionally, when $\obs\in C^M$ for $M>\nu+1$, one can show that the partial averages have an error $\abs{\BA[\obs] - \BA_{\Kback}[\obs]} = \Ocal(\Kback^{-1})$ on invariant circles and islands. In contrast, chaotic trajectories appear to have a convergence rate of $\Ocal(\Kback^{-1/2})$. 


% If we compose the observable with an invariant circle, we can define an observable function on the torus, i.e.~$\obsT = \obs \circ \zbf$. The finite-time Birkhoff average of the function $\obsT$ at a point $\theta \in \Tbb$ is defined (using slightly overloaded notation) as
% \begin{equation*}
%     \BA_{\Kback}[\obsT](\theta) = \frac{1}{\Kback} \sum_{k=0}^{\Kback-1} (\obsT \circ R_\omega^k)(\theta_0) = \frac{1}{\Kback} \sum_{k=0}^{\Kback-1} (\obs \circ \sympmap^k)(\zbf(\theta_0)).
% \end{equation*}
% Assuming $\obsT$ is continuous and $\omega$ is irrational, the limit of these averages is independent of the initial point, where the average is given by the Birkhoff ergodic theorem as
% \begin{equation}
% \label{eq:BirkhoffAverage}
%     \BA[\obsT] = \lim_{\Kback \to \infty} \BA_{\Kback}[\obsT] = \int_\Tbb \obsT(\theta) \dif \theta.
% \end{equation}
% In this way, we connect averages of time series to averages over invariant circles.

% One application of Birkhoff averages is to find Fourier coefficients of $\obsT$. Consider that
% \begin{equation*}
%     \obsT = \sum_{n \in \Zbb} \obsT_n e^{2\pi i n \theta}.
% \end{equation*}
% Then, we can determine the coefficients $\obsT_n$ simply by noting
% \begin{align}
% \label{eq:FourierBirkhoff}
%     \obsT_n &= \int_{\Tbb} \obsT(\theta)e^{-2\pi i n \theta} \dif \theta \\
% \nonumber
%     &= \BA\left[\obsT(\cdot) e^{-2\pi i n \cdot}\right]\\
% \nonumber
%     &= \lim_{\Kback \to \infty} \frac{1}{\Kback} \sum_{k=0}^{\Kback-1}\obsT(\omega k) e^{2\pi i n \omega k}. 
% \end{align}
% If $\obs$ is the identity, the coefficients $\obsT_n = \zbf_n$ provide a Fourier parameterization of an invariant circle
% \begin{equation*}
%     \zbf(\theta) = \sum_{n\in\Zbb} \zbf_n e^{2\pi i n \theta} = \sum_{n\in\Zbb}\BA\left[\zbf(\cdot) e^{-2\pi i n \cdot})\right] e^{2\pi i n \theta}.
% \end{equation*}
% Additionally, the ergodic average of $\obsT$ without weighting is an algorithm to obtain $\obsT_0 = \BA[\obsT]$. 

% In order to apply the above process for finding coefficients, one must obtain the rotation number. In many cases, another application of the ergodic average is to obtain the rotation number $\omega$. For instance, if one has access to a symplectic map $\sympmap:\Tbb\times \Rbb \to \Tbb \times \Rbb$ of the form 
% \begin{equation}
% \label{eq:winding_map}
%     x_{t+1} = x + y_{t+1}, \qquad y_{t+1} = F(x_t, y_t),
% \end{equation}
% the average of $y$ is the rotation number of irreducible circles (i.e., those that wind exactly around the torus). Additionally, if one has access to a point $\xbf_0$ inside of an invariant circle $\zbf \subset \Rbb^2$, one can find the rotation number by averaging the winding about that point.

% However, the winding process to find rotation numbers has some potential difficulties. 
% The most immediate difficulty is with orbits that have complicated shapes (such as crescent- or banana-like orbits), where the average position lies outside of the circle.
% Even more difficult is when $\zbf$ is not injective, as can happen when considering delay embeddings.

% Another difficulty is automatically analyzing islands.
% Using the fact that islands consist of $p$ periodic circles, one can similarly define Fourier series for the observable on each island $\obsT^{(j)} = \obs\circ \zbf^{(j)}$. Then, we see that the subsequences associated with each island in the chain can be written as
% \begin{equation}
% \label{eq:a-island-single}
%     \abf_{j+s p} = \sum_{n\in\Zbb} \obsT_n^{(j)}e^{2\pi i n \omega s}.
% \end{equation}
% For each $n$, the coefficients $\obsT_n^{(j)}$ can be written as a finite discrete Fourier series 
% \begin{equation*}
%     \obsT^{(j)}_n = \sum_{m = 0}^{p-1} \obsT_{mn} e^{2\pi i m j / p}.
% \end{equation*}
% Combining this with \eqref{eq:a-island-single}, we find that the full sequence can be written as 
% \begin{equation}
% \label{eq:a-island}
%     \abf_t = \sum_{n\in\Zbb} \sum_{m=0}^{p-1} \obsT_{mn} e^{2\pi i (n \omega t + m t)/p}
% \end{equation}
% In particular, what one sees is that the signals associated with islands have two frequency components: the rational frequencies $m/p$ associated with jumping between islands and the irrational frequencies $n\omega/p$ associated with the rotation number.
% So, when considering averaging maps such as \eqref{eq:winding_map}, averaging $y_t$ will typically return a rational number $m/p$ associated with the number of islands, rather than the rotation. 
% One process could be to use the denominator could be used to identify islands (as is done in \cite{sander2020}), and then use a second average could be used to determine rotation.
% In the case of higher-dimensional tori and islands, there are also multiple irrational frequencies, making it increasingly difficult to solve for frequencies using winding. 

% Another difficulty is that the $\Ocal(\Kback^{-1})$ convergence rate of the Birkhoff averages on circles and islands is too slow for most applications.
% For smooth enough maps and invariant circles, this can be improved via the \textit{weighted Birkhoff average}
% \begin{equation}
% \label{eq:WBA}
%     \WBA_{\Kback}[\obs](\xbf) = \sum_{k = 0}^{\Kback-1} w_{k,\Kback} (\obs \circ \sympmap^k)(\xbf),
% \end{equation}
% where the coefficients $w_{k,\Kback}$ are sampled from a positive function $w\in C^{\infty}$ compactly supported on $[0,1]$ as
% \begin{equation*}
%     w_{k,\Kback} = \left(\sum_{j=0}^{\Kback-1} w\left(\frac{j+1}{\Kback+1} \right)\right)^{-1} w\left(\frac{k+1}{\Kback+1} \right).
% \end{equation*}

% We can summarize our assumptions in the following setting:
% \begin{hypotheses}
% \label{setting}
%     We assume that the three hypotheses hold:
%     \begin{enumerate}[label=H\arabic*.]
%         \item (Smooth bump function) We have a bump function $w\in C^{\infty}(\Rbb)$ with compact support on $[0,1]$ and $w(x)>0$ for all $x\in(0,1)$.
%         \item (Diophantine) We have a rotation number $\omega$ satisfying a Diophantine condition $(c,\nu)$.
%         \item (Smooth system) We have a symplectic map defined as $\sympmap : X \to X$ where $X$ is a $C^M$ manifold and $\sympmap \in C^M$. Additionally, $X_0 \subseteq X$ is a set where $\sympmap$ is conjugate to island dynamics with $\zbf^{(j)}\in C^M$ (see \eqref{eq:island-conjugacy}), rotation number $\omega$, invariant measure $\mu$ and period $p\geq1$. Finally, $\obs:X\to \Rbb^d$ is an observable in $C^M$.
%     \end{enumerate}
% \end{hypotheses}
% Additionally, we note that the simpler case of an invariant circle can be considered by setting $p=1$ in the above setting. The following theorem gives the convergence rate of the weighted Birkhoff average:
% \begin{theorem}[Das and Yorke\cite{Das2018} Thm 3.1] 
% \label{thm:Das2018}
% Let $m>1$ be an integer. Under Hypotheses~\ref{setting}, there is a constant $C_m$ depending on $w$, $\obs$, $m$, $M$, $\nu$, and $p$ but independent of $x \in X_0$ such that
% \begin{equation*}
%     \abs{\WBA_{\Kback} [\obs](x) - \int_{X_0}\obs \dif \mu} \leq C_m \Kback^{-m},
% \end{equation*}
% provided the `smoothness' $M$ satisfies
% \begin{equation*}
%     M > 1 + m(1+\nu).
% \end{equation*}
% \end{theorem}
% Theorem \ref{thm:Das2018} has been slightly modified for this work. 
% In particular, we have (1) assumed $w\in C^\infty$, (2) restricted ourselves to 1-dimensional quasiperiodic dynamics, and (3) extended the theorem to the case of islands. 
% A proof of this theorem can be found in Sec.~\ref{app:WBA}. 
% The proof deviates from the original by emphasizing the approximate orthogonality of the individual Fourier modes under the weighting function in Lemma \ref{lemma:lambda-orthogonality}.

% When $M=\infty$ for Thm.~\ref{thm:Das2018}, one can obtain constants $C_m$ for any $m \in \Nbb$. That is, the weighted Birkhoff average converges as $\Ocal(\Kback^{-m})$ for all $m$. Of course, this is useful if you want to quickly compute Birkhoff averages. Additionally, this result does not hold for chaotic trajectories, so the convergence rate of the weighted Birkhoff average can be used to classify trajectories \cite{sander2020}. 

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.8\textwidth]{Figures/PaperBackground.png}
%     \caption{ (top) A test signal $\obsT(\theta) = e^{\cos 2\pi \theta}$, sampled at the points $\omega t$ where $\omega = (\sqrt 5 - 1)/2$. (middle) A discrete Fourier transform of the signal, showing peaks near the expected frequencies. (bottom) Three candidate $\Kback=11$ filters: the all-ones filter, a weighted Birkhoff filter, and an tuned filter to the first five roots of the frequency. We see that the all-ones filter is largest where there is a large amount of power if the signal, the weighted filter is small far from the zero frequency, and the tuned filter is zero exactly at the relevant frequencies. The absolute errors of the Birkhoff average for each filter are: (all-ones) $7.11 \times 10^{-2}$, (weighted Birkhoff) $7.38 \times 10^{-3}$, and (tuned) $2.72 \times 10^{-5}$.}
%     \label{fig:background}
% \end{figure*}

% An intuitive way of understanding the weighted Birkhoff average is as a filter on the sequence $\obsT_t = \obs(\sympmap^t(\xbf))$. When $\xbf$ is on an invariant circle, the sequence of observables has the form
% \begin{equation}
% \label{eq:a-sequence}
%     \abf_t = (\sympmap^t\circ \obs)(\xbf) = \obsT(\omega t) = \sum_{n \in \Zbb} \obsT_n \lambda_n^t, \quad \lambda_n = e^{2\pi i n \omega}.
% \end{equation}
% That is, the sequence $\abf_t$ is built out of equispaced samples of the trigonometric functions $e^{2\pi i n \omega \theta}$. When we apply the weights $w_{k,\Kback}$ to the sequence, we find that
% \begin{equation*}
%     \WBA_{\Kback}[\obsT] = \sum_{n\in\Zbb} \obsT_n p(\lambda_n), \qquad p(\lambda) = \sum_{k = 0}^{\Kback-1} w_{k,\Kback} \lambda^k.
% \end{equation*}
% In this way, the weights act as a filter, where $w_{k,\Kback}$ will preferentially remove frequencies from the signal where the polynomial $p$ is small. 

% In Fig.~\ref{fig:background}, we see an example of this for an example observable $h(\theta) = e^{\cos (2\pi \theta)}$. We sample this signal at equispaced points $h(\omega t)$ where $\omega = (\sqrt 5-1)/2$ is the golden ratio. The top plot shows this signal and the samples. The middle plot shows a windowed discrete Fourier transform of the length $10000$ signal. The peaks of the power of the signal appear regularly at multiples of the frequency $\omega$, as is expected from the Fourier form of \eqref{eq:a-sequence}. In the bottom plot, we plot $\abs{p(e^{2\pi i \omega \theta})}$ for three potential filters:
% \begin{itemize}
%     \item The ``all-ones'' filter $w_{k,\Kback} = 1/\Kback$, used for the regular Birkhoff average.
%     \item The weighted Birkhoff filter $w_{k,\Kback}$ sampled from the window function
% \begin{equation*}
%     w = e^{- ( t (1 - t))^{-1}}.
% \end{equation*}
%     \item A ``tuned'' filter that perfectly eliminates the first $\floor{\Kback/2}$ frequencies, found from the coefficients of the polynomial
%     \begin{equation*}
%         p_{\mathrm{tuned}} = \prod_{k=1}^{\floor{\Kback/2}}\frac{(z-e^{2\pi i \omega k})(z-e^{-2\pi i \omega k})}{(1-e^{2\pi i \omega k})(1-e^{-2\pi i \omega k})}.
%     \end{equation*}
% \end{itemize}
% In each case we take $\Kback = 11$. In each case, we can judge the absolute error of the filter's average by comparing it to the exact average (found via a weighted Birkhoff average with $\Kback=10^4$ to be $1.266066$). From Fig.~\ref{fig:background} (bottom), we see the all-ones filter polynomial has relatively large value at the peaks of the spectrum, resulting in the worst error of $7.11 \times 10^{-2}$. The weighted Birkhoff filter is much smaller at the spectral peaks with the most mass, resulting in a more accurate average with error $7.38 \times 10^{-3}$. The tuned filter does the best, with an error of $2.72 \times 10^{-5}$. 

% We note that while the tuned filter is small at the frequencies that dominate the signal, it is large in between. So, while the tuned filter worked well for this example, it would not work well if applied to a signal with a different value of $\omega$, as the polynomial roots are specifically related to multiples of the rotation number. 



==> Deprecated/Sections/3method.tex <==
\section{The Birkhoff Reduced Residual Extrapolation Method (Birkhoff RRE)}
\label{sec:method}
At the end of the previous section, we observed an important property: a filter that is tuned to specific frequencies in a signal can be significantly more effective than an arbitrary bump function. 
In this section, we will introduce a method to learn such a filter from a trajectory.

% Thus, if we were able to learn such a filter, we may be able to find the average much faster. Additionally, if the tuned filter polynomial has roots at multiples of the rotation number, we could determine the rotation number from the trajectory.

In Sec.~\ref{subsec:31}, we introduce a continuous problem for finding such an optimal filter on an invariant circle. Then, we discretize this problem with a Birkhoff average in Sec.~\ref{subsec:32}, which results in a variation of the reduced rank extrapolation (RRE) method \cite{Sidi2017}. Finally, in Sec.~\ref{subsec:33} we explain how we process the obtained filter to find the rotation number of invariant circles.


\subsection{The Least-Squares Problem}
\label{subsec:31}
We begin by defining a function for the action of a filter
\begin{equation*}
    \Fcal_{\Kback}[\obs](\xbf_0) = \sum_{k=0}^{\Kback-1} c_k (\obs \circ \sympmap^k)(\xbf_0),
\end{equation*}
and we call the associated filter polynomial $P_{\Kback}$. 
Note that this is equivalent to a regular Birkhoff average if $c_k = 1/\Kback$ and a weighted Birkhoff average if $c_k = w_{k,\Kback}$. 
Our goal is to find coefficients $c_k$ so that $\norm{\Fcal_{\Kback}[\obsT](\star) - \obsT_0}_{L^2}$ is small, where we are taking a norm over an ergodic region $X_0\subseteq X$ of the form
\begin{equation*}
    \norm{f}_{L^2}^2 = \int_{X_0} \abs{f(\xbf)}^2 \dif \mu.
\end{equation*}
% In the case that the trajectory is an invariant circle or island, this will happen by the filter learning the frequencies of the trajectory. 

% However, we cannot directly minimize 
However, there is a problem: we do not know $\obsT_0$ \textit{a priori}, so we cannot directly minimize $\norm{\Fcal_{\Kback}[\obsT](\star) - \obsT_0}_{L^2}$. 
So, we instead consider filtering the function 
\begin{equation*}
    \dobs(\xbf_0) = (\obs \circ \sympmap)(\xbf_0) - \obs(\xbf_0).
\end{equation*}
This is a convenient choice because $\dobs$ has zero mean and it is easy to calculate from a trajectory of $\obs$. Given $\dobs$, the new goal is to minimize $\norm{\Fcal \dobs(\cdot)}_{L^2}$, under the constraint that $\sum_k c_k = 1$. The constraint ensures the associated polynomial satisfies $P_{\Kback}(1) = 1$, a necessary condition to return the average. Additionally, on an invariant circle or island, $\dobs$ has the same type of Fourier series representation as $\obsT$. So, if a filter learns the rotation vector of $\dobs$, it will also be the rotation vector associated with $\obs$.

The final problem is the method to discretize the norm. For this, we will use a weighted Birkhoff average \eqref{eq:WBA}: 
\begin{equation}
\label{eq:FKg}
    \norm{\Fcal_{\Kback} \dobs}^2_{L^2} \approx \WBA_T \left[\abs{(\Fcal_{\Kback} \dobs \circ \sympmap^t)(\star)}^2\right](\xbf_0).
\end{equation}
Assuming the conditions of Thm.~\ref{thm:Das2018} are met, we can bound the error of the above approximation by
\begin{equation*}
    \abs{\norm{\Fcal_{\Kback} \dobs}^2_{L^2(\Tbb)} - \WBA_T \left[\abs{(\Fcal_{\Kback} \dobs \circ R_\omega^t)(\star)}^2\right](\thetabf_0) } < C T^{-m}
\end{equation*}
for some $C > 0$ and integer $m$. 

In summary, the sum on the right hand side of \eqref{eq:FKg} can be seen as measure of how good a given filter $\filter$ is on an invariant set. Additionally, one can obtain this approximation using only a single trajectory of the dynamical system, rather than having \textit{a-priori} information. We note that we could have also used an unweighted Birkhoff average, and with no more assumptions, this would exactly recover RRE. However, primarily for theoretical reasons, the weighted Birkhoff average acts as a convenient weighting for RRE. In the following section, we will further discuss the details of the implementation of the algorithm.

\subsection{Least Squares Solution}
\label{subsec:32}
Now that we have an energy to minimize, we will discuss the numerical steps. We begin by observing a structure of invariant circle and island signals: they come from pure Fourier series. That is, there are no growing or decaying modes, so the frequencies that we hope to learn via the filter all correspond to roots on the unit circle. Such roots do not change under time reversal (i.e. the conjugate pair $(\lambda_{\nbf}, \bar{\lambda}_{\nbf}) \to (\bar{\lambda}_{\nbf}, \lambda_{\nbf})$ as $t \to -t$). This property corresponds to a linear constraint on the filter that 
\begin{equation}
\label{eq:time-reversal-invariance}
    c_{K+k} - c_{K-k} = 0,    
\end{equation}
where $0 \leq k < K$. Filters satisfying \eqref{eq:time-reversal-invariance} are known as \textit{palindromic}. We note that the converse is not true: time reversal symmetry does not imply roots on the unit circle. However, while not strictly necessary, we have found that this constraint dramatically improves the quality of the results. Throughout the rest of this paper, we will use $K$ to refer to a filter of length $2K+1$, whereas we used $\Kback$ and $T$ to represent filters of length $\Kback$ and $T$ respectively. We will find that $K$ is the number of unknowns of the final least-squares problem.

For the algorithm in this section, we will assume that the user has access to an initial point $\xbf_0 \in X$, a symplectic map $\sympmap$, and an observable function $\obs$. The algorithm begins by simply sampling a trajectory of length $T+2K+1$ starting at $\xbf_0$ by repeated application of $\sympmap$. For many test maps, such as the standard map, this step is very quick. However, in applications where evaluating $\sympmap$ involves simulating a Hamiltonian dynamical system, this step could potentially be the most expensive of the algorithm.

From here, we compute the difference sequence $\ubf_t = \abf_{t+1} - \abf_{t}$ for $0 \leq t < T$. This step amounts to computing the difference function $\dobs \circ \sympmap^t$ from the previous section. Using this notation, the weighted Birkhoff average in \eqref{eq:FKg} can be expressed as the product
\begin{equation*}
    \WBA_T \left[\abs{(\Fcal_{\Kback} \dobs \circ \sympmap^t)(\star)}^2\right](\xbf_0) = \filter^T U^T W_T U \filter,
\end{equation*}
where $U \in \Rbb^{TD\times (2K+1)}$ is the block-Hankel matrix
\begin{equation*}
U = \begin{pmatrix}
        \ubf_{0}   & \ubf_{1} & \dots  & \ubf_{2K} \\
        \ubf_{1}   & \ubf_{2} & \dots  & \ubf_{2K+1} \\
        \vdots     & \vdots   & \ddots & \vdots\\
        \ubf_{T-1} & \ubf_{T} & \dots & \ubf_{T-1+2K}
    \end{pmatrix},
\end{equation*}
and $W_T$ is a diagonal matrix with the weighted Birkhoff weights
\begin{equation*}
   W_T = \begin{pmatrix}
        w_{0, T} \\
        & \ddots \\
        & & w_{T-1, T}
    \end{pmatrix}.
\end{equation*}
We note that the matrix-vector product $U \filter$ can be interpreted as the filter being applied to sliding windows of $\ubf_t$, i.e.~$(U\filter)_t = \Fcal_K[\dobs\circ \sympmap^t](\xbf_0)$. 

For the full least squares problem, we require two more components. First, a filter must return the correct mean, which corresponds to the constraint that $\filter \cdot \bm{1} = P_K(1) = 1$. Second, we add a small amount of regularization. The weighting for the regularization is chosen based on the fact that filters are dual to signals. As such, the filters are regularized via the inverse of another weighted Birkhoff matrix $W_K \in \Rbb^{(2K+1) \times (2K+1)}$ with entries 
\begin{equation*}
    (W_K)_{kk} = \tilde{w}_{k,K} = \frac{w_{k, 2K+1} + w_{K-k, 2K+1}}{2}.
\end{equation*}
Note that $W_K$ has been symmetrized to respect the palindromic symmetry, and can equivalently be thought of as sampling the symmetric bump function $w(1/2 - x) + w(1/2 + x)$. 

In total, we define the following least-squares problem for finding $\filter$: 
\begin{gather}
\label{eq:lsqr1}
    R^2 = \min_{\filter \in \Rbb^{2K+1}} \norm{\begin{pmatrix}
        W_T^{1/2} U \\ \epsilon^{1/2} W_{K}^{-1/2}
    \end{pmatrix}\filter}^2,\\
\nonumber
    \text{s.t. } \bm{1} \cdot \filter = 1, \ \ G\filter = 0,
\end{gather}
where $\epsilon \geq 0$ is a regularization parameter and
\begin{equation*}
    G = \begin{pmatrix} 
           &         & -1 & 0 & 1 &        &   \\
           & \iddots &    &   &   & \ddots &   \\
        -1 &         &    &   &   &        & 1        
    \end{pmatrix}.
\end{equation*}
Here, $G\filter = 0$ is equivalent to the palindromic symmetry \eqref{eq:time-reversal-invariance}. The above problem can be recognized as a weighted and time-reversal constrained version of RRE. 

We enforce the palindromic constraint $G$ by instead considering the projection matrix $P \in \Rbb^{K+1 \times 2K+1}$ and the vector $\halffilter = P \filter$ where $P$ is the orthogonal subspace to $G$
\begin{align}
\label{eq:Pprojection}
    P = \frac{1}{\sqrt{2}}\begin{pmatrix} 
          &         &   & \sqrt{2} &   &        &   \\
          &         & 1 &          & 1 &        &   \\
          & \iddots &   &          &   & \ddots &   \\
        1 &         &   &          &   &        & 1 
    \end{pmatrix}.
\end{align}
Substituting the matrix into \eqref{eq:lsqr1}, we find
\begin{gather}
\label{eq:LeastSquares}
R^2 = \min_{\halffilter \in \Rbb^{K+1}} \halffilter^T \tilde{A} \halffilter + \epsilon \halffilter^T \Whalf^{-1} \halffilter, \\
\nonumber
\text{s.t. } P\bm{1} \cdot \halffilter = 1, 
\end{gather}
where
\begin{equation*}
    \tilde{A} = P U^T W_T U P^T, \qquad \Whalf = P W_K P^T.
\end{equation*}
The effect of multiplying $U$ by $P^T$ is to ``fold $U$ in half'' and to sum the matching columns. This is the form of the problem that we will use in our proofs.

Computationally, we can fully handle the constraints by including $\bm{1}\cdot \filter = 1$ in the projection. We do this by changing variables to a vector $\xibf\in\Rbb^{K}$ (see Sidi \cite{Sidi2017}, pp 41)
\begin{equation*}
    c_k = P_{\xi} \xibf + \ebf_K,
\end{equation*}
where $\ebf_K$ is the $K$th unit vector and
\begin{equation*}
     P_{\xi} = \begin{pmatrix}
        1 & -1 & & & & & & -1 & 1\\
         & \ddots & \ddots & & & & \iddots & \iddots  \\
         & & 1 & -1 & & -1 & 1 \\
         & & & 1 & -2 & 1
    \end{pmatrix}.
\end{equation*} 
Clearly, we have $P_{\xi} \bm{1} = 0$ and that $(P_{\xi})_{k\ell} = (P_{\xi})_{k,-\ell}$, so every constraint is satisfied. We can substitute this into our least-squares problem, giving
\begin{equation}
\label{eq:lsqr-practical}
    R^2 = \min_{\xibf \in \Rbb^{K}}  \norm{\begin{pmatrix}
        W_T^{1/2} U \\ \epsilon^{1/2} W_{K}^{-1/2}
    \end{pmatrix}P_\xi \xibf + \begin{pmatrix}
        W_T^{1/2} U \ebf_0 \\ \epsilon^{1/2} W_{K}^{-1/2} \ebf_0
    \end{pmatrix}}^2.
\end{equation}
We solve this system via a direct QR-based least squares solve, as this is reliably accurate and typically fast enough for the system sizes considered. 

We note that the system could alternatively be solved via an iterative least-squares solver such as LSQR \cite{paige1982}. The matrices $P_\xi$, $W_T^{1/2}$, and $W_{K}^{-1/2}$ can all be applied in $\Ocal(T)$ time. Additionally, the matrix $U$ can be applied $\Ocal(T\log T)$ time via fast Hankel multiplications using the fast Fourier transform. So, an iterative algorithm would have a worst-case run time $\Ocal(TK\log T)$ operations, rather than the $\Ocal(TK^2)$ time to perform the QR-based algorithm. Additionally, in the case that $K$ is chosen much larger than necessary, the iterative algorithm converges in many fewer steps. However, we have not yet found an appropriate preconditioner for this method: a necessary step for convergences to high tolerances.

In total, an algorithm for finding a filter is given below:
\begin{algorithm}[H]
\caption{Reduced Rank Extrapolation}
\label{alg:RRE}
\begin{algorithmic}[1]
\Require Initial point $\xbf_0$, symplectic map $\sympmap$, least squares dimensions $T$ and $K$, regularization $\epsilon$
\State Sample trajectory $\abf_t$ via repeated evaluations of $\sympmap$
\State Compute $\ubf_t$ and weights for $W_T$ and $W_K$
\State Solve \eqref{eq:lsqr-practical} for $\xibf$ via direct QR or iterative LSQR solver
\State Compute $\filter = P_\xi \xibf$ and $R$ from \eqref{eq:lsqr-practical}
\Ensure Best filter $\filter$ and residual $R$
\end{algorithmic}
\end{algorithm}

The above algorithm directly inherits convergence rates of the weighted Birkhoff average. 
\begin{theorem}
\label{thm:RRE-residual-convergence}
    Under Hypotheses \ref{setting}, the residual of \eqref{eq:lsqr1} converges independent of how $T$ depends on $K$ as
    \begin{equation}
    \label{eq:RRE-convergence-rate}
        \epsilon \leq R^2 \leq \epsilon + C_m (2K)^{-2m},
    \end{equation}
    where $m$ and $C_m$ are identical to Thm.~\ref{thm:Das2018}.
\end{theorem}
\begin{proof}
    Consider the solution $c_k = \tilde{w}_{k,K}$. By construction, the filter obeys the constraints. Using Thm.~\ref{thm:Das2018}, $\abs{(U\filter)_t} \leq C_m (2K+1)^{-m}$. So,
    \begin{equation*}
        \filter^T U^T W_T U \filter = \sum_{t=0}^{T-1} w_{t,T} (U\filter)_t^2 \leq C_m (2K)^{-2m}.
    \end{equation*}
    Similarly, the regularization term evaluates exactly as $\filter^T W_K^{-1} \filter = \epsilon$. Combining these computations, we have the upper bound.

    For the lower bound, we consider $\min_{\filter} \filter^T W_K^{-1} \filter \leq R$. Enforcing the $\bm{1} \cdot \filter = 1$ constraint with a Lagrange multiplier $\lambda$ and the palindromic constraint explicitly, the minimizer is found to solve the linear system
    \begin{equation*}
        \tilde{w}_{k,K}^{-1} c_k + \lambda = 0, \quad \sum_{k} c_k = 1.
    \end{equation*}
    This is solved via $c_k = \tilde{w}_{k,K}$ and $\lambda = -2$, the same solution as considered for the upper bound. Substituting $c_k$ back into the least-squares problem gives the lower bound.
\end{proof}
From \eqref{eq:RRE-convergence-rate}, we see that the extrapolation method converges at least as fast as the weighted Birkhoff average, particularly when $\epsilon = 0$. This means that we can also use the convergence of RRE to distinguish between chaotic and non-chaotic trajectories. 

Because the above theorem does not depend on $T$, it does not have any stronger lower bound. Practically, it is required that $Td$ be greater than or equal to $K$ for a full rank linear system. This is an important requirement to ensure that chaotic trajectories do not converge. However, to our knowledge, there is currently no theorem here or in the weighted Birkhoff average literature proving that chaotic trajectories cannot be accelerated, despite strong numerical evidence. We will similarly give no proofs for the extrapolation method in chaos.

In order to classify chaos efficiently, we also consider an adaptive algorithm. For this, we first define the scale-free residual $R_{G}$ as
\begin{equation}
\label{eq:RG}
    R_G = \frac{\sqrt{R^2-\epsilon}}{G}, \quad G^2 = \sum_{t = 0}^{T-1} w_{t,T} \abs{\ubf_t}^2 = \WBA[\abs{\dobs}^2](\xbf_0).
\end{equation}
Because $G$ converges to a nonzero number with $T$ (assuming $\xbf_0$ is not a fixed point), $R_G$ converges at the same rate as $R$. 
For the adaptive algorithm, we increase $K$ from an initial value $K_{\min}$ to a maximum value $K_{\max}$ by an increment of $\Delta K$.
We assume that $T$ scales with $K$ as $T = \ceil{\gamma K/d}$ for some constant $\gamma \geq 1$. 
At each increment, we check whether $R_G < \delta$, and finish the algorithm when this conditions is met.
The fact that $R_G$ is scale-free allows for the algorithm to be applied to multiple orbits for the same map with an accuracy to match the largest scale of the system.
In total, the adaptive algorithm is below:
\begin{algorithm}[H]
\caption{Adaptive Reduced Rank Extrapolation}
\label{alg:adaptiveRRE}
\begin{algorithmic}[1]
\Require Initial point $\xbf_0$, symplectic map $\sympmap$, regularization $\epsilon$, $T$ proportionality constant $\gamma$, convergence cutoff $\delta$, initial $K$ value $K_{\mathrm{init}}$, maximum $K$ value $K_{\max}$, $K$ increment $\Delta K$
\State $K \gets K_{\mathrm{init}}$, $T \gets \ceil{\gamma K/d}$
\While {$K \leq K_{\max}$ and $R_G > \delta$}
    \State Get $\filter$, $R$ via Algorithm \ref{alg:RRE}, reusing trajectory information
    \State Get $R_G$ via \eqref{eq:RG}
    \State $K \gets K + \Delta K$, $T \gets \ceil{\gamma K/d}$
\EndWhile
\Ensure Best filter $\filter$ and residual $R$
\end{algorithmic}
\end{algorithm}
With large enough steps $\Delta K$, the cost of not using matrix updates mostly avoided. Additionally, if one used a doubling method of incrementing $K$, the asymptotic costs are reduced to a logarithmic factor in $K_{\mathrm{max}}$. 

\subsection{Processing the Learned Filter}
\label{subsec:33}
Once we have found a filter $\filter$ for the sequence of observations for a trajectory, the next step is to process the signal. There are two steps to this process. The first is simple: we distinguish chaotic trajectories from non-chaotic trajectories via a tolerance for the residual. For simplicity, we typically use the same tolerance as in Algorithm \ref{alg:adaptiveRRE}. If the residual is above the tolerance, we deem the trajectory ``chaotic,'' and otherwise it is an invariant circle or an island. We note that choosing the tolerance for a specific problem depends on the desired accuracy, the tolerable amount of computation, and the accuracy of the $\sympmap$ evaluation. However, any error in the computation of $\filter$ will lead to more difficulty in the following steps, so lower tolerances are always more reliable in RRE.

For this section, we will use the following result about the convergence of the roots of $\filter$:
\begin{theorem}
\label{thm:least-squares}
    Under Hypotheses \ref{setting}, let $\filter_K$ be a sequence of solutions to \eqref{eq:LeastSquares} with $T = \ceil{\gamma K}$ for $\gamma \geq 1$ and let $P_K(z)$ be the filter polynomial with coefficients $\filter_K$. Then, for all $M_\perp \in \Nbb$, $M_T \in \Nbb$ satisfying $M > d + M_T \nu$, and $n$ such that $\abs{\dobsT_n} \neq 0$, there exists a sequence $z_{K,n}$ such that $P_K(z_{K,n}) = 0$ and
    \begin{equation}
    \label{eq:lambdaconvergence}
        \abs{\lambda_n - z_{K,n}} < C_n K^{-M_*}
    \end{equation}
    where 
    \begin{equation*}
        M_* = \min\left(\frac{2M - d}{2M/\Mperp + \nu} , \ M_T \right).
    \end{equation*}
\end{theorem}
\begin{remark}
    If $M = \infty$, Equation \eqref{eq:lambdaconvergence} holds for all $M_* \in \Nbb$.
\end{remark}
The above theorem essentially states that the roots of the filter necessarily approach the points $\lambda_n$ associated with multiples of the rotation number and the island period. 
The proof of this theorem is given in App.~\ref{subsec:46}, using the results developed throughout App.~\ref{sec:proofs}.


In the case that we deem the trajectory non-chaotic, our next step is to find the spectrum of the filter. 
This is done by solving the equation
\begin{equation*}
    P_K(\lambda) = \sum_{k = 0}^{2K} c_k \lambda^k = 0,
\end{equation*}
for every root $\lambda_j$. We do this by reducing the polynomial to another Chebyshev polynomial with half the dimension, then solving for the eigenvalues of the associated colleague matrix \cite{good1961} (see App.~\ref{app:palindromic-roots}). Due to the majority of eigenvalues being on the unit circle, this eigenvalue problem is well conditioned. The only exception to this is when $\lambda = -1$ is a root, as happens with $p=2$ islands. In this case, the palindromic coefficients force $-1$ to be a double root, causing a square root of the error of this frequency. 

Throughout the rest of this section, we assume that $d=1$ and therefore the trajectory is either an invariant circle or a $d=1$ island.
Now that we have the roots $\lambda_j$, the next step is to determine which roots represent the majority of the signal.
This step is heuristic: we assume that the low-frequency oscillations will dominate the Fourier spectrum, so we can use this information to prune the important frequencies from the less important ones. To do this, we first restrict to values of $\lambda_j$ that are very close to the unit circle by some tolerance on the order of the square root of machine epsilon (due to the aforementioned sensitivity of $-1$ as a root). The remaining eigenvalues are sorted by solving the weighted least-squares system for each eigenvalue's prominence in the signal
\begin{equation*}
    W_T^{1/2} \tilde \Phi V = W_T^{1/2} A,
\end{equation*}
where
\begin{equation*}
    \tilde \Phi = 
    \begin{pmatrix}
        \lambda_0^0 & \dots & \lambda_{2K}^0 \\
        \vdots & & \vdots \\
        \lambda_0^{T} & \dots & \lambda_{2K}^{T}
    \end{pmatrix}, \quad A = \begin{pmatrix}
        \abf_0^T \\ \vdots \\ \abf_{T+2K}^T
    \end{pmatrix}.
\end{equation*}
The eigenvalues are then sorted by the value of norm of the rows of $V$.

Using the top few eigenvalues (arbitrarily chosen to be $10$), the next step is to determine if the sequence corresponds to an island. We do this by noticing a key difference between a $p\geq 2$ island and a Diophantine invariant circle: the island spectrum \eqref{eq:a-island} has rational frequencies whereas the invariant circle \eqref{eq:a-sequence} does not. So, if the sequence is an island, we expect a prominent rational frequency $\omega_j = (2\pi i)^{-1} \arg \lambda_j$ in the sorted eigenvalues. For this, we use a Farey-sequence method from \cite{sander2020} (Algorithm 2) to determine whether a given root is rational to a specified tolerance $\epsilon_{\mathrm{rat}}$ and bounded denominator $p \leq p_{\max}$. If one of the roots is rational by this algorithm, we consider it to be an island chain with the largest found period $p$. From here, we can rerun Algorithm \ref{alg:RRE} on the ``stacked'' signal with dimension $\hat{d} = p d$
\begin{equation*}
    \hat{\abf}_t = \begin{pmatrix}
        \abf_{pt} \\ \abf_{pt+1} \\ \vdots \\ \abf_{pt+p-1}
    \end{pmatrix},
\end{equation*}
with a filter length $\hat{K} = \floor{K/d}$.
Using this signal is equivalent to working simultaneously with the $p$ invariant circles of $\sympmap^p$ with the same rotation number. The resulting filter will be that of an invariant circle and the above steps can be repeated, skipping the step of checking for rational roots.

Now, consider the case that no rational roots of the filter are found. In order to determine the rotation number, we simply choose the frequency that appears first in the sorted eigenvalues, i.e. $\omega = (2\pi i)^{-1} \arg(\lambda_0)$ where $\lambda_0$ is the first eigenvalue after sorting. We note that this is not always true: invariant circles can be found where the largest Fourier coefficient does not correspond to the rotation number. However, we have not found this practically to be an issue for any of our examples.

Once the rotational frequency $\omega$ is determined, we can obtain the coefficients of the invariant circle associated with the signal by solving another linear system. This time, because typically $\omega$ is resolved to very high accuracy, we solve the linear system
\begin{equation}
\label{eq:circle-projection}
     W_T^{1/2} \Phi V = W_T^{1/2} A,
\end{equation}
where 
\begin{equation*}
    \Phi = 
    \begin{pmatrix}
        \lambda_1^0 & \lambda_1^0 %& \lambda_1^0 
        & \dots & \lambda_1^0 \\
        \lambda_1^{-L} & \lambda_1^{-L+1} %& \lambda_1^{-L+2} 
        & \dots & \lambda_1^{L} \\
        % \lambda_1^{-2L} & \lambda_1^{-2L+2} & \lambda_1^{-2L+4} & \dots & \lambda_1^{2L} \\
        \vdots & \vdots & \vdots & \ddots & \vdots \\
        \lambda_1^{-LT} & \lambda_1^{T(-L+1)} %& \lambda_1^{T(-L+2)} 
        & \dots & \lambda_1^{LT} \\
    \end{pmatrix}, \quad \lambda_1 = e^{2\pi i \omega},
\end{equation*}
and $L$ is the number of coefficients wanted, chosen to control the condition number of the least-squares problem (see Sec.~\ref{app:choosing-L}).
The approximated invariant circles are then given as
\begin{equation*}
    \zbf^{(j)}(\theta) = \sum_{\ell = -L}^L V_{\ell,d(j-1):dj-1}e^{2\pi i \ell \theta},
\end{equation*}
where we are using `Matlab notation' for slicing the rows of $V$ into each island component. 

Once an invariant circle or island chain is found, the fit can be validated via a residual from the parameterization. 
In particular, we can evaluate the residual
\begin{align}
\nonumber
    R_p^2 &= \frac{1}{pJ} \sum_{j=0}^{J-1} \left(\vphantom{\sum_{j=1}^{p-1}}\abs{\zbf^{(1)}(j h + \omega) - \sympmap(\zbf^{(p)}(j h))}^2\right. \\
    &\quad \qquad \qquad +  \left.\sum_{j = 1}^{p-1} \abs{\zbf_{(j+1)}(hj) - \sympmap(\zbf^{(j)}(hj))}^2 \right), \\
\label{eq:validation-error}
    &\approx \frac{1}{p} \left(\vphantom{\sum_{j=1}^{p-1}}\int_{\Tbb}\abs{\zbf^{(1)}(\theta + \omega) - \sympmap(\zbf^{(p)}(\theta))}^2 \dif \theta\right.\\
    & \quad \qquad \qquad + \left.\sum_{j = 1}^{p-1} \int_{\Tbb}\abs{\zbf_{(j+1)}(\theta) - \sympmap(\zbf^{(j)}(\theta))}^2 \dif \theta \right),
\end{align}
where $h = 1/J$ for $J \in \Nbb$. The residual $R_p$ is essentially an $L^2$ measurement of the conjugacy \eqref{eq:island-conjugacy}. If this residual is small, then the conjugacy is likely correct. Furthermore, a small $R_p$ likely puts the island within the basin of convergence for the parameterization method \cite{haro2016}, which could be used to refine the estimate of the island. Thus, Birkhoff RRE could be seen as a method of finding an initial guess for higher-accuracy methods.

==> Deprecated/Sections/4proof.tex <==
\section{Proofs}
\label{sec:proofs}
In this section, we will prove that as $K$ and $T$ increase, the frequencies of the filter polynomial solutions of \eqref{eq:LeastSquares} applied to islands go to the frequencies appearing in \eqref{eq:a-island}, i.e.
\begin{equation*}
    \omega_{m\nbf} = \frac{\nbf \cdot \omega + m}{p}, \qquad \nbf \neq 0, \qquad 0 \leq m < p.
\end{equation*}
With this notation, the sequence $\ubf_t$ on islands can be written as a Fourier series
\begin{equation*}
    \ubf_t = \sum_{m = 0}^{p-1} \sum_{\nbf\in\Zbb^d \backslash\{0\}} \dobsT_{m\nbf} \lambda_{m\nbf}^t, \qquad \lambda_{m\nbf} = e^{2\pi i \omega_{m\nbf}}.
\end{equation*}

It is convenient to be able to transform between the above multi-index $(m,\nbf)$ and a linear ordering of the frequencies over $\Zbb$. Let $\Pi : n \mapsto (m,\nbf)$ be the bijective indexing over the integers and $\Pi_{\nbf} : n\mapsto \nbf$ be the projected ordering onto $\nbf$. We require two things of the bijection:
\begin{enumerate}
    \item Conjugacy symmetry $\Pi(n) = - \Pi(-n)$, and
    \item Monotonicity in $\nbf$: $\norm{\Pi_{\nbf}(n)}_{\infty} \leq \norm{\Pi_{\nbf}(n')}_{\infty}$ for $\abs{n} < \abs{n'}$. 
\end{enumerate}
Otherwise, the ordering is arbitrarily fixed (say, lexicographically). 
Note that the conjugacy symmetry implies that $\Pi(0) = (0,0)$. 
Using the 1D ordering, we use the abbreviated notation
\begin{equation*}
    \omega_n = \omega_{\Pi(n)}, \quad \lambda_n = \lambda_{\Pi(n)}, \quad \dobsT_n = \dobsT_{\Pi(n)}, \quad \text{etc.}
\end{equation*}

The monotonicity condition is important for translating the convergence of multi-indices to convergence in the single index. 
In particular, the ordering tells us that
\begin{equation*}
    \norm{\Pi_{\nbf}(n)}_\infty = \begin{cases}
        0 & \abs{n} = 0, \\
        1 & 0 < \abs{n} \leq \frac{3^d-1}{2}, \\
        \vdots & \vdots \\
        m & \frac{(2m-1)^d - 1}{2} < n \leq \frac{(2m+1)^d-1}{2}, \\
        \vdots & \vdots
    \end{cases}
\end{equation*}
In this way, $\norm{\Pi_{\nbf}(n)}_{\infty} \sim c_{\infty} n^{1/d} $. From this, there are equivalent bounds for any other norm on $\Pi_{\nbf}(n)$, which we use for rates of convergence of Fourier series in the $2$-norm.




To motivate the steps in the following sections, we first consider the problem of polynomial perturbation alone.
Let $\halffilter = P^T \filter$ be a palindromic filter with roots $\lambda_n$ on the unit circle for $1 \leq \abs{n} \leq K$. 
Then, evaluation of the associated polynomial is a linear function of the coefficients:
\begin{equation*}
    P_K(\lambda_n) = \lambda_n^K \bm \phi_n^T \halffilter = 0,
\end{equation*}
where
\begin{equation*}
    \bm \phi_n = \bm \phi_{m\nbf} = \begin{pmatrix}
        1 \\ \sqrt{2} \cos(2\pi \omega_n) \\ \vdots \\ \sqrt{2} \cos(2 \pi K \omega_n)
    \end{pmatrix} = P \begin{pmatrix}
        \lambda_n^{-K} \\ \vdots \\ \lambda_n^{-1} \\ 1 \\ \lambda_n \\ \vdots \\ \lambda_n^K
    \end{pmatrix}.
\end{equation*}
Now, we consider how the root $\lambda_n$ is perturbed when we perturb $\halffilter$ by an amount $\delta \halffilter$. Letting the perturbation of $\lambda_n$ be $\delta \lambda_n$, a direct application of chain rule finds
\begin{equation}
\label{eq:eval-perturbation}
    \delta \lambda_n = -\frac{\bm \phi_n^T \delta \halffilter}{\pd{\lambda_n^K \bm \phi_n^T}{\lambda_n} \halffilter} = - \frac{\delta P_K(\lambda_n)}{P_K'(\lambda_n)},
\end{equation}
where $\delta P_K$ is the polynomial with coefficients $\delta \halffilter$. So, if we want to show that a root is not strongly perturbed, we have two simultaneous goals:
\begin{enumerate}
    \item We must bound $\bm \phi_n^T \delta \halffilter$ so that it is small, and
    \item We must bound $P_K'(\lambda_n)$ away from zero.
\end{enumerate}
We note that we do not have to specifically bound $\delta \halffilter$ so that it is small. Rather, we must make sure the perturbation is only large in a direction orthogonal to the vector $\bm \phi_n$.

In order to find the perturbation $\delta \halffilter$, we perturb the least squares problem \eqref{eq:LeastSquares}. Solving the system with $\halffilter = \halffilter_0 + \delta \halffilter$ under the assumption that $\bm \phi_0^T \halffilter_0 = 1$ and $\bm \phi_n^T \halffilter_0 = 0$, we find
\begin{equation*}
    \delta \halffilter = - \halffilter_0 + \frac{(\tilde A + \epsilon \Whalf)^{-1}\bm \phi_0}{\bm \phi_0^T (\tilde A + \epsilon \Whalf)^{-1}\bm \phi_0}.
\end{equation*}
Substituting this into the eigenvalue perturbation formula \eqref{eq:eval-perturbation}, we find that
\begin{equation*}
    \delta \lambda_n = - \frac{1}{P'_K(\lambda_n)} \frac{\bm \phi_n^T (\tilde A + \epsilon \Whalf)^{-1}\bm \phi_0}{\bm \phi_0^T (\tilde A + \epsilon \Whalf)^{-1}\bm \phi_0}.
\end{equation*}



The key insight of the proof is showing that the modes $\bm \phi_n$ are nearly orthogonal under the inner product defined by $W_K$. 
That is, if we let $\dbf = \Whalf^{-1/2} \halffilter$ and $\tilde{B} = \Whalf^{1/2} \tilde{A} \Whalf^{1/2}$, we have the new least-squares problem
\begin{equation}
\label{eq:transformedleastsquares}
    \min_{\dbf} \dbf^T (\tilde{B} + \epsilon I) \dbf, \qquad \text{s.t. } \bm \psi_0^T \dbf = 1,
\end{equation}
where $\bm \psi_n = \Whalf^{1/2} \bm \phi_n$ and we have used the identity $\bm \psi_0 = \Whalf^{1/2} P \bm{1}$ for the constraint. 
In this new basis, polynomial evaluation is equivalent to evaluating $\bm \phi_n^T \halffilter = \bm \psi_n^T \dbf$. 
Additionally, the eigenvalue perturbation becomes
\begin{equation}
\label{eq:lambda-perturbation}
    \delta \lambda_n = - \frac{1}{P'_K(\lambda_n)} \frac{\bm \psi_n^T (\tilde B + \epsilon I)^{-1}\bm \psi_0}{\bm \psi_0^T (\tilde B + \epsilon I)^{-1}\bm \psi_0}
\end{equation}
In the following sections, we show the matrix $\tilde B$ is approximately diagonalized in the basis of $\bm \psi_n$, implying the right term in the above formula is small. 

We start in Sec.~\ref{subsec:41} where we show that as $T$ grows, the normal matrix approaches a normal matrix from the continuous problem. Then, we show that as $K$ grows, errors associated with the decay of Fourier coefficients of $\dobsT$ (Sec.~\ref{subsec:42}) and the orthogonality of the modes $\bm \psi_n$ (Sec.~\ref{subsec:43}) also decay sufficiently fast. These matrix perturbation bounds are then combined in Sec.~\ref{subsec:44} to obtain Thm.~\ref{thm:SVD}, a subspace perturbation theorem for the normal matrix. 
Finally, the results are combined in the proof of Thm.~\ref{thm:least-squares}, given in Sec.~\ref{subsec:46}.


\subsection{Choosing $T$ via Birkhoff average convergence}
\label{subsec:41}

This section links the finite-time least square problem
\eqref{eq:LeastSquares} 
to the invariant measure least squares problem 
\eqref{eq:filter-l2-norm}. 
In particular, the finite time normal matrix is
\begin{equation*}
    \tilde{A} = P U^T W_T U P^T, 
\end{equation*}
where 
\begin{equation*}
    (U^T W_T U)_{mn} = \WBA_T[(\dobs\circ\sympmap^m)\cdot(\dobs\circ\sympmap^n)](\xbf_0)
\end{equation*}
and we assume that $\xbf_0$ is in an island. We will compare the error of $\tilde{A}$ when compared against the infinite-time normal matrix defined as
\begin{equation*}
    E_{TA} = \tilde{A} - A, \qquad A = P A_{\infty} P^T,
\end{equation*}
where
\begin{equation*}
    (A_{\infty})_{mn} = \BA[(\dobs\circ\sympmap^m)\cdot(\dobs\circ\sympmap^n)](\xbf_0).
\end{equation*}
When expanded in Fourier series, the matrix $A$ becomes
\begin{equation*}
    A = \sum_{n =1}^\infty 2 \abs{\dobsT_n}^2 \bm \phi_n \bm \phi_n^T.
\end{equation*}


The term $E_{TA}$ is the error introduced by the Birkhoff average used to find the elements of $A$, and depends on the value of $T$ and the initial point on the orbit $\xbf_0$. Specifically, the error has the form
\begin{align}
\label{eq:Ecoef}
    E_{TA} = P (U^T W_T U - A_\infty) P^T,
\end{align}
where
\begin{multline*}
     (U^T W_T U - A_\infty)_{mn} = \WBA_T[(\dobs\circ\sympmap^m)\cdot (\dobs\circ\sympmap^n)](\xbf_0) \\- \BA[(\dobs\circ\sympmap^m)\cdot(\dobs\circ\sympmap^n)](\xbf_0).
\end{multline*}
We can bound $E_{TA}$ in Frobenius norm as:
\begin{lemma}
\label{lemma:ET_entrywise}
    Under Hypotheses \ref{setting} (H1-2), there exists a constant $C_{T,M_T}$ independent of $k$ and $\ell$ such that
    \begin{equation}
    \label{eq:ET_entrywise}
        \abs{E_{TA, k\ell}} \leq C_{T,M_T} T^{-M_T},
    \end{equation}
    provided that $M > d + \nu M_T$.
\end{lemma}
\begin{proof}
    The weighted Birkhoff average in \eqref{eq:Ecoef} is expanded as 
    \begin{equation*}
        (U^T W_T U)_{mn} = \sum_{t = 0}^{T-1} w_{t,T} \ubf_{m+t} \cdot \ubf_{n+t},
    \end{equation*}
    where the signal $\ubf_{m+t}\cdot \ubf_{n+t}$ can be written in terms of the Fourier series as
    \begin{equation*}
        \ubf_{m+t}\cdot \ubf_{n+t} = \sum_{k, \ell\in\Zbb}\dobsT_k \cdot \dobsT_\ell \lambda_k^{m+t} \lambda_\ell^{n+t} = \sum_{k\in\Zbb} U_{k,m,n}\lambda_k^t.
    \end{equation*}
    Using the convolutional structure of the second equality above, one can show that $U_{k,m,n}\leq C_{U,M} k^{-M}$ where $C_{U,M}$ is independent of $m$ and $n$. The proof of Thm.~\ref{thm:Das2018} only depends on the decay rates of these coefficients, so Thm.~\ref{thm:Das2018} implies the bound \eqref{eq:ET_entrywise} independent of $m$ and $n$.
    
    % \mr{The below is slightly wrong and for the invariant circle case, because of the sum not including $m=0,n$. However, none of this is really interesting anyway. In the end, I think we should remove all of this.
    
    % We can write the Fourier series of $\dobsT(\cdot) \dobsT(\cdot + \bm \phi)$ as a convolution:
    % \begin{equation*}
    %     \dobsT(\theta)^T \dobsT(\theta + \bm \phi) = \sum_{n \in \Zbb} \left[\sum_{m \in \Zbb} e^{2\pi i m \bm \phi} \dobsT_{m}^T \dobsT_n \right] e^{2\pi i n \theta} = \sum_{n\in\Zbb} \tilde{g}_n e^{2\pi i n \theta}.
    % \end{equation*}
    % Because $\dobsT \in C^{M}$, we have a coefficient $C_{g,M}$ such that $\abs{\dobsT_n} < C_{g,M} \abs{n}^{-M}$. Using this, we can bound $\tilde{g}_{n}$ as
    % \begin{equation*}f
    %     \abs{\tilde{g}_n} \leq C_{g,M}^2 \sum_{m\in\Zbb \backslash \{0, n\}} \abs{m}^{-M} \abs{n-m}^{-M} = C_{g,M}^2 \sum_{m \in \Zbb \backslash \{0, n\} } \abs{m(n-m)}^{-M}.
    % \end{equation*}
    % We can bound the above sum by integrals for $n>2$:
    % \begin{align*}
    %     \abs{\tilde{g}_n} &< 2 C^2_{g,M} \left[2 (n-1)^{-M} + \int_{1}^{n/2} (x(n-x))^{-M} \dif x + \int_{1}^\infty (x(x+n))^{-M} \dif x   \right] ,\\
    %     &< 4 C^2_{g,M}\left[2 (n-1)^{-M} + \left((2^{M})+1\right)n^{-M} \int_{1}^{\infty} x^{-M} \dif x \right],\\
    %     &< C_{\tilde{g},M}n^{-M}.
    % \end{align*}}
\end{proof}
\begin{remark}
    Here and throughout this paper, constants suppress information about $\dobsT$, $\omega$, and the bump function $w$. They never suppress information on system size.
\end{remark}

From here, we consider the perturbation in the weighted least squares problem \eqref{eq:transformedleastsquares}:
\begin{equation*}
    \tilde{B} = B + E_T, 
\end{equation*}
where
\begin{equation*}
    E_T = \Whalf^{1/2} E_{TA} \Whalf^{1/2}, 
\end{equation*}
and
\begin{equation*}
    B = \Whalf^{1/2} A \Whalf^{1/2} = \sum_{n=1}^\infty 2 \abs{\dobsT_n}^2 \bm \psi_n \bm \psi_n^T.
\end{equation*}
The perturbation of $B$ can be bounded in Frobenius norm using our previous result:
\begin{lemma}
\label{lemma:ET}
    Under the same conditions as Lemma \ref{lemma:ET_entrywise}, we have
    \begin{equation*}
        \norm{E_T}_F \leq C_{T,M_T} T^{-M_T}.
    \end{equation*}
\end{lemma}
\begin{proof}
    Directly calculating the norm:
    \begin{align*}
        \norm{E_T}^2_F &= \norm{\Whalf^{1/2} E_{TA} \Whalf^{1/2}}^2_F, \\
        &= \sum_{k, \ell = 0}^{K} E_{TA,k\ell}(\Whalf)_{kk}(\Whalf)_{ll}, \\
        & \leq C_{T,M_T}^2 T^{-2M_T}\sum_{k, \ell = 0}^{2K} \tilde{w}_{k,K} \tilde{w}_{\ell,K}, \\
        &= C_{T,M_T}^2 T^{-2M_T}.
    \end{align*}
\end{proof}



\subsection{Bounding the tail error}
\label{subsec:42}
From here, we are interested in showing that the perturbation of $B$ with respect to the rank $N \leq K$ subspace
\begin{equation*}
    E_B = B - \Psi \Sigma^2 \Psi^T
\end{equation*}
is small in some norm, where 
\begin{equation*}
    \Psi = \begin{pmatrix}
        \bm \psi_1 & \dots & \bm \psi_N
    \end{pmatrix}, \qquad \Sigma^2 = \begin{pmatrix}
        \sigma_1^2 \\ 
         & \ddots \\
         &  & \sigma_N^2
    \end{pmatrix},
\end{equation*}
and
\begin{equation*}
    \sigma_j^2 = 2\abs{\dobsT_j}^2.
\end{equation*}
A bound on $E_B$ shows that if $N$ is large enough, the linearly independent modes in $\Psi$ capture most of the Fourier content of $\dobsT$. 

\begin{lemma}
\label{lemma:EB}
    If $\dobsT \in C^{M}$ with Fourier coefficient bounds $\abs{\dobsT_{m\nbf}} \leq C_{g,M} \norm{\nbf}^{-M}$, we have for some constant $C_B$
    \begin{equation*}
        \norm{E_B}_F < C_{B} N^{-2M/d+1}
    \end{equation*}
\end{lemma}
\begin{proof}
    By the triangle inequality,
    \begin{equation*}
        \norm{E_B}_F \leq \sum_{n > N} 2 \abs{\dobsT_n}^2 \norm{\bm \psi_n\bm \psi_n^T}_F = \sum_{n > N} 2 \abs{\dobsT_n}^2 \norm{\bm \psi_n}_2^2.
    \end{equation*}
    Looking at the $\norm{\bm \psi_n}_2^2$ term, we have
    \begin{equation}
    \label{eq:psi_norm}
        \norm{\bm \psi_n}^2_2 = \frac{\sum_{k = -K}^K \WBAw(k / (K+1)) \cos^2(2\pi k \omega_n)}{\sum_{k=-K}^K \WBAw(k/(K+1))} < 1.
    \end{equation}
    For the sum over $\abs{\dobsT_n}^2$, we note that the multi-indexing monotonicity condition gives the bound 
    \begin{align*}
        \norm{\dobsT_n}^2 &= \norm{\dobsT_{\Pi(n)}}^2, \\
        &\leq C_{g,M} \norm{\Pi(n)}^{-2M}, \\
        &\leq C_{2} n^{-2M/d}.
    \end{align*}
    Using this, we find
    \begin{align}
    \nonumber
        \sum_{n > N} \abs{\dobsT_n}^2 &< \int_{N}^\infty C_{g,M}^2 x^{-2M/d} \dif x, \\
    \nonumber
        &= C_{g,M}^2 \left[ \frac{x^{-2M/d+1} d}{-2M+d} \right]_{N}^{\infty}, \\
    \label{eq:g_tail_energy}
        &= \frac{dC_{g,M}^2}{2M-d} N^{-2M/d+1}.
    \end{align}
    Combining \eqref{eq:psi_norm} and \eqref{eq:g_tail_energy} and letting $C_B = \frac{dC_{g,M}^2}{2M-d}$, we have our result.
\end{proof}

\subsection{Error of approximate orthogonalization}
\label{subsec:43}

In this section, we show that as $K$ grows, $\Psi$ approaches orthonormality. First, we bound the error of individual inner products $\ip{\bm \psi_n}{\bm \psi_m}$ for $0 \leq n,m \leq N$ away from the Kronecker delta $\delta_{nm}$. One can view this as a statement about aliasing for our specific set of frequencies. Then, we use this to bound the difference of $B$ from a orthonormal matrix. For the first step, we first need the following lemma:
\begin{lemma}[Poisson summation formula] 
\label{lemma:PoissonSummation}
For each $f \in L^2(\Rbb)$,
\begin{equation*}
    \sum_{n\in\Zbb} f(n) = \sum_{n\in\Zbb} \int_{\Rbb}f(x) e^{-2\pi i n x} \dif x.
\end{equation*}
\end{lemma}

We start with a helper lemma:
\begin{lemma}
\label{lemma:lambda-orthogonality}
    Under Hypotheses \ref{setting} H1 and H2, for all $\Mperp \in \Nbb$ there are constants $C_{\lambda, \Mperp} > 0$ independent of $n$ such that
    \begin{equation*}
        \abs{S_{m\nbf} - \delta_{(m,\nbf),0}} < C_{\lambda, \Mperp} \norm{\nbf}^{\Mperp \nu} K^{-\Mperp},
    \end{equation*}
    where 
    \begin{equation*}
        S_{m\nbf} = \sum_{t=0}^{T-1} \WBAw_{t,T} \lambda_{m\nbf}^t, \quad \delta_{(m,\nbf),0} = \begin{cases}
            1 & m = 0 \text{ and } \nbf = 0, \\
            0 & \text{else}.
        \end{cases}
    \end{equation*}
\end{lemma}
\begin{proof}
    Applying the Poisson summation formula, we have
    \begin{align*}
        S_{m\nbf} &= \frac{1}{A_K}\sum_{t \in \Zbb} \int_{\Rbb} \WBAw\left(\frac{x}{K+1}\right) e^{2\pi i (\omega_{m\nbf}-t) x}\dif x,\\
        &= \frac{K+1}{A_K} \sum_{t\in\Zbb} \int_{-1}^1 \WBAw(x) e^{2\pi i  (K+1) (\omega_{m\nbf} - t) x} \dif x,
    \end{align*}
    where
    \begin{equation*}
        A_K = \sum_{t=0}^{T-1} w\left(\frac{t+1}{T+1} \right).
    \end{equation*}
    The factor $A_K$ scales as $K$, so for some constant $C_W$ we have $(K+1)/A_K < C_{W}$.

    From here, we can perform repeated integration by parts against $\WBAw$. Doing so, we have that
    \begin{align*}
        &\abs{\int_{-1}^1 \WBAw(x) e^{2\pi i  (K+1) (\omega_{m\nbf} - t) x} \dif x}\\
        &\qquad= (K+1)^{-\Mperp} \abs{2 \pi (\omega_{m\nbf} - t)}^{-\Mperp}\\
        &\quad \qquad \times \abs{\int_{-1}^1 \WBAw^{(\Mperp)}(x) e^{2\pi i  (K+1) (\omega_{m\nbf} - t) x} \dif x}, \\
        &\qquad \leq K^{-\Mperp} \abs{2\pi (\omega_{m\nbf} - t)}^{-\Mperp} \norm{\WBAw^{(\Mperp)}}_{L^1}.
    \end{align*}
    Going back to $S_{m\nbf}$, we have
    \begin{equation*}
        \abs{S_{m\nbf}} \leq  C_W \norm{\WBAw^{(\Mperp)}}_{L^1} K^{-\Mperp} \sum_{n \in \Zbb} \abs{2 \pi (\omega_{m\nbf} - t)}^{-\Mperp}.
    \end{equation*}
    To bound the sum, let $t_0$ be the closest integer to $m\omega$. Then,
    \begin{multline*}
        \sum_{t \in \Zbb} \abs{2 \pi (\omega_{m\nbf} - t)}^{-\Mperp} = \abs{2 \pi (\omega_{m\nbf} - t_0)} \\
        + \sum_{t \in \Zbb\backslash\{t_0\}} \abs{2 \pi (\omega_{m\nbf} - t)}^{-\Mperp}.
    \end{multline*}
    The term on the first line is bounded by an $O(\norm{\nbf}^{\Mperp(1+\nu)})$ Diophantine condition, while the rest of the sum is bounded by a constant. The Diophantine bound dominates, giving $\sum_t \abs{\omega_{m\nbf} - t}^{-\Mperp} \leq C_{\omega, \Mperp} \norm{\nbf}^{\Mperp(1+\nu)}$. Using this, we have our result.
    
\end{proof}


The above lemma serves as a numerical linear algebra reinterpretation of the results of the weighted Birkhoff average \cite{Das2018}. 
We note that it can easily be used to prove Thm.~\ref{thm:Das2018}:
\begin{proof}[Proof of Thm.~\ref{thm:Das2018}]
    Assuming a $C^M$ island chain, the signal can be written as 
    \begin{equation*}
        (\obs \circ \sympmap^t)(\xbf_0) = \sum_{m=0}^{p-1} \sum_{\nbf \in \Zbb^d }\obsT_{m\nbf} \lambda_{m\nbf}^t,
    \end{equation*}
    where $\abs{\obsT_{m\nbf}} < C \norm{\nbf}^{-M}$. Then, the average can be written as
    \begin{align*}
        \WBA_T[\obs](\xbf_0) &= \sum_{m=0}^{p-1} \sum_{\nbf \in \Zbb^d }\obsT_{m\nbf} \sum_{t=0}^{T-1}w_{t,T} \lambda_{m\nbf}^t,\\
        &= \sum_{m=0}^{p-1} \sum_{\nbf \in \Zbb^d }\obsT_{m\nbf} S_{m\nbf}.
    \end{align*}
    Applying Lemma \ref{lemma:lambda-orthogonality}, we find
    \begin{equation*}
        \abs{\WBA_T[\obs](\xbf_0) - \obsT_0} < p C_{\lambda,m} \sum_{n=1}^{\infty} \norm{\nbf}^{-M+m\nu}.
    \end{equation*}
    Using the condition that $M > d + m\nu$, we know the above sum converges, giving the result.
\end{proof}

Returning to the proof of the RRE root convergence, we can also look at the orthogonality of the $\bm \psi_m$ modes:
\begin{lemma}
\label{lemma:orthogonality}
    Under Hypotheses \ref{setting} (H1-2), for all $\Mperp \in \Nbb$ the basis vectors $\bm \psi_n$ and $\bm \psi_m$ are nearly orthonormal with constants $C_{\psi, \Mperp} > 0$ independent of $n$ and $m$ as
    \begin{equation*}
        \abs{\bm \psi_n^T \bm \psi_m - \delta_{nm}} < C_{\psi, \Mperp} (m+n)^{\Mperp \nu / d} K^{-\Mperp}
    \end{equation*}
\end{lemma}
\begin{proof}
    We can write
    \begin{align*}
        \bm \psi_n^T \bm \psi_m &= \sum_{k = -K}^K \tilde{w}_{k+K, K} \cos(2\pi k \omega_n)\cos(2 \pi k \omega_m),\\
        &= \frac{1}{4} (S_{n+m} + S_{n-m} + S_{m-n} + S_{-m-n}),
    \end{align*}
    where
    \begin{equation*}
        S_n = S_{\Pi(n)}. 
    \end{equation*}
    The result follows directly from Lemma \ref{lemma:lambda-orthogonality} and the ordering of $\Pi$. 
\end{proof}


We aim to turn the result in Lemma \ref{lemma:orthogonality} into an error term for the normal matrix from a known singular value decomposition. Specifically, we consider the singular value decomposition of $\Psi$:
\begin{equation*}
    \Psi = U (I + \Delta) V^T,
\end{equation*}
where $\Delta$ measures the separation of $\Psi$ from orthogonality.
Using this decomposition, we can represent the normal matrix as
\begin{equation}
\label{eq:FullPerturbation}
    \tilde{B} = Q \Sigma^2 Q^T + E_{\Delta} + E_B + E_T,
\end{equation}
where $Q = U V^T$ and
\begin{equation*}
    E_\Delta = (\Psi-Q)\Sigma^2 Q^T + Q \Sigma^2(\Psi-Q)^T + (\Psi-Q)\Sigma^2(\Psi-Q)^T.
\end{equation*}
We recognize $Q \Sigma^2 Q^T$ as an approximate eigenvalue decomposition of $\tilde{B}$, which is the subject of the Sec.~\ref{subsec:44}. However, first we must bound the error introduced via $E_{\Delta}$:
\begin{lemma}
\label{lemma:EDelta}
    Under the conditions of Lemma \ref{lemma:orthogonality}, there exists a constant $C_\Psi$ such that if
    \begin{equation*}
        \Delta_{\max} = C_\Psi K^{-\Mperp} N^{1+\Mperp\nu/d} < 1,
    \end{equation*}
    the matrix $\Psi$ is full rank with singular values $1+\Delta_{m}$ satisfying $-\Delta_{\max} < \Delta_{m} < \Delta_{\max}$.
    Additionally, the normal matrix error term is bounded as
    \begin{equation*}
        \norm{E_\Delta}_2 < C_{\Delta} K^{-\Mperp} N^{1+\Mperp\nu/d}.
    \end{equation*}
\end{lemma}
\begin{proof}
    In order to bound $E_\Delta$, it is easiest to bound $\norm{\Delta}_2 = \norm{\Psi - Q}_2$. Then, the bound for the full norm is a straightforward application of the triangle inequality. 
    
    The bounds for $\Delta$ are obtained by through the singular values of $\Psi$, which are defined as the square roots of the eigenvalues of $\Psi^T \Psi$. We can bound the eigenvalues of $\Psi^T \Psi$ by a Gershgorin argument using bounds on the entries from Lemma \ref{lemma:orthogonality}. We consider the Gershgorin circles for each row, all centered at $1$, defined as
    \begin{equation*}
        C_m = \left\{z\in\Cbb \mid \abs{z - 1} \leq5 R_m \right\}
    \end{equation*}
    with radii
    \begin{equation*}
        R_m = \sum_{n=0}^N\abs{(\Psi^T \Psi - I)_{mn}}.
    \end{equation*}
    By the Gershgorin theorem (Thm.~\ref{thm:gershgorin}), we know the squares of the singular values of $\Psi$ must lie within the largest of these circles.
    
    We can bound the radii as
    \begin{align}
    \nonumber
        R_m &= \sum_{n=0}^N \abs{\bm \psi_m^T \bm \psi_n -\delta_{mn}}, \\
    \nonumber
            &\leq C_{\bm \psi, \Mperp}K^{-\Mperp} \sum_{n=0}^N (N + n)^{\Mperp \nu/d}, \\
    \label{eq:GershgorinBound}
            &< C_\Psi K^{-\Mperp} N^{1+\Mperp\nu/d}.
    \end{align}
    So,
    \begin{align}
    \label{eq:DeltaBound}
        \abs{(1+\Delta_{m})^2-1} &= \abs{2\Delta_{m} + \Delta_{m}^2},\\
    \nonumber
        &< C_\Psi K^{-\Mperp} N^{1+\Mperp\nu/d}.
    \end{align}
    This bound gives the first part of the theorem, as $\abs{\Delta_{m}} < \abs{2\Delta_{m} + \Delta_{m}^2}$ when $\abs{\Delta_{m}} < 1$.
    Combining this with the fact that $\norm{U}_2 = \norm{V}_2 = 1$ and $\norm{\Sigma^2}_2 \leq \norm{\dobsT}^2_{L^2}$, we have the error term result.
\end{proof}

\subsection{Eigenvalue perturbation}
\label{subsec:44}
Now, we have enough information to directly apply symmetric eigenvalue and eigenvector perturbation theory to Eq.~\eqref{eq:FullPerturbation}. The proof has two steps. First, we show for eigenvalues separated by a gap, the perturbation from $E$ maintains that gap for large enough $K$. From here, we prove the angle of the eigenvector subspace is near that of the associated modes $\bm \psi_n$. At the end of the section, we specify the general invariant subspace theory to the most useful used in Birkhoff RRE as a corollary. 

Before we state the theorem, we first define the angle between subspaces
\begin{definition}[$\nu$-gap, from Stewart and Sun\cite{Stewart1990}]
\label{def:nu-gap}
    Let $\Xcal, \Ycal$ be the $N$-dimensional subspaces of $\Rbb^K$ with associated unitary matrices $X, Y \in \Rbb^{K, N}$. We define the $X$ projection operator as $P_X = X X^T$ and similarly $P_Y = Y Y^T$. For a given matrix norm $\nu$, we define the $\nu$-gap as
    \begin{equation*}
        \rho_{\nu}(\Xcal, \Ycal) = \nu(P_X - P_Y).
    \end{equation*}
    In particular, we define the following subspace angles:
    \begin{align*}
        \rho_2 &= \norm{\sin(\Theta[\Xcal, \Ycal])}_2 = \norm{P_X - P_Y}_2, \\
        \rho_F &= \sqrt{2} \norm{\sin(\Theta[\Xcal, \Ycal])}_F = \norm{P_X - P_Y}_F.
    \end{align*}
\end{definition}

Given this, the eigenvalue perturbation is as follows:
\begin{theorem}
\label{thm:SVD}
    Under Hypotheses \ref{setting}, let $0<\alpha<\beta$ and such that that there exists $L\geq 1$ singular values that $\sigma_n^s \in [\alpha,\beta]$. Additionally, suppose there is a gap $\delta$ such that $\sigma_n^2 \notin [\alpha-\delta,\alpha] \cup [\beta,\beta+\delta]$ for all $n$. 
    % be repeated singular value such that $s = \sigma_{n_1} = \sigma_{n_2} = \dots = \sigma_{n_L}$ for $L\geq 1$. Let the gap between $s$ and the next nearest singular value be 
    % \begin{equation*}
    %     \delta = \min_{n \notin \{n_l\}} \abs{\sigma_n^2 - s^2}.
    % \end{equation*}
    Then, under the condition that $\Delta_{\max} \leq 1/2$ (see Lemma \ref{lemma:EDelta}) and
    \begin{align}
    \nonumber
        \epsilon_B = &\ C_{T, M_T} T^{-M_T} + C_B N^{-2M/d+1} \\
    \nonumber
        &+  C_{\Delta} K^{-\Mperp} N^{1+\Mperp\nu/d}, \\
    \label{eq:spectrum-gap}
        < &\ \frac{\delta}{4},
    \end{align}
    the eigenvalues $\tilde{\sigma}_n^2$ of $\tilde{B}$ are bounded as
    \begin{equation*}
        \abs{\tilde{\sigma}_{n}^2 - \sigma_n^2} \leq \epsilon_B.
    \end{equation*}
    
    \mr{Is there a simple way to do this without indexing? I just cant figure it out...} Furthermore, let $n_\ell$ for $1\leq \ell \leq L$ index the singular values $\sigma_{n_\ell}^2 \in[\alpha,\beta]$. Then, the associated invariant subspace $X_1 = \begin{pmatrix} \xbf_{n_1} & \dots & \xbf_{n_{L}} \end{pmatrix}$ is close to the modes $\Psi_s = \begin{pmatrix} \bm \psi_{n_1} & \dots & \bm \psi_{n_{L}} \end{pmatrix}$ as
    \begin{multline}
    \label{eq:subspace-error}
        \norm{\sin (\Theta[\Rcal(X_1), \Rcal(\Psi_s)])}_F \leq C_{B\Psi} N^{-2M/d+1} \\ + C_{T\Psi}T^{-M_T} + C_{\Delta\Psi} K^{-\Mperp} N^{1+\Mperp\nu/d}.
    \end{multline}
\end{theorem}
\begin{proof}
    The proof for the eigenvalue bounds is a direct application of Weyl's theorem (see Thm.~\ref{thm:Weyl}). We note that $\epsilon$ gives a bound for the spectral radius of the perturbation, so $-\epsilon \leq \epsilon_n \leq \epsilon_1 \leq \epsilon$. A direct application combined with Lemmas \ref{lemma:ET}, \ref{lemma:EB}, and \ref{lemma:EDelta} then gives the eigenvalue result.
    
    For the subspace bound, we use Davis-Kahan $\sin(\Theta)$ theorem (Thm.~\ref{thm:DavisKahan}). To begin, we note that the eigenvalue perturbation theorem guarantees that there are exactly $L$ eigenvalues of $\tilde B$ in the region $[\alpha - \delta/4, \alpha + \delta/4]$. So, $\tilde{B}$ has a spectral resolution (eigenvalue decomposition)
    \begin{equation*}
        \begin{pmatrix}
            X_1^* \\ X_2^*
        \end{pmatrix} \tilde B \begin{pmatrix}
            X_1 & X_2
        \end{pmatrix} = \Diag(L_1, L_2),
    \end{equation*}
    where $L_1 \in \Rbb^{L \times L}$ and $X_1 \in \Rbb^{L \times K+1}$ are the eigenvalue-eigenvector pairs associated with the eigenvalues in $[\alpha-\delta/4, \alpha+\delta/4]$, and $(L_2, X_2)$ are the rest of the eigenvalues and eigenvectors, where $L_2\in \Rbb^{K+1-L \times K+1-L}$ has a spectrum in $\mathbb R \backslash [\alpha-\delta/4, \beta+3\delta/4]$.
    
    For the residual $R$ in Thm.~\ref{thm:DavisKahan}, we want to bound the distance to the subspace $Z = \Psi_s$. Let $M = \Sigma_s^2 \Diag(\sigma_{n_1}^2, \dots, \sigma_{n_L}^2)$. Then, the residual has the form
    \begin{align*}
        R &= \tilde B Z - Z M, \\
          &= (\Psi \Sigma^2 \Psi^T + E_B + E_T)\Psi_s - \Psi_s\Sigma_s^2.
    \end{align*}
    Now, let $P_s\in\Rbb^{N\times L}$ be the projection $P_{s,ij} = \delta_{in_j}$, so that $\Psi_s = \Psi P_s$ and $\Sigma_s^2 = P_s^T \Sigma^2 P_s$. We have
    % $\Psi_\perp$ include the modes of $\Psi$ not in $\Psi_s$ and $\Sigma_\perp^2$ be the associated submatrix of $\Sigma^2$. Then,
    % \begin{multline*}
    %     R = \Psi_s\Sigma_s^2 (\Psi_s^T \Psi_s - I) + \Psi_\perp \Sigma_\perp^2 \Psi_\perp^T \Psi_s + (E_B + E_T) \Psi_s.
    % \end{multline*}
    \begin{align*}
        R &= \Psi \Sigma^2 (\Psi^T\Psi-I)P_s + (E_B + E_T)\Psi P_s.
    \end{align*}
    To bound the above, we note that $\norm{\Sigma^2}_2 \leq \norm{\dobsT}_{L^2}^2$ and that Lemma \ref{lemma:EDelta} gives $1/2 \leq \norm{\Psi}_2\leq 3/2$. For the matrix $(\Psi^T \Psi - I)$ we can bound the $2$ norm by Eq.~\eqref{eq:DeltaBound}. So,
    \begin{multline*}
        \norm{R}_F \leq \frac{3 C_\Psi}{2} \norm{\dobsT}_2^2 K^{-\Mperp} N^{1+\Mperp\nu/d} \\+ \frac{3}{2}(C_{T, M_T} T^{-M_T} + C_B N^{-2M/d+1}).
    \end{multline*}
\end{proof}

The combination of three constants $T$, $N$, and $K$ can make using Thm.~\ref{thm:SVD} unwieldy. This can be remedied by choosing $N$ and $T$ to scale with $K$. In practice, we use $T = \gamma K$ for some $\gamma \geq 1$, so we can dramatically simplify this statement. 
\begin{corollary}
\label{corollary:SVD}
    Take the setting of Thm.~\ref{thm:SVD}. Let $K = \gamma T$ with $\gamma > 0$ and $N = K^{\alpha_*}$ where
    \begin{equation*}
        \alpha_* = \frac{d}{2M/\Mperp +\nu}.
    \end{equation*} 
    Then, there exists a $K_* > 0$ such that for all $K>K_*$ \eqref{eq:spectrum-gap} is satisfied, the subspace in $X_1$ in Thm.~\ref{thm:SVD} is well defined, and the subspace distance is bounded as
    \begin{equation}
    \label{eq:nice-subspace-bound}
        \norm{\sin \Theta[\Rcal(X_1), \Rcal(\Psi)]} \leq C_* K^{-M_*},
    \end{equation}
    where 
    \begin{equation*}
    % \label{eq:Mstar}
        M_* = \min\left(\frac{2M - d}{2M/\Mperp + \nu} , \ M_T \right).
    \end{equation*}
    Moreover, for the same $N$ scaling, we have the bounds
    \begin{equation*}
        \norm{\Psi^T \Psi - I}_2 < C_{\Psi} K^{-M_*}, \qquad \norm{\Psi^T \bm \psi_0}_2 < C_{\psi_0} K^{-M_*}.
    \end{equation*}
\end{corollary}
\begin{proof}
    To obtain the value of $M$, we consider $N$ to scale as $K^\alpha$ for a to-be-determined value of $\alpha$. In this case, the subspace error term \eqref{eq:subspace-error} is
    \begin{multline*}
        \norm{\sin (\Theta[\Rcal(X_1), \Rcal(\Psi_s)])}_F \leq C_{B\Psi} K^{\alpha(-2M/d+1)} \\ + C_{T\Psi}\gamma^{-M_T}K^{-M_T} + C_{\Delta\Psi} K^{-\Mperp+\alpha(1+\Mperp\nu/d)}.
    \end{multline*}
    So, the dominant error will be $\mathcal O(K^{-M_*})$, where
    \begin{equation*}
        M_* = \min\left(\frac{\alpha(2M-d)}{d}, \ M_T, \ \frac{d \Mperp - \alpha(d+\Mperp \nu)}{d}\right).
    \end{equation*}
    We choose the value of $\alpha$ to balance the first and third arguments. Doing so, we find
    \begin{equation*}
        \alpha = \frac{d}{2M/\Mperp +\nu}.
    \end{equation*}
    Substituting this value of $\alpha$ into $M_*$, we find our result.

    The bound on $\Psi^T \Psi - I$ comes from substituting $N$ into \eqref{eq:GershgorinBound}. For the bound on $\Psi^T \bm \psi_0$, we use Lemma \ref{lemma:orthogonality}
    \begin{align*}
        \norm{\Psi^T \bm \psi_0}_2^2 &= \sum_{n=1}^N (\bm \psi_n^T\bm \psi_0)^2, \\
        &\leq C_{\psi,M_\perp}N^{1+2M\perp \nu/d}K^{-2M_\perp}.
    \end{align*}
    Substituting $N$ into this expression gives the result.
\end{proof}
\begin{remark}
    Because $\Mperp$ is arbitrary, the value of $M_*$ can approach arbitrarily close to
    \begin{equation*}
        M_* = \min\left(\frac{2M - d}{\nu} , \ M_T \right).
    \end{equation*}
    \mr{I think that $M_T$ might basically always than $(2M-d)/\nu$. We can choose $M_T = \floor{(M-d)/\nu} = \floor{(2M-d)/\nu - M/\nu}$. So, if $M/\nu > 1$, then $M_T$ is surely the dominant rate. }
\end{remark}



\subsection{The Least-Squares Problem}
\label{subsec:46}
We are now able to prove Thm.~\ref{thm:least-squares}:
\begin{proof}[Proof of Thm.~\ref{thm:least-squares}]
    We begin by fixing an $n$ such that $\abs{\dobsT_n} \neq 0$. We will perturb about the degree two $\halffilter$ that is orthogonal to $\bm \phi_n$, i.e.
    \begin{equation*}
        \halffilter = \frac{1}{1-\cos(2\pi \omega_n)} \begin{pmatrix}
            -\cos(2\pi \omega_n) \\ 2^{-1/2} \\ 0 \\ \vdots \\ 0
        \end{pmatrix}.
    \end{equation*}
    Because we treat $n$ as fixed, the derivative of the characteristic polynomial $P_K'(\lambda_n)$ is fixed.

    
    % The proof has three major steps:
    % \begin{enumerate}
    %     \item We show that the residual of the least squares problem is not too large when a polynomial of the form \eqref{eq:refpoly} is used as an ansatz.
    %     \item We use the matrix perturbation developed in the previous sections to show that the error correction from that polynomial is small in the direction of evaluating $\lambda_n$.
    %     \item We apply polynomial perturbation theory to show that the root cannot move too much.
    % \end{enumerate}

    % \mr{Move this somewhere? ::: and a weighting function $w$ s.t. $W_s > w(x) > w_s$ for $s/2 \leq x \leq 1-s/2$ and $0 < s < 1$}

    % \mr{Be careful with cbf tilde} We start by fixing a value of $\alpha < 1/4$ and by assuming $\omega$ satisfies the condition in Lemma \ref{lemma:DenominatorDistribution}. Then,
    % using Lemma \ref{lemma:DenominatorDistribution}, we choose $\tilde M$ such that $m\geq \tilde M$ implies the continued fraction denominator obeys $\alpha^{-1} K^\eta \leq L_m \leq s K$ where $\eta < 1$. Choosing the associated polynomial $P_{\alpha, \omega, m, p}$, we know the associated vector of coefficients $\halffilter_K$ will be padded by greater than $s K$ zeros. Then, letting $\tilde{\dbf}_K = \Whalf^{-1/2} \halffilter_K$ and using Lemma \ref{lemma:refpolybound}, we have
    % \begin{equation*}
    %     \norm{\tilde{\dbf}_K} \leq \norm{\Whalf^{-1/2}}_2 \norm{\tilde{\filter}_K} \leq w_s^{-1/2} C_\alpha.
    % \end{equation*}

    % We expect the solution to \eqref{eq:transformedleastsquares} to be nearby $\tilde{\dbf}_K$ in certain directions. To see this, we can write the solution to the least squares problem via
    % \begin{equation*}
    %     \begin{pmatrix}
    %         \tilde B + \epsilon I & \bm \psi_0 \\ \bm \psi_0^T & 0 
    %     \end{pmatrix}
    %     \begin{pmatrix}
    %         \dbf_K \\ \mu
    %     \end{pmatrix}
    %     =
    %     \begin{pmatrix}
    %         0 \\ 1
    %     \end{pmatrix}
    % \end{equation*}
    % where $\mu$ is a Lagrange multiplier for the constraint. If we choose $\dbf_K = \tilde{\dbf}_K + \delta \dbf_K$, we find the new system
    % \begin{equation}
    % \label{eq:Deltadsystem}
    %     \begin{pmatrix}
    %         \tilde B + \epsilon I & \bm \psi_0 \\ \bm \psi_0^T & 0 
    %     \end{pmatrix}
    %     \begin{pmatrix}
    %         \delta \dbf_K \\ \mu
    %     \end{pmatrix}
    %     =
    %     \begin{pmatrix}
    %         -(\tilde B + \epsilon I)\tilde{\dbf}_K \\ 1 - \bm \psi_0^T \tilde{\dbf}_K.
    %     \end{pmatrix}
    % \end{equation}
    % By construction, we have $\bm \psi_0^T \tilde{\dbf}_K = P_{\alpha, \omega, m, p}(1) = 1$, so the constraint is satisfied. Similarly, for $1 \leq \abs{n} < K^\eta$, we have $\bm \psi_n^T \tilde \dbf_K = P_{\alpha, \omega, m, p}(\lambda_n) = 0$. So, looking at $\tilde{B}$ applied to $\tilde{\dbf}$, we have
    % \begin{align*}
    %     \norm{\tilde{B} \tilde{\dbf}} &\leq \norm{\sum_{n = 1}^{\infty} 2 \abs{\dobsT_n}^2 \bm \psi_n \bm \psi_n^T \tilde{\dbf}} + \norm{E_T}_F \norm{\dbf}, \\
    %     &\leq w_s^{-1/2} C_\alpha \left(\sum_{n > K^{\eta}} 2 \abs{\dobsT_n}^2 + C_{T, M_T} T^{-M_T}\right),\\
    %     &\leq C_1 K^{\eta(-2 M + 1)}+ C_2 T^{-M_T}.
    % \end{align*}
    % We are specifically interested in how much polynomial evaluation changes at a root $n < K^{\eta}$ by the perturbation $\delta \dbf_K$, which amounts to bounding the value of $\bm \psi_n^T \delta \dbf_K$. To find this, we first must solve the linear system \eqref{eq:Deltadsystem}. The matrix $\tilde{B} + \epsilon I$ is invertible, so the Lagrange multiplier can be found via
    % \begin{equation*}
    %     \mu = -(\bm \psi_0^T (\tilde B+\epsilon I)^{-1} \bm \psi_0)^{-1}.
    % \end{equation*}
    % Then, solving for $\bm \psi_n^T \delta \dbf_K$, we have
    % \begin{equation}
    % \label{eq:Delta-dbf-evaluation}
    %     \bm \psi_n^T \delta \dbf_K = \frac{\bm \psi_n^T (\tilde B + \epsilon I)^{-1} \bm \psi_0}{\bm \psi_0^T (\tilde B + \epsilon I)^{-1} \bm \psi_0}.
    % \end{equation}

    % To bound \eqref{eq:Delta-dbf-evaluation}, we must lower bound the denominator and upper bound the numerator.
    % \mr{Sketchiness starts now.}
    Now, consider the perturbation formula \eqref{eq:lambda-perturbation}. 
    If we bound the numerator quadratic form $\bm \psi_n^T (\tilde B + \epsilon I)^{-1}\bm \psi_0$ to be much smaller than the denominator term $\bm \psi_0^T (\tilde B + \epsilon I)^{-1}\bm \psi_0$, we have our result. 
    For this, let $\delta>0$ be a gap in the spectrum so that $\sigma_m^2 \notin (\sigma_{n}^2 - \delta, \sigma_{n}^2)$ for all $m$.
    Then, we can split the spectrum into $L<\infty$ mode numbers $n_\ell$ where $\sigma_{n_\ell}^2 \geq \sigma_n^2$ and the rest are in the interval $[0, \sigma_n^2-\delta]$.
    By choosing $K>K*$ as in Cor.~\ref{corollary:SVD}, we can diagonalize the operator $\tilde B + \epsilon I$ as
    \begin{equation*}
        \tilde B + \epsilon I = \begin{pmatrix}
            X_1 & X_2
        \end{pmatrix} \begin{pmatrix}
            L_1 & \\ & L_2
        \end{pmatrix}
        \begin{pmatrix}
            X_1^T \\ X_2^T
        \end{pmatrix}
        % \tilde \Psi (\tilde \Sigma^2 + \epsilon I) \tilde \Psi^T + \tilde \Psi_{\perp} (\tilde \Sigma_\perp^2 + \epsilon I) \tilde \Psi_{\perp}^T, 
    \end{equation*}
    where $L_1$ has a spectrum in $[\sigma_n-\delta/4 + \epsilon, \max_{\ell} (\sigma_{n_\ell})+\delta/4+\epsilon]$, $L_2$ has a spectrum in $[\epsilon, \sigma_n-3\delta/4 + \epsilon]$, and $X_1$ and $X_2$ are the associated eigenvectors. 
    % $(\tilde \Sigma^2)_{\ell\ell} = \tilde \sigma_{\ell}^2 \geq \sigma_n^2 - \delta/4 > 3\sigma_n^2/4 $ and $0 \leq ( \tilde \Sigma_{\perp}^2)_{\ell\ell} \leq \sigma_n^2 - 3\delta/4 < \sigma_n^2/4 $. 
    % Additionally, $\tilde \Psi$ orthogonal and its range is close to $\Psi$ \mr{with the bound in the remark}.

    Substituting this representation into \eqref{eq:lambda-perturbation}, we have
    \begin{equation*}
        \delta \lambda_n = -\frac{1}{P'_K(\lambda_n)} \frac{\begin{pmatrix}
            X_1^T \psi_n \\
            X_2^T \psi_n
        \end{pmatrix}^T\begin{pmatrix}
            L_1 & \\ & L_2
        \end{pmatrix}\begin{pmatrix}
            X_1^T \psi_0 \\
            X_2^T \psi_0
        \end{pmatrix}}{\begin{pmatrix}
            X_1^T \psi_0 \\
            X_2^T \psi_0
        \end{pmatrix}^T\begin{pmatrix}
            L_1 & \\ & L_2
        \end{pmatrix}\begin{pmatrix}
            X_1^T \psi_0 \\
            X_2^T \psi_0
        \end{pmatrix}}.
    \end{equation*}
    Due to the regularization, the denominator is bounded from below by $\epsilon$. For the numerator, we will show that $X_2^T \bm \psi_n$ and $X_1^T \bm \psi_0$ are both small. 

    We start with $X_1^T \bm \psi_0$. First, we note that because $X_1$ is unitary,
    \begin{align*}
        \norm{X_1^T \psi_0} &= \norm{X_1 X_1^T \psi_0}. % X_1 is unitary
    \end{align*}
    Now, we can compare this to the projector onto the range of $\Psi_1$ using Corollary \ref{corollary:SVD} and Definition \ref{def:nu-gap}:
    \begin{align*}
         \norm{X_1^T \psi_0} &\leq \norm{(X_1 X_1^T - P_{\Psi_1}) \psi_0} + \norm{P_{\Psi_1} \psi_0} \\ % Subspace angle between X_1 and \Psi_1 is bounded
         &\leq C_* K^{-M_*} + \norm{P_{\Psi_1} \psi_0}.
    \end{align*}
    We can further compare $P_{\Psi_1}$ against $\Psi_1 \Psi_1^T$, giving
    \begin{align*}
        \norm{X_1^T \psi_0} &\leq C_* K^{-M_*} + \norm{(P_{\Psi_1}-\Psi_1 \Psi_1^T)\psi_0} + \norm{\Psi_1 \Psi_1^T \psi_0}.
    \end{align*}
    To bound the middle term, we first note that
    \begin{equation*}
        \norm{P_{\Psi_1} - \Psi_1 \Psi_1^T}_F = \norm{\Psi_1^T \Psi_1 - I}_F.
    \end{equation*}
    Then, because $\Psi_1$ is a submatrix of $\Psi$, the bounds from Corollary \ref{corollary:SVD} apply, giving
    \begin{align*}
        \norm{X_1^T \psi_0} \leq C_1 K^{-M_*}.
    \end{align*}

    As for $X_2^T \bm \psi_n$, we have
    \begin{align*}
        \norm{X_2^T \bm \psi_n}_2 &= \norm{X_2 X_2^T \bm \psi_n}, \\
        &= \norm{(I-X_1 X_1^T) \bm \psi_n}.
    \end{align*}
    Applying the subspace bound from Corollary \ref{corollary:SVD}, we have
    \begin{align*}
        \norm{X_2^T \bm \psi_n}_2 &\leq \norm{(I-P_{\Psi_1}) \bm \psi_n} + \norm{(P_{\Psi_1}-X_1 X_1^T) \bm \psi_n}, \\
        &\leq C_* \norm{\psi_n} K^{-M_*}.
    \end{align*}

    These bounds, combined with the bounds $\norm{L_1}_2 \leq \max_m (\sigma_m)+\delta/4 + \epsilon $ and $\norm{L_2}_2 \leq \sigma_n-3\delta/4 + \epsilon$ give the result.
\end{proof}



==> Deprecated/Sections/5experiments.tex <==
\section{Examples}
\label{sec:examples}

\begin{figure*}
    \centering
    \includegraphics[width=0.7\textwidth]{Figures/ResidualConvergence.png}
    \caption{(a) A Poincar\'e plot of the standard map with $k=0.7$, colored by trajectory classification of integrable, chaotic, or indeterminate. (b) Convergence of the weighted Birkhoff doubling error with respect to trajectory length. Trajectories are colored by the ending point on this plot, with $R > 10^{-5}$ chaotic, $R < 10^{-11}$ integrable, and the rest indeterminate. (c) Convergence of RRE residual with respect to trajectory length. (d) The same as data as (b), on the same domain as (c). From (c) and (d), we see that the RRE residual appears to converge much more rapidly than the weighted Birkhoff average. }
    \label{fig:residual-convergence}
\end{figure*}

In this section, we give two methods of the Birkhoff RRE method applied to symplectic maps. 
In Sec.~\ref{subsec:standard-map}, we apply Birkhoff RRE to the Chirikov standard map in order to investigate its convergence properties.
We show that the convergence of the RRE residual is significantly more efficient in the number of samples than the weighted Birkhoff average (WBA).
As a consequence, RRE can classify trajectories with many fewer symplectic map iterations.
We also show that the roots of the filter polynomial converge like Thm.~\ref{thm:SVD}.

In the second section, we explore the performance of Birkhoff RRE on a stellarator example.
We show how the method classifies chaotic and integrable trajectories, as well as finding Fourier representations of circles and islands.
The rotation number and residuals are also reported.
The symplectic map is obtained by numerically integrating magnetic field lines from an interpolated field, so this example additionally shows the performance on a map with symplecticity breaking error.

\subsection{Standard Map Convergence}
\label{subsec:standard-map}


For the first experiment, we are interested in comparing the convergence and classification of Birkhoff RRE vs WBA. 
For RRE, we measure convergence via the square root of the least-squares residual $R$ defined in \eqref{eq:LeastSquares}. 
For WBA, we use the method of \cite{sander2020}, and compare the averages of two consecutive averages. 
That is, given a symplectic map $\sympmap$ and an observable $\obs$, the WBA residual is
\begin{align*}
    R_{\text{WBA}} &= \norm{\WBA_T[\obs](\xbf_0) - \WBA_T[\obs](\sympmap^T (\xbf_0)) },\\
    &= \norm{\sum_{t=0}^{T-1}w_{t,T}\abf_t - \sum_{t=0}^{T-1}w_{t,T} \abf_{t+T} }.
\end{align*}
We note that both residuals have the same theoretical rate guarantees for $C^\infty$ functions, so it is necessary to numerically check that RRE converges significantly faster.

We are interested in performing a comparison where the total number of map evaluations $N$ is kept constant. 
In particular, we compare $N = (2+\gamma)K+1$ for RRE against $N = 2T$ for WBA, where we choose the `rectangularity' constant to be $\gamma = 2$. 
The example dynamical system we compute with is the Chirikov standard map \eqref{eq:standard-map} with $k=0.7$ (see also Fig.~\ref{fig:standard-map}). In order to handle the map domain $\Tbb \times \Rbb$, we use the smooth observable $\obs : \Tbb \times \Rbb \to \Rbb^2$
\begin{equation*}
    \obs(x,y) = (y+0.5)\begin{pmatrix}
        \cos(2\pi x) \\ \sin(2\pi x)
    \end{pmatrix}.
\end{equation*}

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/misclassification.png}
    \caption{Number of integrable trajectories of Fig.~\ref{fig:residual-convergence} misclassified, with the tolerance of both WBA and RRE set to $10^{-11}$. We see that RRE converges to a low misclassification rate much more efficiently than WBA in the number of map iterations.}
    \label{fig:misclassification}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{Figures/FrequencyConvergence.png}
    \caption{(a) A Poincar\'e plot of the standard map, with three invariant circle with initial $x$ points $0.1$, $0.35$, and $0.4$. (b-d) Convergence plots for the absolute error of the learned frequencies from the polynomial filter vs filter length $K$. The absolute error is computed by comparing to the frequency learned from a $K=1500$ simulation. In (b), we see very rapid convergence for the smooth central circle. In (c), we see slower, but still rapid convergence of the learned frequencies. In (d), for an invariant circle near the edge of chaos, we see significantly slower convergence. The errors are approximately straight in this plot, indicating linear convergence of the roots.}
    \label{fig:frequency-convergence}
\end{figure*}


A Poincar\'e plot of the standard map is found in Fig.~\ref{fig:residual-convergence} (a), where $1000$ trajectories are plotted. 
The trajectories are classified by a long-time $N=10^5$ weighted Birkhoff average, with the three categories of nested invariant circles and islands (blue, $R_{\text{WBA}} < 10^{-11}$), chaos (red, $R_{\text{WBA}} > 10^{-5}$), and indeterminate (green, $10^{-5} \leq R_{\text{WBA}} \leq 10^{-11}$. 
The convergence of the WBA residual used to classify these trajectories as a function of $N$ is found in Fig.~\ref{fig:residual-convergence} (b).
Visually, the `indeterminate' trajectories are typically either at the transition of trajectory types (e.g.~circles to islands or chaos) or have a near small-denominator rotation number.
We note that difficult classification on transitional domains is the typical behavior of any numerical method depending on a continuous quantity.
Additionally, misclassifications are likely to happen for any trajectory classification algorithm, as orbits on one side of a classification boundary can shadow orbits on the other side for arbitrarily long periods of time. 

In Fig.~\ref{fig:residual-convergence} (c), we plot the convergence of the RRE residual for $N \leq 2801$ and $\epsilon = 0$.
For comparison, we plot the WBA residual on the same domain in Fig.~\ref{fig:residual-convergence} (d). 
We see that RRE converges significantly quicker than WBA, with most residuals reaching the machine precision limit before $N=1000$. 
% On all three plots Fig.~\ref{fig:residual-convergence} (b)-(d), we include a black horizontal line at $10^{-11}$ representing the tolerance used for classification for both methods. 
% We can visually confirm that this tolerance effectively separates the majority of trajectories for both methods.

In Fig.~\ref{fig:misclassification}, we compare the number of misclassified integrable trajectories for RRE and WBA.
To obtain this number, we subtract the number of blue trajectories below the $10^{-11}$ tolerance (shown as a black horizontal line in Figs.~\ref{fig:residual-convergence} (b)-(d)) from the total number of blue trajectories for each value of $N$.
We see that RRE classification happens an order of magnitude faster than that of WBA.

Next, we consider the convergence of the roots of the filter polynomials. We consider three invariant circles of the standard map, plotted in Fig.~\ref{fig:frequency-convergence} (a). The three circles are increasingly difficult to approximate. The inner circle is near the core of the nested circles, and is well approximated by a small number of Fourier modes. The yellow circle is more complex, and the green circle is a case on the edge of chaos. 

For each circle, we perform RRE to high accuracy ($K=1500$, $\gamma = 3$) and obtain the rotation number $\omega$ by the process described in Sec.~\ref{subsec:33}. Then, for increasing $K$, we let $P_K$ be the filter polynomial for $\gamma = 3$ fixed and let $\zbf_{K,n}$ be the associated roots. By Thm.~\ref{thm:least-squares}, we expect the roots to converge faster than $\Ocal(K^{-M_*})$ for all $M_*$. To measure this, in Fig.~\ref{fig:frequency-convergence} (b-d) we plot the error
\begin{equation*}
    E_{K,m} = \min_{n} \abs{\zbf_{K,n} - e^{2\pi i m \omega}}
\end{equation*}
for a variety of values of $m$ for each circle. In all cases, we find that the convergence for lower multiples of the rotation number is faster than that for higher multiples. This likely due to the higher prominence of these Fourier modes in the signal. For both the small and medium circles, the rotation number converges to the correct value for values of $K$ less than $100$, corresponding to less than $500$ iterations of the map. For the outer circle, the roots converge significantly more slowly, reaching machine precision at around $K=400$. Additionally, the lines are approximately straight, indicating near linear exponential convergence of $\Ocal(e^{-\alpha K})$ for some $\alpha$ (note that our theorems give a guarantee weaker than linear convergence, but faster than any algebraic convergence). As the circles become more difficult to approximate, higher multiples of the rotation number are found to converge due to a higher number of modes with nontrivial Fourier coefficients, with over $50$ multiples converging to high accuracy for the outer circle.


\subsection{A Stellarator Example}

% \begin{figure*}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/stell_classification.png}
%     \caption{ (Upper left) A Poincar\'e plot of a stellarator example. This example has a mix of invariant circle, island, and chaotic trajectories.  The Birkhoff RRE classification of these trajectories into invariant circles (upper right), islands (bottom left) and chaos (bottom right) are included as well. }
%     \label{fig:stellarator-classification}
% \end{figure*}

% \begin{figure*}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/stell_residuals.png}
%     \caption{}
%     \label{fig:stellarator-residuals}
% \end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{Figures/stell_all_plots.png}
    \caption{Caption}
    \label{fig:stell-all-plots}
\end{figure*}

In this section, we consider our method applied to stellarators, a type of toroidal plasma confinement device. 
Stellarators use large magnetic fields to confine the charged particles that comprise a plasma within the device.
In particular, high energy particles approximately follow magnetic field lines, described by the dynamical system
\begin{equation*}
    \dot{\xbf} = \Bbf(\xbf),
\end{equation*}
where $\Bbf$ is the magnetic field and $\xbf = r \ebf_r(\phi) + z \ebf_z$ is the cylindrical position vector with radial position $r$, azimuthal angle $\phi$, and $z$ is the vertical position. 
Magnetic field line dynamics is a 1.5D Hamiltonian system, and a symplectic map is obtained by following the magnetic ODE is solved numerically over a field period in $\phi$. 
We note that the stellarator map has another dramatic difference from the standard map: the domain $(r, z) \in \mathbb{R}^2$ does not have the rotation number ``built in.'' 
In the case of the standard map, an average of the $y$ coordinate gives the rotation number, whereas the magnetic axis of the stellarator is not necessarily known \textit{a priori}.


We specifically evolve the magnetic field using the Julia \texttt{Tsit5} integrator in combination with the \texttt{StellaratorOptimmizationMetrics.jl} on a configuration with many islands \cite{}.
The magnetic field is interpolated using a grid from a previous simulation using cubic splines. 
We note that both the integrator and the simulation result in potentially non-symplectic errors in the map.
These errors affect the clarity of classifying trajectories, as the Birkhoff RRE residuals do not reach the same low levels as the previous example.
The errors also make identifying rational numbers and rotation numbers more difficult, and the associated tolerances must also be raised. 
This leads to a potentially increased chance of mis-classification.
A Poincar\'e plot showing the $1000$ trajectories is found in Fig.~\ref{fig:stell-all-plots}(a).

We perform the adaptive Birkhoff RRE classification \ref{alg:adaptiveRRE} on $1000$ initial points using $\obs : (r,z) \mapsto (r,z)$, $K_{\min} = 50$, $K_{\max} = 400$, $\Delta K = 50$, $\gamma = 3$, $\epsilon = 0$, and $\delta = 10^{-7}$. 
With these parameters, a maximum of $(2+\gamma)K_{\max}+1 = 2001$ iterations of the map are used per invariant circle, and a minimum of $(2+\gamma)K_{\min}+1 = 251$ iterations are used. 
We note that the cutoff $\delta$ is chosen low enough to distinguish chaos, but high enough that it is resilient to the noise of evaluating the return map (compare to the value of $10^{-11}$ for the standard map). 
After the adaptive RRE algorithm is run, we attempt to fit an invariant circle or island chain to every trajectory, regardless of whether the algorithm converged before the tolerance. 
Then, we evaluate the validation error \ref{eq:validation-error} for each invariant circle.

We plot the invariant circles and islands parameterizations in Fig.~\ref{fig:stell-all-plots}(b-c), with the islands colored by the period $p$. We only plot those with a validation error below the threshold $R_p < 10^{-2}$. The associated rotation numbers to the circles and islands are plotted in Fig.~\ref{fig:stell-all-plots}(f). In Fig.~\ref{fig:stell-all-plots}(d), we plot the chaotic trajectories, defined as those with the RRE residual satisfying $R > 5 \times 10^{-7}$. We note that this value is different than the tolerance used for classification. This is because the standard needed to classify as integrable is separate from the accuracy needed to obtain an effective parameterization. 

In Fig.~\ref{fig:stell-all-plots}(f-g), we plot the Birkhoff RRE residual $R$ and validation error $R_p$ on a logarithmic scale. 
We find the two plots have similar features: both residuals tend to be larger in regions of chaos (the inner core and outer ring) and smaller where there are integrable trajectories. However, we find that the parameterization residual tends to give a sharper indicator of correctness, with chaotic trajectories typically appearing as more red. 

    

==> Deprecated/Sections/6conclusion.tex <==
\section{Conclusions}
\label{sec:conclusions}


- This diagonalization part of the method is seemingly extensible to higher dimensional objects
- Backwards error analysis
- Continuous version? \cite{Duignan}

==> Deprecated/Sections/preamble.tex <==
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{epstopdf}
\usepackage{mathdots}
\usepackage{nicefrac}
\usepackage{enumitem}

\usepackage{algorithm, algpseudocode}
\algrenewcommand\algorithmicrequire{\textbf{Input:}}
\algrenewcommand\algorithmicensure{\textbf{Output:}}

\usepackage{amsthm}
\usepackage{bm}
\usepackage{bbm}
\usepackage{color}

% Theorem stuff
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}%[section]%[theorem]
\newtheorem{remark}[theorem]{Remark}%[section]%[theorem]
\newtheorem{hypotheses}[theorem]{Hypotheses}
\newtheorem{definition}[theorem]{Definition}


\newcommand{\sympmap}{\bm{F}} % Symplectic map 
\newcommand{\obs}{\tilde{\bm{h}}}
\newcommand{\dobs}{\tilde{\bm{g}}}
\newcommand{\obsT}{\bm{h}}
\newcommand{\dobsT}{\bm{g}}
\newcommand{\BA}{\mathcal{B}} % Birkhoff Average
\newcommand{\WBA}{\mathcal{W}\mathcal{B}} % Weighted Birkhoff Average
\newcommand{\WBAw}{w} % the weighting function for the weighted Birkhoff average
\newcommand{\Kback}{\bar{K}} % Length of filter w/o folding
\newcommand{\Whalf}{\tilde{W}_K}
\newcommand{\Mperp}{M_{\perp}} % Continuity number for orthogonality of modes
\newcommand{\refpoly}{P_{\alpha, \omega, n, p}}

\newcommand{\abf}{\bm{a}} % Observable sequence
\newcommand{\Bbf}{\bm{B}} % Magnetic field
\newcommand{\filter}{\bm{c}} % Filter
\newcommand{\halffilter}{\tilde{\bm{c}}} % The folded filter by $P$
\newcommand{\dbf}{\bm{d}} % Weighted filter in proofs
\newcommand{\ebf}{\bm{e}} % Unit Vector
\newcommand{\nbf}{\bm{n}} % Multiindex
\newcommand{\pbf}{\bm{p}} % Something in the least squares proof
\newcommand{\qbf}{\bm{q}} % Something in the least squares proof
\newcommand{\ubf}{\bm{u}} % Difference observable sequence
% \newcommand{\vbf}{\bm{v}} % Just a temporary vector
\newcommand{\xbf}{\bm{x}} % Just a point
\newcommand{\zbf}{\bm{z}} % Invariant Circle
\newcommand{\thetabf}{\bm{\theta}}
\newcommand{\omegabf}{\bm{\omega}}

\newcommand{\xibf}{\bm{\xi}} % Filter for direct solving

\newcommand{\Abf}{\bm{A}} % The right hand side of solving for frequencies

\newcommand{\Cbb}{\mathbb{C}} % Complex numbers
\newcommand{\Nbb}{\mathbb{N}} % Natural numbers
\newcommand{\Rbb}{\mathbb{R}} % Reals
\newcommand{\Tbb}{\mathbb{T}} % Torus
\newcommand{\Zbb}{\mathbb{Z}} % Integers

\newcommand{\Fcal}{\mathcal{F}} % Filter operator
\newcommand{\Ocal}{\mathcal{O}} % Big-O notation
\newcommand{\Rcal}{\mathcal{R}} % Subspace range
\newcommand{\Xcal}{\mathcal{X}} % Subspace
\newcommand{\Ycal}{\mathcal{Y}} % Subspace

% Personal commands
\newcommand{\mr}[1]{{\color{blue}\textbf{MR:} #1}}
\newcommand{\abs}[1]{\left | #1 \right |}
\newcommand{\norm}[1]{\left \lVert #1 \right \rVert}
\newcommand{\ip}[2]{\left\langle #1 , \ #2 \right\rangle }
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\DeclareMathOperator{\Diag}{Diag}
% \newcommand{\dif}{\, \mathrm{d}}
\newcommand{\dif}{\hspace{1pt} \mathrm{d}}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\DeclareMathOperator*{\argmax}{arg\,max}

==> Deprecated/Sections/tmp.tex <==
Things I have to introduce:
  - Time reversal symmetry
  - $g$ function
  - Constraint
  - Integral over ergodic region

  How to do all of this at once?

  Maybe, introduce the problem all at once

==> Deprecated/base_polynomial.tex <==
\section{The Base Polynomial}
\label{subsec:45}

In the introduction, we mentioned that not only do we need control over the normal matrix, but also over the filter that we perturb around. For this, we will use the following polynomial:
\begin{lemma}
\label{lemma:refpolybound}
    Let $0 < \omega \leq 1$ have a sequence of continued fractions approximants with $\{a_n / L_n \}$. For any $n \geq 1$ and $\alpha < 1/4$, define the polynomial
    \begin{equation}
    \label{eq:refpoly}
        \refpoly(z) = \left(\prod_{j = 1}^{\floor{\alpha p L_{n}}}\frac{(z - \lambda_j)(z - \lambda_{-j})}{(1 - \lambda_j)(1 - \lambda_{-j})}\right)
        \left(\prod_{j = \floor{\alpha p L_{n}}+1}^{\floor{{p L_{n}}/{2}}}\frac{(z - \tilde \lambda_j)(z - \tilde \lambda_{-j})}{(1 - \tilde \lambda_j)(1 - \tilde \lambda_{-j})}\right)
    \end{equation}
    where for $0 \leq \ell < p$ and $j\geq 0$
    \begin{equation*}
        \tilde \lambda_{j p + \ell} = e^{2 \pi i (j a_n/L_n + \ell)/p}.
    \end{equation*}
    Then, the polynomial obeys the bound $\abs{\refpoly(z)} \leq C_\alpha$ for $\abs{z} \leq 1$ and $C_\alpha > 1$, where $C_\alpha$ is independent of $\omega$ and $m$.
\end{lemma}
\begin{proof}
    The proof consists of comparing the polynomial above to the polynomial with equispaced nodes 
    \begin{equation*}
        Q_{\alpha, \omega, n, p}(z) = \prod_{j = 1}^{\floor{{L_{n}}/{2}}}\frac{(z - \tilde \lambda_j)(z - \tilde \lambda_{-j})}{(1 - \tilde \lambda_j)(1 - \tilde \lambda_{-j})}.
    \end{equation*}
    We begin by assuming $L_n$ is odd. In this case, the polynomial coefficients of $Q_{\alpha, \omega, n, p}$ can be thought of as a column of the inverse discrete Fourier transform. This is because we have $Q(1) = 1$ and $Q(\tilde \lambda_j) = 0$ for $1 \leq \abs{j} \leq \floor{\nicefrac{L_n}{2}}$ So, $Q_{\alpha, \omega, n, p}$ is simply the interpolation of a unit vector that is nonzero at $1$, i.e.~$\qbf = F^{-1} \ebf_0$ where $\qbf$ are the polynomial coefficients and $F$ is the mapping from Fourier coefficients to values at equispaced nodes.

    The problem of how Fourier interpolation changes when the nodes are perturbed is addressed in \cite{yu2023}. In this paper, Yu and Townsend prove an analogue to the Kadec-$1/4$ theorem \cite{kadets1964} from sampling theory, which states that as long as the locations of Fourier nodes does not move a length farther than $\alpha/4$ from the equispaced grid, the mapping from these Fourier space to these modes $\tilde{F}$ does not differ too much in norm from the standard mapping, i.e.
    \begin{equation*}
        \norm{\tilde F} \leq (1 + \phi_\alpha)\norm{F}_2,
    \end{equation*}
    where $\norm{F} = L_n$ and $\phi_\alpha = 1 - \cos \pi \alpha + \sin \pi \alpha$. Additionally, via Weyl's inequality we have
    \begin{equation*}
        \norm{\tilde F^{-1}}_2 \leq \frac{1}{(1 - \phi_\alpha) \norm F}_2.
    \end{equation*}
    
    We can apply these identities to our problem. In particular, we note that continued fraction approximations obey the bound
    \begin{equation*}
        \abs{\omega - \frac{a_n}{L_n}} < \frac{1}{L_n^2}.
    \end{equation*}
    Using this, we find that $\abs{\lambda_j - \tilde \lambda_j} < \alpha \pi / L_n$ for $\abs{j} < \floor{\alpha L_n}$, obeying the hypothesis for the $1/4$ theorem. Hence, the coefficients of $\refpoly$ 
    \begin{equation*}
        \norm{\pbf_{\alpha, \omega, n}}_2 = \norm{\tilde F^{-1} \ebf_0}_2 \leq \frac{1}{(1-\phi_\alpha)\sqrt{L_n}}. 
    \end{equation*}
    The bound directly follows from the above inequality. 
\end{proof}
The polynomials $\refpoly$ also obeys a bound on its derivatives. In Lemma \ref{lemma:refpolyderivbound}, we show that general polynomials with perturbed roots have lower bounds on their derivatives. We state the result for our polynomial as a corollary:
\begin{corollary}
\label{corollary:refpolyderivbound}
    Let $\alpha < 1/4$. The derivative of $\refpoly(z)$ at each root $\lambda$ obeys
    \begin{equation*}
        \abs{\refpoly'(\lambda)} \geq C N^{-4\alpha}
    \end{equation*}
    for some constant $C$.
\end{corollary}
\begin{proof}
    See Lemma \ref{lemma:refpolyderivbound} and use the bounds from the proof of Lemma \ref{lemma:refpolybound}.
\end{proof}


The polynomials $\refpoly$ also obeys a bound on its derivatives. In Lemma \ref{lemma:refpolyderivbound}, we show that general polynomials with perturbed roots have lower bounds on their derivatives. We state the result for our polynomial as a corollary:
\begin{corollary}
\label{corollary:refpolyderivbound}
    Let $\alpha < 1/4$. The derivative of $\refpoly(z)$ at each root $\lambda$ obeys
    \begin{equation*}
        \abs{\refpoly'(\lambda)} \geq C L_n^{-4\alpha}
    \end{equation*}
    for some constant $C$.
\end{corollary}
\begin{proof}
    See Lemma \ref{lemma:refpolyderivbound} and use the bounds from the proof of Lemma \ref{lemma:refpolybound}.
\end{proof}


==> Deprecated/poly_deriv.tex <==



\subsection{Bounding the polynomial derivative}
\begin{lemma}
\label{lemma:refpolyderivbound}
    Let
    \begin{equation*}
        p(z) = \prod_{\substack{0 \leq n < N \\ n \neq 0}} \frac{z - \lambda_n}{\lambda_0 - \lambda_n}, \qquad \lambda_n = e^{2\pi i (n + \alpha_n)/N},
    \end{equation*}
    where $\alpha_n < \alpha$. If $\alpha < 1/4$, the derivative of $p$ at the roots $\lambda_m$ obeys
    \begin{equation*}
        \abs{p'(\lambda_m)} \geq C N^{-4\alpha}, \qquad 1 \leq m < N
    \end{equation*}
    for some constant $C$.
\end{lemma}
\begin{proof}
    Evaluating $p'$ at a node, we have
    \begin{equation*}
        p'(\lambda_m) = \frac{1}{\lambda_0 - \lambda_m} \prod_{\substack{0 \leq n < N \\ n \neq 0, m}}\frac{\lambda_m - \lambda_n}{\lambda_0 - \lambda_n}.
    \end{equation*}
    We can reorder the product numerator so that
    \begin{equation*}
        p'(\lambda_m) = \frac{1}{\lambda_0 - \lambda_m} \prod_{\substack{0 \leq n < N \\ n \neq 0, m}}\frac{\lambda_m - \lambda_{m - n}}{\lambda_0 - \lambda_n},
    \end{equation*}
    where we identify $\lambda_n = \lambda_{n-N}$. Focusing on the term inside the product, we have
    \begin{multline*}
        \lambda_m - \lambda_n = 2 i e^{\pi i (m + n +\alpha_m + \alpha_n)/N} \sin\left(\pi \frac{m - n + \alpha_m - \alpha_n}{N} \right),
    \end{multline*}
    so
    \begin{multline*}
        \frac{\lambda_m - \lambda_{m-n}}{\lambda_0 - \lambda_n} = - e^{\pi i (\alpha_m + \alpha_{m-n} - \alpha_0 - \alpha_n)} \\
        \times \frac{\sin\left(\pi (n + \alpha_m - \alpha_{m-n})/N \right)}{\sin\left(\pi (n + \alpha_n - \alpha_{0})/N \right)},
    \end{multline*}
    and
    \begin{align*}
        \log & \abs{p'(\lambda_m)} = \log \abs{\frac{1}{\lambda_0 - \lambda_m} } \\
        &+ \sum_{\substack{0 \leq n < N \\ n \neq 0, m}} \log \left(\frac{\sin\left(\pi (n + \alpha_m - \alpha_{m-n})/N \right)}{\sin\left(\pi (n + \alpha_n - \alpha_{0})/N \right)}\right), \\
        =& \ C \\
        &+ \sum_{\substack{0 \leq n < \floor{(N-1)/2} \\ n \neq 0, m}}\log \left(\frac{\sin\left(\pi (n + \alpha_m - \alpha)/N \right)}{\sin\left(\pi (n - \alpha_{0} + \alpha )/N \right)}\right) \\
        &+\sum_{\substack{\ceil{(N-1)/2 + 1} \leq n < N \\ n \neq 0, m}}\log \left(\frac{\sin\left(\pi (n + \alpha_m + \alpha)/N \right)}{\sin\left(\pi (n - \alpha_{0} - \alpha )/N \right)}\right),
    \end{align*}
    where $C$ is a constant that includes the the leading term as well as the factor contributed by $n=N/2$ when $N$ is even, which are both bounded from below. Now, for $0 \leq n < \floor{(N-1)/2}$, we have
    \begin{multline*}
        \sin\left(\frac{\pi(n + \alpha_m - \alpha)}{N}\right) 
        \geq 
        \sin\left( \frac{\pi (n - \alpha_0 + \alpha)}{N}\right) 
        \\
        - \frac{\pi (2 \alpha - \alpha_0 - \alpha_m)}{N}
        \cos\left(\frac{\pi(n + \alpha_m - \alpha)}{N}\right).
    \end{multline*}
    So,
    \begin{align*}
        &\sum_{\substack{0 \leq n < \floor{(N-1)/2} \\ n \neq 0, m}} \log \left(\frac{\sin\left(\pi (n + \alpha_m - \alpha)/N \right)}{\sin\left(\pi (n - \alpha_{0} + \alpha )/N \right)}\right)
        \geq \\ 
        & \quad \geq
        \sum_{\substack{1 \leq n < \floor{(N-1)/2}}} \log \left( 1 - \frac{\pi (2 \alpha - \alpha_0 - \alpha_m)}{N}\right.\\
        &\qquad \qquad \qquad \times \left.\frac{\cos\left(\pi(n + \alpha_m - \alpha)/N\right)}{\sin\left(\pi (n - \alpha_{0} + \alpha )/N \right)}\right),\\
        & \quad \geq 
        \sum_{\substack{1 \leq n < \floor{(N-1)/2}}} \log \left( 1 - \frac{\pi (2 \alpha - \alpha_0 - \alpha_m)}{N}\right.\\
        &\qquad \qquad \qquad \times \left. \cot\left(\pi (n - \alpha_{0} + \alpha )/N \right)\right), \\
        & \quad \geq
        \sum_{\substack{1 \leq n < \floor{(N-1)/2}}} \log \left( 1 - \frac{2 \alpha - \alpha_0 - \alpha_m}{n - \alpha_{0} + \alpha} \right), \\
        & \quad \geq -(2\alpha - \alpha_0 - \alpha_m) \sum_{\substack{1 \leq n < \floor{(N-1)/2}}} \frac{1}{n - \alpha_0 + \alpha}, \\
        % & \geq -\frac{(2 \alpha - \alpha_0 - \alpha_m)(1 + 2 \alpha)}{1-2\alpha} \sum_{\substack{1 \leq n < \floor{(N-1)/2}}} \frac{1}{n - \alpha_{0} + \alpha}, \\
        & \quad \geq  -(2\alpha - \alpha_0 - \alpha_m) \left(\frac{1}{1-\alpha_0 + \alpha} + \int_{1-\alpha_0 + \alpha}^{N/2} \frac{1}{x} \dif x \right), \\
        & \quad =  -(2\alpha - \alpha_0 - \alpha_m)\left(\frac{1}{1-\alpha_0 + \alpha} \right.\\
        &\qquad \qquad \qquad \left.- \log(1 - \alpha_0 + \alpha) - \log 2 + \log(N) \right), \\
        & \quad \geq -(2\alpha - \alpha_0 - \alpha_m) \log N + C,
    \end{align*}
    where we used $\alpha < 1/4$ for the logarithm to have a valid domain and the facts that $1/x \geq \cot x$ for $0 < x \leq \pi/2$ and $\log(1 - y) \geq -y/(1-y)$ for $0 \leq y < 1$. By symmetry, we similarly have
    \begin{multline*}
        \sum_{\substack{\ceil{(N-1)/2 + 1} \leq n < N \\ n \neq 0, m}}\log \left(\frac{\sin\left(\pi (n + \alpha_m + \alpha)/N \right)}{\sin\left(\pi (n - \alpha_{0} - \alpha )/N \right)}\right) \\\geq -(2\alpha + \alpha_0 + \alpha_m) \log N + C,
    \end{multline*}
    In total, we find
    \begin{align*}
        \log \abs{p'(\lambda_m)} \geq - 4 \alpha \log N + C,
    \end{align*}
    so
    \begin{align*}
        \abs{p'(\lambda_m)} \geq C N^{- 4 \alpha }
    \end{align*}
\end{proof}

==> Deprecated/polynomial_derivative_bound.tex <==
\section{Bounding the polynomial derivative}
\begin{lemma}
\label{lemma:refpolyderivbound}
    Let
    \begin{equation*}
        p(z) = \prod_{\substack{0 \leq n < N \\ n \neq 0}} \frac{z - \lambda_n}{\lambda_0 - \lambda_n}, \qquad \lambda_n = e^{2\pi i (n + \alpha_n)/N},
    \end{equation*}
    where $\alpha_n < \alpha$. If $\alpha < 1/4$, the derivative of $p$ at the roots $\lambda_m$ obeys
    \begin{equation*}
        \abs{p'(\lambda_m)} \geq C N^{-4\alpha}, \qquad 1 \leq m < N
    \end{equation*}
    for some constant $C$.
\end{lemma}
\begin{proof}
    Evaluating $p'$ at a node, we have
    \begin{equation*}
        p'(\lambda_m) = \frac{1}{\lambda_0 - \lambda_m} \prod_{\substack{0 \leq n < N \\ n \neq 0, m}}\frac{\lambda_m - \lambda_n}{\lambda_0 - \lambda_n}.
    \end{equation*}
    We can reorder the product numerator so that
    \begin{equation*}
        p'(\lambda_m) = \frac{1}{\lambda_0 - \lambda_m} \prod_{\substack{0 \leq n < N \\ n \neq 0, m}}\frac{\lambda_m - \lambda_{m - n}}{\lambda_0 - \lambda_n},
    \end{equation*}
    where we identify $\lambda_n = \lambda_{n-N}$. Focusing on the term inside the product, we have
    \begin{equation*}
        \lambda_m - \lambda_n = 2 i e^{\pi i (m + n +\alpha_m + \alpha_n)/N} \sin\left(\pi \frac{m - n + \alpha_m - \alpha_n}{N} \right),
    \end{equation*}
    so
    \begin{equation*}
        \frac{\lambda_m - \lambda_{m-n}}{\lambda_0 - \lambda_n} = - e^{\pi i (\alpha_m + \alpha_{m-n} - \alpha_0 - \alpha_n)} \frac{\sin\left(\pi (n + \alpha_m - \alpha_{m-n})/N \right)}{\sin\left(\pi (n + \alpha_n - \alpha_{0})/N \right)},
    \end{equation*}
    and
    \begin{align*}
        \log \abs{p'(\lambda_m)} =& \log \abs{\frac{1}{\lambda_0 - \lambda_m} } + \sum_{\substack{0 \leq n < N \\ n \neq 0, m}} \log \left(\frac{\sin\left(\pi (n + \alpha_m - \alpha_{m-n})/N \right)}{\sin\left(\pi (n + \alpha_n - \alpha_{0})/N \right)}\right), \\
        =& \ C + \sum_{\substack{0 \leq n < \floor{(N-1)/2} \\ n \neq 0, m}}\log \left(\frac{\sin\left(\pi (n + \alpha_m - \alpha)/N \right)}{\sin\left(\pi (n - \alpha_{0} + \alpha )/N \right)}\right) \\
        &+\sum_{\substack{\ceil{(N-1)/2 + 1} \leq n < N \\ n \neq 0, m}}\log \left(\frac{\sin\left(\pi (n + \alpha_m + \alpha)/N \right)}{\sin\left(\pi (n - \alpha_{0} - \alpha )/N \right)}\right),
    \end{align*}
    where $C$ is a constant that includes the the leading term as well as the factor contributed by $n=N/2$ when $N$ is even, which are both bounded from below. Now, for $0 \leq n < \floor{(N-1)/2}$, we have
    \begin{equation*}
        \sin\left(\frac{\pi(n + \alpha_m - \alpha)}{N}\right) 
        \geq 
        \sin\left( \frac{\pi (n - \alpha_0 + \alpha)}{N}\right) 
        - \frac{\pi (2 \alpha - \alpha_0 - \alpha_m)}{N}
        \cos\left(\frac{\pi(n + \alpha_m - \alpha)}{N}\right).
    \end{equation*}
    So,
    \begin{align*}
        \sum_{\substack{0 \leq n < \floor{(N-1)/2} \\ n \neq 0, m}} &\log \left(\frac{\sin\left(\pi (n + \alpha_m - \alpha)/N \right)}{\sin\left(\pi (n - \alpha_{0} + \alpha )/N \right)}\right)
        \geq \\ & \geq
        \sum_{\substack{1 \leq n < \floor{(N-1)/2}}} \log \left( 1 - \frac{\pi (2 \alpha - \alpha_0 - \alpha_m)}{N} \frac{\cos\left(\pi(n + \alpha_m - \alpha)/N\right)}{\sin\left(\pi (n - \alpha_{0} + \alpha )/N \right)}\right),\\
        & \geq 
        \sum_{\substack{1 \leq n < \floor{(N-1)/2}}} \log \left( 1 - \frac{\pi (2 \alpha - \alpha_0 - \alpha_m)}{N} \cot\left(\pi (n - \alpha_{0} + \alpha )/N \right)\right), \\
        & \geq
        \sum_{\substack{1 \leq n < \floor{(N-1)/2}}} \log \left( 1 - \frac{2 \alpha - \alpha_0 - \alpha_m}{n - \alpha_{0} + \alpha} \right), \\
        & \geq -(2\alpha - \alpha_0 - \alpha_m) \sum_{\substack{1 \leq n < \floor{(N-1)/2}}} \frac{1}{n - \alpha_0 + \alpha}, \\
        % & \geq -\frac{(2 \alpha - \alpha_0 - \alpha_m)(1 + 2 \alpha)}{1-2\alpha} \sum_{\substack{1 \leq n < \floor{(N-1)/2}}} \frac{1}{n - \alpha_{0} + \alpha}, \\
        & \geq  -(2\alpha - \alpha_0 - \alpha_m) \left(\frac{1}{1-\alpha_0 + \alpha} + \int_{1-\alpha_0 + \alpha}^{N/2} \frac{1}{x} \dif x \right), \\
        & =  -(2\alpha - \alpha_0 - \alpha_m)\left(\frac{1}{1-\alpha_0 + \alpha} - \log(1 - \alpha_0 + \alpha) - \log 2 + \log(N) \right), \\
        & \geq -(2\alpha - \alpha_0 - \alpha_m) \log N + C,
    \end{align*}
    where we used $\alpha < 1/4$ for the logarithm to have a valid domain and the facts that $1/x \geq \cot x$ for $0 < x \leq \pi/2$ and $\log(1 - y) \geq -y/(1-y)$ for $0 \leq y < 1$. By symmetry, we similarly have
    \begin{align*}
        \sum_{\substack{\ceil{(N-1)/2 + 1} \leq n < N \\ n \neq 0, m}}\log \left(\frac{\sin\left(\pi (n + \alpha_m + \alpha)/N \right)}{\sin\left(\pi (n - \alpha_{0} - \alpha )/N \right)}\right) \geq -(2\alpha + \alpha_0 + \alpha_m) \log N + C,
    \end{align*}
    In total, we find
    \begin{align*}
        \log \abs{p'(\lambda_m)} \geq - 4 \alpha \log N + C,
    \end{align*}
    so
    \begin{align*}
        \abs{p'(\lambda_m)} \geq C N^{- 4 \alpha }
    \end{align*}
\end{proof}

==> Sections/0glossary.tex <==
\section*{Glossary of quantities}
\mr{There are too many letters in this document, so I am making something that at least keeps track of things. Disclaimer: the use of tildes is also inconsistent and mostly bad. It appears that I started using tildes to designate objects that had been projected down by $P$. However, this logic conflicts directly with the thing I define as $A$, making it so that the tildes probably just do more to confuse than help...}
\begin{figure*}
\begin{center}
    \begin{tabular}{c|c}
         Quantity & Meaning \\ \hline
         $\Rbb$ & The real numbers \\
         $\Tbb$ & The torus on $[0,1)$ \\
         $\Zbb$ & The integers \\\
         $C^M$  & $M$-times differentiable functions \\
         $L^p$ & Space of functions with bounded $p$-norm \\
         $M$ & Commonly used for number of derivatives, including... \\
         $M_g$ & for $\dobsT$ \\
         $M_T$ & for Lemma \ref{lemma:ET_entrywise} \mr{Probably a bad name}\\
         $\sympmap$ & The symplectic map \\
         $X$ & The domain of $\sympmap$ \\
         $\zbf$ & An invariant torus or circle \\
         $d$ & The dimension of the invariant torus \\
         $X_0$ & The image of the invariant torus \\
         $\mu$ & The invariant image of $\zbf$ on $X_0$ \\
         $\omega$ & The rotation number in $\Tbb$ \\
         $\omegabf$ & The rotation vector in $\Tbb^d$ \\         
         $\nbf$ & Mode numbers for multidimensional Fourier series \\
         $c$, $\nu$ & Diophantine constants \\
         $\obs$ & Observable on $X$ \\
         $\obsT$ & Observable composed with KAM parameterization on $\Tbb$ \\
         $\obsT_n$ & Fourier coefficients of $\obsT$ \\
         $R_\omega$ & The rotation map on the torus \\
         $\dobsT$ & $\obsT \circ R_\omega - \obsT$, main function used in the analysis \\
         $m$, $n$, $\ell$, $t$, $j$, $k$ & Integers \\
         $\theta$ & Element of $\Tbb$ \\
         $\thetabf$ & Element of $\Tbb^d$\\
         $T$ & Maximum time in Birkhoff average \\
         $\BA_T$ & Finite-time Birkhoff average \\
         $\BA$ & Birkhoff average limit \\
         $\WBA_T$ & Weighted Birkhoff average \\
         $w_{t,T}$ & Weighted Birkhoff average weights \\
         $w$ & Function that $w_{t,T}$ are sampled from \mr{Change this?}\\ 
         & \textbf{and} bound used for non-uniform DFT theorems \\
         $\lambda_{\nbf}$ & Ideal roots of filter polynomial : $e^{2\pi i \nbf \cdot \omegabf}$ \\
         $\filter$ & Filter weights (to be solved for, cf. $w_t$) \\
         $K$ & $\filter$ is length $2K+1$ \\
         $\ksm$ & The parameter in the standard map \\
         $\ebf_n$ & $n$th unit vector \\
         $\abf_t$ & Samples of $\obs$ \\
         $\Abf_t$ & Averaged values of $\abf_t$ with $\filter$ \\
         $\ubf_t$ & $\abf_{t+1} - \abf_t$, samples of $\dobs$ \\
         $U$ & Rectangular block Hankel matrix with entries $\ubf_t$ \\
         & Also used as a matrix in SVD \mr{This one seems fine} \\
    \end{tabular}
\end{center}
\end{figure*}
\begin{figure*}
\begin{center}
    \begin{tabular}{c|c}
        Continued... \\ \hline
         $q_K$ & Polynomial with coefficients $\filter$ \\
         $F_K$ & Filter operation on sequence $\obs$ \\
         $P$, $G$, $P_{\xi}$ & Time reversal projection matrices \\
         $\halffilter$ & Folded filter weights $P \filter$ \\
         $\tilde{A}$ & Matrix in least-squares problem \\ 
         $A$ & Limit of $\tilde{A}$ as $T\to\infty$ \\
         $\epsilon$ & Regularization parameter \\ 
         & Also used for some other small numbers \\
         $J$ & Number of islands \\ 
         $\phi_n$ & Cosine basis function used in the proof \\
         $W$ & Diagonal matrix with weights $w_t$ \\ 
         $\psi_n$ & Weighted cosine basis function $W^{1/2} \phi_n$ \\
         $\dbf$ & Weighted filter polynomial $W^{-1/2} \filter$ \\
         $\tilde{B}$ & Weighted least-squares matrix \\
         $B$ & Limit of $\tilde{B}$ as $T \to \infty$ \\
         $E$ & Error matrix, including \\
         $E_T$ & Error in $\tilde{E}$ due to finite $T$: $\tilde A - A$ \\
         $E_B$ & Error in $B$ due to finite $K$ \\
         $E_\Delta$ & Error in $B$ from SVD with known SVs from non-orthogonality \\
         $\Sigma$ & Matrix of approximate singular values of $B$ \\ 
         $\Delta$ & Matrix used for perturbation of near-orthogonal modes \\
         $N$ & Number of modes $\psi_n$ considered in approximating $\tilde B$ \\&(choice of $N$ discussed after Thm. \ref{thm:SVD}) \\
         $\Xcal$, $\Ycal$ & Subspaces \\
         $X$, $Y$ & orthogonal matrices representing $\Xcal$ and $\Ycal$ \\
         $\delta$ & Spectral gap \\ 
         $L_n$ & Continued fraction denominators of $\omega$ \\
         $q_{\alpha, \omega, n}$ & Polynomials used for comparison \\
         $\gamma$ & Proportionality constant in adaptive algorithm \\
         $\bar{\epsilon}$ & Convergence tolerance of adaptive algorithm \\
         $\Pi(n)$ and $\Pi_{\nbf}(n)$ & Multi-indexing functions
    \end{tabular}
\end{center}
\end{figure*}
